Beyond Control: Exploring Novel File System Objects for Data-Only Attacks on Linux Systems

The widespread deployment of control-flow integrity has propelled non-control data attacks into the mainstream. In the domain of OS kernel exploits, by corrupting critical non-control data, local attackers can directly gain root access or privilege escalation without hijacking the control flow. As a result, OS kernels have been restricting the availability of such non-control data. This forces attackers to continue to search for more exploitable non-control data in OS kernels. However, discovering unknown non-control data can be daunting because they are often tied heavily to semantics and lack universal patterns. We make two contributions in this paper: (1) discover critical non-control objects in the file subsystem and (2) analyze their exploitability. This work represents the first study, with minimal domain knowledge, to semi-automatically discover and evaluate exploitable non-control data within the file subsystem of the Linux kernel. Our solution utilizes a custom analysis and testing framework that statically and dynamically identifies promising candidate objects. Furthermore, we categorize these discovered objects into types that are suitable for various exploit strategies, including a novel strategy necessary to overcome the defense that isolates many of these objects. These objects have the advantage of being exploitable without requiring KASLR, thus making the exploits simpler and more reliable. We use 18 real-world CVEs to evaluate the exploitability of the file system objects using various exploit strategies. We develop 10 end-to-end exploits using a subset of CVEs against the kernel with all state-of-the-art mitigations enabled.

==> 7-defense.tex <==
\section{Mitigation Against Sensitive File Attacks}

We designed a mitigation to protect the file from malicious writing. Our prototype demonstrates negligible overall performance overhead. Protecting all key objects is labor-intensive; moreover, the number of key objects may increase if future works put forward new strategies to make more objects exploitable. In contrast, our design centers around ensuring the integrity of sensitive files. The number of sensitive files is limited, less than 10, and they are primarily used in transition to root, a scenario that is uncommonly encountered. Therefore, we use whitelist mechanisms to protect these files. %\jim{Rare, white list. design trust base,  but simple imple}


\vspace{3pt}
\noindent \textbf{Design.}
We use a whitelist to protect all pre-defined sensitive files, and only root can update the list. We only trust the user as root if \code{cred->uid} is zero, and the other objects that have \code{uid} fields are not trusted, such as \code{inode->i_uid}. Therefore, we need the strongest protection on the whitelist and \code{cred}, such as using hypervisor and TEE, serving as the trusted root.

The core concept is safeguarding the file content integrity of selected sensitive files. Our defense prevents both direct file content corruption (towards page cache and disk storage) and indirect manipulation (through \code{setuid} bit). 
However, metadata does not require protection because the goal of corrupting metadata is to write the file content.
%so attacks can be defended as long as we protect the content's integrity.
%It is because our mitigation guarantees the essential integrity of file contents. 
The defense denies malicious content writing even if the permission metadata is corrupted.
The design concepts are further elaborated below:



\begin{itemize}

\item \textit{Uncache Sensitive Files.}
    Up-to-date file system design caches the file content when accessing it, increasing the possibilities of file content corruption. To avoid this, our defense prevents the sensitive content from being cached.


\item \textit{Disk Commands Sanitization.}
    Attackers can corrupt the file content on the disk by objects containing corrupted sector numbers. Our defense imposes extra sanitization on disk commands accessing the sectors to ensure non-root users cannot write sensitive files' sectors.


\item \textit{Additional Check of \code{setuid} Bit.}
    An unprivileged user can edit sensitive files by adding \code{setuid} bit of an edit executable file owned by root. Given a list of valid programs with \code{setuid}, our defense checks the list and the user in \code{cred} before executing them.

\end{itemize}



% merge this into design concepts
% The files are divided into two groups. The first one includes five sensitive files whose content is protected from malicious writing. First, we disable the page caches for sensitive files; thus, file content lies on the disk only. Then we can encode addition checks about the sector number before sending the writing command to a disk device. The other group contains the executable files whose owners are root without setuid bit. If any one of them has setuid bit, an unprivileged user can execute them as root to write read-only files. We program more checks when executing with setuid. 
\vspace{3pt}
\noindent \textbf{Implementation.}
%
We implement the prototype on the Linux Kernel v5.15. 
Specifically, if the inode name matches any sensitive files when reading or writing a file, we add the \code{O_DIRECT} flag at the very beginning to uncache the sensitive files. 
%
Disk commands sanitization verifies current user's privilege with \code{uid} from \code{current task_struct}
if the disk command is intended for a sensitive file sector. We implement checks on SCSI commands as a prototype, while many other hard disk formats can adopt the same method.
We also provide a helper application to parse the sector number pointing at sensitive files.
Finally, our defense ensures the executable files that can edit another file are never executed with setuid attribute before checking it at \code{bprm_fill_uid} function. 



% If the user is not the root, this command will be denied to send.
% For disk commands sanitization, Our prototype is implemented on SCSI, and , such as NVMe. We define two principles to ensure the file content on the disk is not corrupted by malicious users.

% referecne to evalutation
% 
% We also created a page-aligned temporal buffer for read and write syscall. Because direct I/O requires the buffer that exchanges data with the disk to be aligned with the page size.
%Set the \code{O_DIRECT} flag for the \code{filp} structure in \code{do_filp_open} function: \code{flags |= O_DIRECT};
%behavior of \code{O_DIRECT} mode. If files are not read in 4K-aligned blocks, reading will fail.
%When sending commands (cmd) to the disk device, the function \code{__scsi_execute} should be used. Within this function, we perform the following checks.
% (1) Verify if the command is intended to write to a sector of a sensitive file. Its sector is stored as a global variable since it remains constant as long as the sensitive file is not moved.
%\ziyue{Our prototype is implemented on SCSI, and other hard disk formats like NVMe also work using the same principle.}


% In this work, we implemented our proposed
% defense against DirtyCred on the Linux kernel v5.16.15. In our implementation, we manually modified the ways of allocating cred
% objects and file object in kernel. If the allocation is for privileged
% ones, we allocate them using virtual memory. To be specific, when
% allocating cred objects, we examine the privilege based on the UID of
% the object. If the UID matches GLOBAL_ROOT_UID, which means the allocation is for privileged cred objects, we use vmalloc as the allocator to
% allocate virtual memory for the object. For file objects, we examines
% the file’s mode. If the file is opened with write permission, we will
% allocate the file object with vmalloc accordingly. Our implementation
% is available at [2].

\begin{table}[t!]

\centering
\caption{The performance of our proposed mitigation.}
\label{tab:lmbench}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\bottomrule[0.5pt]
\bottomrule[0.5pt]

\textbf{Item}      & \textbf{Baseline} & \textbf{Mitigation} & \textbf{Overhead (\%)} \\ \hline \rowcolor{mygray}
2p/0k Ctx Switch   & 1.24 & 1.29 & 3.70 \\ 
UDP                & 4.94 & 4.82 & -2.53 \\ \rowcolor{mygray}
TCP                & 6.78 & 6.72 & -0.91 \\ 
0K File Create     & 3.98 & 3.92 & -1.43 \\ \rowcolor{mygray}
0K File Delete     & 2.71 & 2.67 & -1.27 \\ 
10K File Create    & 8.54 & 8.72 & 2.18 \\ \rowcolor{mygray}
10K File Delete    & 4.33 & 4.32 & -0.29 \\
Mmap               & 41.08K & 40.36K & -1.75 \\ \rowcolor{mygray}
Pipe               & 5882.8 & 6212 & 5.60 \\

\bottomrule[0.5pt]
\bottomrule[0.5pt]

\end{tabular}}
\end{table}


\vspace{3pt}
\noindent \textbf{Performance Evaluation.} 
Our experiment environment is to run the Linux kernel on a bare metal machine with 12 Intel cores, 16GB RAM, and a 1TB HDD, and the kernel configuration is on Debian 11 Bullseye. The benchmark uses LMbench v3.0\cite{lmbench}. We ran LMbench five times to obtain the average performance.
%the average parameters obtained from 5 runs in \cref{tab:lmbench}.
%
Compared to the baseline of the unpatched kernel, our mitigation introduces a small overhead.
The overhead of file creation and deletion overhead is less than  3\%, which is reasonable from various perspectives. 
Our defense has a negligible impact on the page cache since access to critical files is infrequent and lightweight. 
Additionally, sector numbers remain largely unchanged, resulting in little performance overhead.


\vspace{3pt}
\noindent \textbf{Discussion.}
% more attack surface. 
% need domain knowledge.
% labor: compatibility of various file systems and device drivers.
% performance overhead
%
We select the sensitive files used in exploits, such as \code{/etc/shadow} and \code{/etc/passwd}. Various applications may introduce additional sensitive files, which require domain knowledge and manual efforts. The complete protection is challenging for development because of the compatibility of various file systems and device drivers. 
%
Furthermore, in our prototype, we assume the strongest protections are in place to secure the pre-defined whitelist of the sensitive files, rather than implementing a fully-fledged trusted execution environment. It's important to note that updating the whitelist may cause new attack surfaces, necessitating careful handling.
And we solicit future researchers to apply more comprehensive techniques in guarding the file systems.


==> back/Old-5-imp.tex <==
\section{Implementation}
\label{sec:design_imple}

% \jim{TODO: the specific data structures, bio-page, inode-imode, and so on, and the reason to choose them: they do not consider the specific file system implementation or different driver}
% \jim{TODO: put the modeling of xarray in implementation}


%And we dump the kernel IR using wllvm. 

This section introduces the design and implementation details of the tool, \underline{F}ile \underline{S}ystem analysis using \underline{T}ype-based \underline{A}ccess \underline{P}ath (\name{}), including the concrete input of the \name{}, the two steps of static analysis, and the process of dynamic verification with the user space triggering program.


\subsection{Initial Object Selection}

\name{} requires three input types, file metadata, file content, and read/write direction, which indicates the essential elements of a file system. We select the input as follows, considering the adaption for different file system implementations or drivers.

\textbf{Selecting reasons for file metadata selection.}
File metadata has an abstracted data structure in VFS that supports any file system implementations; thus, we give the input name of structure type and the inside field, \code{inode->i_mode}. 
\jim{We only need to trace this flag \code{inode->i_mode} after analyzing the semantics of different data structures of the Linux kernel. File metadata consists of four parts: (1) The owner or group identifications of a file (\code{inode->i_uid} and \code{inode->i_gid}), i.e., uid and gid, which are programmed as subfields of structures, \code{kuid_t->uid_t}, \code{kgid_t->gid_t}. We directly treat the objects whose types are these structure types mentioned as sensitive without the further refinement of matching multiple structures because they represent the user identifications. (2) Capability of a file is used for security checks in two ways: One is that the uid and gid inside \code{inode} (represents a file on the disk) are mapped to the user namespace to check the user's capability, and the sensitive data is similar to (1). The other is that load the capability of a file from the disk into a structure \code{kernel_cap_struct} that organizes capability, which is also used in \code{cred} for the capability of a process. Matching this struct type for sensitive data is enough because of its semantics. (3) Access control list is implemented as \code{posix_acl->a_entries}, and the type of field \code{a_entries} is also a struct, \code{posix_acl_entry}, which contains the access control information for different users. (4) The read, write, and execution permissions (rwx) (owner, group, and other) of a file are encoded into the low 12 bits of \code{inode->i_mode}. Besides, more states of a file are encoded into high bits, such as setuid and setgid. This field is an integer, and its value propagates to objects of other types, such as \code{file->f_mode}, which requires tracing its propagation.}





%\wenbo{should be many?}
\textbf{Selecting reasons for file content.}
Because each data exchange request goes through the unified interface in the buffer cache layer, we select the field representing the sector number used by the interface as a source. 

File content is stored into \code{address_space->i_pages} if page cache is enabled, which is treated as input. Due to the complex organization of page pointers, such as \code{xarray}, we leverage a heuristic method to model its usages. Besides, the page that holds the content is eventually handed over to \code{buffer_head->b_page} and \code{bio->bi_io_vec->bv_page} whether page cache is enabled or not. These two are also unified to support different file systems or drivers, and we take them as input, therefore.

\textbf{Selecting reasons for read/write direction.} Read/write direction can be inferred by the events recorded between the main memory and peripheral disk. As shown in \cref{fig:example-read-write}, \code{count_vm_events()} is called when there is a data exchange in which the first argument indicates copying from/to virtual memory. \name{} takes as input the function name with selected values of its first argument, \code{PGPGOUT} and \code{PGPGIN}.

%\code{inode->i_uid->val}

\subsection{Static Analysis}






%\jim{TODO: rewrite}
%Function summary: return type, arg1 type, arg2 type, ...
%, In order to collect a complete set of critical flags, \name{}, supposes to analyze the propagation of the three kinds of input modeling flags on kernel PDG forward and backward. \name{} can directly analyze the data and control dependency of file metadata because Linux kernel implements it as the fields in structures. However, the start-up flags related to file content and read/write direction require a preparation analysis.

%\jim{TODO: merge and rewrite}
The static analysis consists of flags preparing to identify start-up ones and tracing the propagation of the start-up flags.
The process of identifying start-up flags varies for the three kinds of inputs, in which file content and event types require the preparation shown in \cref{fig:overview}. As file metadata is critical non-control data, we only need to find the corresponding flags in structures. 
%After building the  PDG (Program Dependency Graph), \name{} identifies the flags that determine obtaining the page cache. As for read/write direction, \name{} finds the flags that determine to record either write or read, which are on behalf of the data exchange directions. Therefore, preparing flags relies on the data propagation on PDG, which is resolved by \typename{} (\underline{T}ype-based \underline{A}ccess \underline{P}ath).
\name{} traces the propagation of start-up flags to find more effective flags through their data and control dependency, which also requires \typename{} to perform forward and backward analysis. 
%And we find the critical non-control data covers all layers of file system shown in \cref{tab:identified-data}.

\subsubsection{Flag Preparing}
%\name{} needs to identify the flags directly related to the three inputs as the start-up to analyze flag propagation. 
%Because file metadata itself is critical, which requires finding the signifying flags of metadata only by processing the input string. 
\name{} conducts flag preparation for file content and event types to find the start-up flags, which relies on the data propagation based on \typename{} \cref{sec:type-analysis} generated PDG (Program Dependency Graph). As for the start-up flags related to file content, \typename{} finds the location (instruction) of getting the page from page cache by matching the type-based access path. Then it launches a backward analysis on the control-dependency graph to analyze the flags that control the instruction execution. The flags are also refined by type-based access paths. For read/write direction, \name{} identifies the unified function for recording with the event type argument as shown in \cref{fig:example-read-write}. Then it backward tracks the control dependency of executing the function with different arguments to collect the flags using \typename{}.


\subsubsection{Flag Propagation}
\name{} starts from the top struct type and then forwards matches to the bottom field of the access path of start-up flags. Once a matched type-based access path is found, it analyzes the data and controls the dependency of the known flags forward and backward. The analysis iteratively collects flags into an interesting set until there is no new flag. The flag \code{bio->bi_opf} determines the read/write direction that can be identified at the start-up. In \cref{fig:example-data-dependency}, the flag is used to populate to \code{request->cmd_flags} in the lower driver layer, so that we can find the populated flags by data dependency. In \cref{fig:example-control-dependency}, the value of \code{bio->bi_opf} is controlled by a local variable \code{is_read} whose value comes from \code{iov_iter->data_source}. This flag represents the user request at the upper layer, in that \name{} can automatically find by analyzing the control dependency of \code{bio->bi_opf}.

(1) \textit{Forward Analysis.}
\name{} first forwards the PDG for known flags. On the one hand, there is a data dependency where the value of a known flag assigns to a sink flag, as shown in \cref{fig:example-data-dependency}. \name{} collects the sink one into the interesting set. On the other hand, the known flag can be used in a comparison condition to control other flags' values, which should also be put into the set.

(2) \textit{Backward Analysis.}
Similarly, \name{} backward traces the data- and control-dependent flags of known flags. Since the known one can be used as a sink operand in an assignment, \name{} accordingly takes out the source flag as the critical. Besides, the value of the known flag is possibly controlled by another one, which requires the backward tracing of the control flow.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/dynamic.pdf}
    \caption{Dynamic verification. This contains three major steps that are writing-related operation (\ding{172}\ding{173}\ding{174}), reading-related operation (\ding{175}\ding{176}\ding{177}), and verification. }
    \label{fig:dynamicv}
\end{figure}

\subsection{Dynamic Verification}
\label{sec:dyn_veri}

% \subsubsection{Dynamic Verification}
% \label{sec:overview-dynamic}
%\jim{TODO:merge and rewrite}
To verify the effective flags that can be exploited, \name{} resorts to GDB scripts to automatically execute the code containing flags. GDB scripts require not only the types but also the names of type instances, i.e., variables. However, the field names are optimized as integers represent the indices of struct types, and variable names directly vanish in LLVM IR. Type metadata in IR can get ahold of the names, so \typename{} solves the input names of GDB scripts.

There are three steps to verifying a flag's effectiveness. When writing to a file with the write permission normally, we record the flag's value. We try to write to a read-only file by resetting the flag's value using the recorded one. Finally, we check whether the content of the read-only file is changed. If so, the flag is treated as critical.

%There are three kinds of flags related to file metadata, file content, and read/write direction, respectively, at dynamic verification. 
Specifically, there are two parts in~\cref{fig:dynamicv}. The left part represents the kernel running in QEMU, which contains three user space programs corresponding to three verification steps. 
(1) A user space program triggers the flag usage to record the normal value when writing. (2) The second one tries to write a read-only file by resetting the flag with the recorded value using GDB scripts automatically. (3) The final user program re-opens the read-only to check whether its content is changed. 
The right part in~\cref{fig:dynamicv} is GDB scripts, which take as input the variable and field names and manual breakpoints. We combine the user space program to explain. After the writing-related operation hits the breakpoint (\ding{172}), the kernel is paused, and the hook handler (\ding{173}) written in GDB records (\ding{174}) the value of a flag when executing a user program that writes a writable file normally. 
%Then the other program  (or write in particular cases) a read-only file. 
At the time of triggering (\ding{175}) the flag usage for read-only files, GDB then executes the hook handler (\ding{176}) that automatically changes (\ding{177}) the flag with the previously recorded value. After GDB finishes, the last user program verifies the effectiveness of the flag.
%(3) Finally, the user program in QEMU verifies whether changing the flag results in successful writing in the second step by checking the content of the read-only file.


The two user triggering programs (1 and 2) are developed as three forms for three kinds of input. Because the program needs to cautiously invoke a sequence of system calls with the carefully selected arguments, we manually program the three format codes as follows.

\begin{itemize}[leftmargin=*]

\item Change the flags that are metadata when using in security checks at VFS layer. The flags are used by different system calls, such as \code{open} and \code{write}, and we treat them differently. For the flags used in \code{open} (such as \code{inode->i_mode}), we call \code{open} with the arguments that indicate setuid. For the flags in \code{write} (such as \code{file->f_mode}), we call \code{write} with the file descriptor that is created \code{open} that only requests read a file, \code{O_RDONLY}, because the file is readable for a normal user.

\item Change the flags that determine obtaining file content at the page cache layer and the layers lower than it. We also open the read-only file with a read request (\code{O_RDONLY}) to obtain a file descriptor. Then we invoke the system calls that re-map page cache with the file descriptor as an argument, such as \code{mmap}, \code{splice}. After that, we call a system call \code{write} to write into page cache.

\item Change the flags that decide to read/write direction at relatively low layers, which focus on exchanging data between the page in memory and the block number on disk. Although the data exchange processes of file metadata and content are the same at lower layers, eventually. Considering the real scene for attacks, if attackers control the flag to write to the physical disk but cannot control the page's content, they still cannot change with desired values. Thanks to direct IO, which bypasses page cache to directly exchange data with disk and the user buffer page as shown in \cref{fig:file-system}. Therefore, we open a file using direct IO (\code{O_DIRECT}) with a read-only flag. Finally, we call \code{read} to trigger the data exchange of disk with the user buffer, which can turn into a write operation by changing the flag. %During the data exchange, GDB scripts automatically corrupt the flags to reverse the exchange direction.

\end{itemize} 

\subsection{Implementation}
We implement \name{} using LLVM/Clang 15.0.0 based on the IR dumping from wllvm and QEMU 2.11.1 for dynamic verification. The static analysis contains 5k LoC (C++). Dynamic verification includes 451 lines for GDB scripts of dynamic verification (python and C) and 275 lines for the user space triggering program (C). 
%
We evaluate \name{} on Linux kernel v5.15.58 with a manual configuration that enables various file systems. 

==> back/Old-motivating.tex <==
\begin{figure}[t]

% \begin{minted}[highlightlines={3,12}]{c} 
% struct bio {
%   ...
%   unsigned int    bi_opf;	
%   ...
% }

% #define bio_op(bio) \
%   ((bio)->bi_opf & REQ_OP_MASK)

% blk_qc_t submit_bio(struct bio *bio) {
%   ...
%   if (op_is_write(bio_op(bio))) {
%     count_vm_events(PGPGOUT, count);
%   } else {
%     task_io_account_read(bio->bi_iter.bi_size);
%     count_vm_events(PGPGIN, count);
%   }
%   ...
% }
% \end{minted}
\centering
\includegraphics[width=0.95\linewidth]{figure/bio_opf.pdf}
\caption{The motivating example. The non-control data \code{bio->bi_opf} controls the read or write direction.}
\label{fig:example-read-write}
\end{figure}

\section{Motivating Example} 
Infamous ``dirty" CVEs target a small portion of non-control data in the file system of Linux kernel, which are all flags, such as the \code{pipe_buffer->flags} in Dirty Pipe~\cite{CVECVE2059:online}, and the \code{file->f_mode} in Dirty Cred~\cite{lin2022dirtycred}.
%
However, those attacks only target specific non-control data, while the exploitability of the vast majority of non-control data has never been investigated.
%
In the following, we present an example of non-control data, discovered by our tool and can be exploited easily to achieve privilege escalation.
 
%We suspect that there are many more such exploitable non-control data waiting to be discovered.
%the state-of-the-art kernel enforcing schemes only protect limited well-known non-control data. Attacking other data out of protection can easily bypass the schemes.

%\wenbo{refer to the example in the PeX paper, first introduce non-control data controllability, and then discuss which file to attack, after that, give steps about how to exploit }
%Indeed, after skimming through the relevant logic of read/write requests in the file system, we find a new non-control data \code{bio->bi_opf} without much effort. 
\noindent \textbf{Data Explanation.} \cref{fig:example-read-write} shows a data structure named \code{bio} at generic block layer from Linux v5.15.58. 
%
It provides the capability for the kernel to perform block I/O operations.
%
Inside the \code{bio} structure, the field \code{bi_opf} is a flag (line 3) representing the direction of data exchange (line 12).
%
When reading data from disk to memory, the kernel records a reading event \code{PGPGIN}, while writing is the \code{PGPGOUT} (lines 12-17).  
%
In other words, \code{bio->bi_opf} controls the file operations to be either a \textit{read} or \textit{write}.
%
The block layer of the file system relies on \code{bio->bi_opf} totally to decide whether one operation is the read or write operation. 
%
Moreover, we further observe that the system calls \code{read} and \code{write} have the same parameters, containing both the file descriptor and the buffer.
%
Therefore, one can turn a read operation into a write operation by corrupting the \code{bio->bi_opf}. 
%
As a result, the manually-crafted payload in the buffer will be written to the file, even though the file is read-only.



\noindent \textbf{Exploitability.} \jim{(1) heap. (2) time window. (3) how to spray the correct bio.} Kernel allocates \code{bio} in heap using \code{kmalloc} (before v5.11) or \code{kmem_cache_alloc}.

%Because the kernel directly writes to disk using the user's buffer when using direct IO, we control the buffer content ahead before changing direction. 
\noindent \textbf{Experiment.} We write an exploit of \jim{CVExxxx} to corrupt \code{bio->bi_opf} on a real environment with Linux kernel v5.15.58.
%
Our experiment shows that one can easily  exploit \code{bio->bi_opf} to write to \code{/etc/passwd} to achieve privilege escalation.
%
We give detailed steps in the following.
%
First, a non-root user opens the read-only \code{/etc/passwd} with direct IO mode to get a file descriptor \code{fd}. 
%
Then, the user calls \code{read} system call on \code{fd} and passes a buffer \code{buf} with crafted payload. 
%
Before the file system executes \code{submit_bio}, we corrupt \code{bio->bi_opf} from 0 to 1. 
%
As a result, the read becomes write, and the user buffer \code{buf} with the crafted payload is copied to \code{/etc/passwd}.
%
Finally, with the corrupted \code{/etc/passwd}, the non-root user escalates the privilege to root.
%Note that there is a content inconsistency between page cache and disk after directly writing to the disk. 

%\textbf{Data \code{bio->bi_opf}} is an important data struct that represents block I/O operations, which connects the pages in memory and the block number on disk. When there is a data exchange between memory and peripheral disk, a \code{bio} is allocated, and its field \code{bi_opf} signifies the direction of data exchange. Because the content of the user buffer can be controlled by attackers to write to disk when using direct IO. Therefore, we verify this flag same as \code{iomap_dio->flags}. Note that there is a content inconsistency between page cache and disk after directly writing to the disk, we need to check the file content on the disk to verify flag effectiveness.

The above example shows the importance of critical non-control data in the file system. Just by flipping one bit, a non-root user can achieve privilege escalation easily.
%
However, there is no systematic study on the file system to identify the critical non-control data for privilege escalation.
%
To fill up the gap, this paper proposes new techniques and develops an automatic analysis to identify all critical non-control data in the file system.

==> back/Old-tech.tex <==


\section{Data Propagation Using \typename{}}

\jim{Remove this section. }
\label{sec:type-analysis}

%\wenbo{only part of 3.2.2, 3.2.3 is missing?}
%\jim{TODO: rewrite}

\begin{figure}
\centering
\begin{subfigure}[t]{0.9\linewidth}
\begin{minted}[highlightlines={6}]{c}
bool blk_update_request(struct request *req, 
    blk_status_t error, unsigned int nr_bytes) {
...
	if (req->rq_flags & RQF_MIXED_MERGE) {
		req->cmd_flags &= ~REQ_FAILFAST_MASK;
		req->cmd_flags |= req->bio->bi_opf & REQ_FAILFAST_MASK;
	}
...
}
\end{minted}
\caption{Data dependency.}
\label{fig:example-data-dependency}
\end{subfigure}

\begin{subfigure}{0.9\linewidth}
\begin{minted} [highlightlines={11,12,15}]{c}
static inline unsigned char iov_iter_rw(const struct iov_iter *i)
{
	return i->data_source ? WRITE : READ;
}

static ssize_t __blkdev_direct_IO(struct kiocb *iocb, 
    struct iov_iter *iter, unsigned int nr_pages) {
  ...
  bool is_read = (iov_iter_rw(iter) == READ)
  ...
  if (is_read) {
    bio->bi_opf = REQ_OP_READ;
    ...
  } else {
    bio->bi_opf = dio_bio_write_op(iocb);
  }
  ...
}
\end{minted}

\caption{Control dependency.}
\label{fig:example-control-dependency}
\end{subfigure}
\caption{The data- and control-dependency between non-control data.}
\label{fig:example-data-control}

\end{figure}

%\name{} proposes \underline{M}ulti-type based \underline{A}ccess \underline{P}ath (\typename{}) to refine the non-control data propagation, which is field-sensitive and inter-procedural. \name{} needs to trace the propagation of the variables that match the input struct types (field names) to identify more data that has data or control dependency. However, tracing the precise value flow of variables requires a field-sensitive and inter-procedural points-to analysis, which is too heavy to apply to large code base programs \cite{sui2016svf}, such as Linux kernel. We utilize types to refine the non-control data that are propagated from input by data and control dependency, which is scalable and fast for large programs.
We develop \typename{} (\underline{T}ype-based \underline{A}ccess \underline{P}ath) to refine the data propagation in file system, which is field-sensitive and inter-procedural. \typename{} is required to handle the data and control dependency of critical non-control data when resolving the propagation of the critical, as shown in \cref{fig:example-data-control}.

The value-flow analysis based on expensive pointer analysis is not scalable for large code-base programs \cite{sui2018value,sui2016svf}, i.e., Linux kernel. In this work, we develop an efficient and precise approach using the type-based access path, which contains a sequence of pairs, including type and accessed field, to abstract the value-flow propagation in order to capture the tainted flow in a highly efficient manner. 
In one extreme (a naive way to derive the type-based access path), we can identify all the variables with the same types with the tainted input of interest. For example, all variables with \code{unsigned short} type are tainted when matching the field \code{inode->i_mode}, which is also \code{unsigned short}. Only matching the single variable type can cause too many spurious tainted candidates. 
In order to further refine the imprecise results with reasonable overhead for whole-program analysis, we propose to use the type-based access path, which describes how an object is accessed (e.g., through which field of a particular typed aggregated object).
The access path for the above example is $[(inode,i\_mode)(unsigned \; short, \varnothing)]$. Note that the access path possibly includes more than one type of object and its subfield.

Existing works utilize type matching to refine the target functions for indirect calls~\cite{lu2019does, zhang2019pex}, yet they can not directly be applied to general data propagation and face the three problems of analysis precision: (1) \textit{Lack of modeling of memory accesses}. Most existing type-based approaches ~\cite{lu2019does, zhang2019pex} do not analyze the statements of memory access, such as \code{load} and \code{store}, which causes imprecise. (2) \textit{Inaccurate types}. The type analysis requires accurate types. Nevertheless, the state-of-the-art works obtain types from the original types in instructions but not in the source, which is inaccurate and not designed to contain semantics \cite{LLVM30Ty17:online}. 
Our evaluation shows that around 20\% is inaccurate, as shown in \cref{tab:eval-tame}. 
Therefore, this work uses the type system implemented by the metadata, which is recommended by the LLVM community \cite{LLVM30Ty17:online}. 
(3) \textit{Lack of type inference}. Although metadata provides accurate types, it is only instrumented for a limited number of IR variables, which is insufficient for analysis. \typename{} infers more types than instrumented ones.

\typename{} is proposed to use the accurate types that are instrumented by metadata to refine the data propagation. For more accuracy, it models the memory access instructions and refers more types than the instrumented ones. 

%
Last but not least, the type metadata provides not only the accurate types but also the field names and variable names, which facilitate dynamic verification. Because \name{} automatically launches GDB scripts to verify the effectiveness of identified data, which needs to gain the names of the variable and the field to reset the flag's value to save manual efforts.
%is based on the type system implemented by IR metadata, and there are two reasons. (1) Accurate types are required to populate the multi-type-based access paths, which directly influence the analysis results. Since the types in the original type system are not precise or stable, we use the accurate types in metadata followed by the recommendation of LLVM community \cite{LLVM30Ty17:online}. (2) T

%\name{} analyzes non-control data by data structure types with fields (struct-fields), which raise demand for precise and stable types in IR. However, state-of-the-art works still use types directly extracted from IR instructions, which are not designed to contain semantics \cite{LLVM30Ty17:online} and face many problems as discussed in \cref{sec:type-problems}. Furthermore, we need to satisfy the requirement of field names in struct types as the input modeling, and variable names as the output of static analysis to feed to dynamic verification. We develop a \typename{} (\underline{M}etadata-based \underline{A}ccurate ty\underline{P}e analy\underline{S}is) to obtain the accurate types from a reliable type system based on type metadata in IR, and provide field names in structures and variable names for \name{}. 

%However, it is not trivial to get types and names from metadata when analyzing IR instructions. Because the metadata is only instrumented for the defined variables in the C source code, but not for IR variables. For example, metadata is instrumented for a defined variable with struct type, however, not for the field in struct because it has no corresponding variable in C. As shown in \cref{fig:example-data-dependency}, we cannot directly get the type of the field, \code{req->bio->bi_opf} at line 6, which is fatal to analyze critical struct-fields. Due to the SSA-format IR that unfolds C statements, e.g., getting a field is implemented as a \code{getelementptr} instruction and stored to a temporary IR variable. \typename{} needs to infer more types of IR variables at IR variable granularity.

%This section first introduces type problems of the old types in IR instructions. Then we develop \typename{} based on the reliable type system implemented by IR metadata, which faces the gap between the types of C variables and IR variables. \typename{} fills the gap by inferring more types than the instrumented one at IR granularity. The inference rules are listed in \cref{algo:type}.


\subsection{Object and Subfield Types in LLVM IR}
\label{sec:type-problems}
%
A type system is a fundamental building block for static analysis; however, getting the accurate types and their dependence from IR is still challenging. We explain the problems of the original type system that existing works use and insufficient accurate types that are instrumented when using the metadata-based type system. \typename{} is proposed to infer more accurate types based on instrumented metadata.

\subsubsection{Original Type System in LLVM}
To the best of our knowledge, state-of-the-art type analysis is based on the original  LLVM type system, which directly gets types from IR using the interface \code{Value::getType()}. However, the type names in IR are not really designed to be used as semantics, according to LLVM community \cite{LLVM30Ty17:online}. 
%Furthermore, LLVM has discarded to obtain the struct types if they are not defined in current files, i.e., opaque types, which brings difficulty to using the original interface.

The type system has many intractable problems for deriving accurate types. For example, a struct type is possibly optimized to an array that loses type information; a struct type may vanish in IR after linking; the type name is likely added to a suffix string due to opaque pointers in C language, and so on. There are many differences comparing types that get from the original type system at the IR level and the accurate ones from metadata reflecting the types of the source code, as shown in \cref{tab:eval-tame}.
%The new feature disclaims maintaining the pointee type in IR and deprecates all calls to \code{PointerType::getElementType()} and \code{Type::getPointerElementType()}, which increases development costs to obtain pointee type by migrating to different kinds of instructions \cite{OpaquePo49:online}. Besides, the migration instructions are still facing inaccurate type problems. 

% hightlight two points:
% (1) not stable: some work only in O0, and some do not work after linking
% (2) not precise: type names are not really designed to be used as semantic information

\subsubsection{Type System Based on LLVM's Metadata}
LLVM community and researchers try to solve type problems using various methods. 
Type-based alias analysis (TBAA) \cite{TypeEqua7:online} does not distinguish different pointer types and treats all pointers as the same, which is hard to support multi-layer struct analysis. LLVM community instruments type metadata in IR and recommend using it to obtain type information \cite{LLVM30Ty17:online}. 
Therefore, we develop \typename{} to utilize the type metadata for type analysis. 


However, the type metadata is only instrumented at the variable definitions in C code but not for IR, which leads to a gap between the C code variables and IR variables. Much required type information in IR instructions is lost when analyzing IR. More importantly, we cannot get the type of a field that derives from a struct if there is no corresponding defined variable of the field in C code. Our approach based on a type-based access path can successfully solve this issue.

\jim{
TBAA is used in \cite{milburn2022mitigating}, which cannot be used in -O0, requiring specific optimization, nor handle bitcast instruction.
TODO: 1) further comparison with metadata, the granularity of type instrumentation. 2) S\&P'22 accepts two type-based analysis papers: ``Mitigating Information Leakage Vulnerabilities with Type-based Data Isolation \cite{milburn2022mitigating}".
``Practical Program Modularization with Type-Based Dependence Analysis\cite{lu2022practical}". This work is very similar to ours, tracing types of data flow to refine more propagated targets (only in a story of modularization, in which I should learn storytelling skills). Its weakness: First, it has an important assumption: ``\textbf{We assume that the underlying compiler (e.g., LLVM) is correct in providing the type information of data"}. We find that around 20\% types are incorrect, and we use the accurate types implemented by LLVM metadata. Second, it adds the model of the memory-access instructions based on MLTA (this model is only one-layer but not multi-layer? I am not sure, the paper does not clarify this point. We model the memory-access instructions in a manner of multi-layer types). Note the refinement of multi-layer structures is represented as a multiple access path in our paper, but type elevation in their paper. Third, it is an intra-procedural analysis, which cannot apply to our work directly. Fourth, pointer authentication is out of \cite{lu2022practical}'s consideration, but our work can fix most cases, for example, \code{container_of} (an IR variable could have more than one type because it corresponds to more than one variable in source code). Finally, it still avoids handling opaque pointers, which is the future of the LLVM/Clang compiler. Our work is compatible with opaque pointers.
}
%Specifically, the IR of \cref{fig:example-data-dependency} is shown in \cref{fig:example-type-metadata-ir}, the first argument \texttt{\%0} is \code{req} that is a pointer to the base type \code{request}, which is instrumented the metadata \texttt{!11868} using a specific call to \code{llvm.dbg.value} at line 2. Then we can figure out the variable's name ``req", and its type in \texttt{!3540}, which is a pointer type in \texttt{!3541} by analyzing \code{baseType}. There is no instrumented type metadata when taking out the inside field, \code{req->bio}, because the field is not a defined variable in the C source code. \typename{} leverages the existing type metadata to infer more types at IR variable granularity by the rules in blue at \cref{algo:type}.
%which are represented by the rules in blue in \cref{algo:type}.

%    %6 = load i32 (i32)*, i32 (i32)** getelementptr inbounds (%struct.D, %struct.D* @global_d, i64 0, i32 0, i64 0, i32 1), align 8, !dbg !100, !tbaa !101
%   !101 = !{!102, !103, i64 8}
% TBAA does handle bitcast or can not be used in -O0




% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{\linewidth}
% \begin{minted}{c}
% static ssize_t __blkdev_direct_IO(struct kiocb *iocb, 
%         struct iov_iter *iter, unsigned int nr_pages) {
%     struct blkdev_dio *dio;
%     struct bio *bio;
%     ...
%     bio = bio_alloc_kiocb(iocb, nr_pages, &blkdev_dio_pool);
% 	dio = container_of(bio, struct blkdev_dio, bio);
% 	...
% 	    if (is_read) {
% 			bio->bi_opf = REQ_OP_READ;
% 			if (dio->should_dirty)
% 				bio_set_pages_dirty(bio);
% 		}
% 	...
% }

% \end{minted}
% \caption{The non-control data representing read or write direction.}
% \label{fig:example-type-metadata-c}
% \end{subfigure}


% \begin{subfigure}[t]{\linewidth}
% \begin{minted}{llvm}
% define internal i64 @blkdev_direct_IO(%struct.kiocb* noundef %0, %struct.iov_iter* noundef %1) #0 !dbg !6241 {
%   ...
%   %206 = tail call %struct.bio* @bio_alloc_kiocb(%struct.kiocb* noundef %0, i16 noundef zeroext %205, %struct.bio_set* noundef nonnull @blkdev_dio_pool) #6, !dbg !6679
%   call void @llvm.dbg.value(metadata %struct.bio* %206, metadata !6618, metadata !DIExpression()) #7, !dbg !6642
%   %207 = getelementptr %struct.bio, %struct.bio* %206, i64 -1, i32 12, !dbg !6681
%   call void @llvm.dbg.value(metadata i16* %207, metadata !6617, metadata !DIExpression()) #7, !dbg !6642
% }

% \end{minted}
% \caption{The non-control data representing read or write direction.}
% \label{fig:example-type-metadata-ir}
% \end{subfigure}

% \caption{The non-control data representing read or write direction.}
% \label{fig:example-type-metadata}
% \end{figure}


% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{\linewidth}
% \begin{minted}{c}
% #define WC_MODE_FUA(wc)  ((wc)->writeback_fua)

% static inline void bio_set_op_attrs(struct bio *bio, unsigned op,
% 		unsigned op_flags) {
% 	bio->bi_opf = op | op_flags;
% }

% static void __writecache_writeback_pmem(struct dm_writecache *wc, 
%         struct writeback_list *wbl) {
%   struct bio *bio;
%   struct writeback_struct *wb;
%   ...
%   wb = container_of(bio, struct writeback_struct, bio);
%   ...
%   bio_set_op_attrs(bio, REQ_OP_WRITE, WC_MODE_FUA(wc) * REQ_FUA);
%   ...
% }

% \end{minted}
% \caption{The non-control data representing read or write direction.}
% \label{fig:example-type-metadata-c}
% \end{subfigure}


% \begin{subfigure}[t]{\linewidth}
% \begin{minted}{llvm}
% define internal i64 @__writecache_writeback_pmem(%struct.kiocb* noundef %0, %struct.iov_iter* noundef %1) #0 !dbg !6241 {
% }

% \end{minted}
% \caption{The non-control data representing read or write direction.}
% \label{fig:example-type-metadata-ir}
% \end{subfigure}

% \caption{The non-control data representing read or write direction.}
% \label{fig:example-type-metadata}
% \end{figure}


% \newcommand{\mathscalet}{0.8}
% \begin{figure}
%     % \centering
%     % \begin{scriptsize}
%     \[\small\begin{split}\scalebox{\mathscalet}{\textrm{[LOAD]}}{\ \ } & \dfrac{\tau_q(\gamma_q, l_q),\, \theta_q: p=*q}  { \tau_p(\gamma_p = \gamma_q, l_p=l_q-1),\, \theta_p = \theta_q } \\ \scalebox{\mathscalet}{\textrm{[GEP]}}{\ \ \ } &  \dfrac{\tau_q,\, \theta_q: p=\&(q \rightarrow i),\, \tau_i =\text{Type}(\tau_q, i)}  { \begin{aligned}\tau_p(\gamma_p = \gamma_i, l_p = l_i + 1),\, &s\!f_p =[s\!f_q, (\tau_q, i)] \\ &\forall s\!f_p \in \theta_p, \forall s\!f_q \in \theta_q\end{aligned}} \\ \scalebox{\mathscalet}{\textrm{[BINARY]}}\  & \dfrac{\tau_q,\, \theta_q,\, \tau_p,\, \theta_p :r=p \otimes q} { \tau_r = \tau_q,\, \theta_r = \theta_q \bigcup \theta_p } \\  \scalebox{\mathscalet}{\textrm{[PHI]}}\ \ \ & \dfrac{\tau_q,\, \theta_q,\, \tau_p,\, \theta_p :r=\phi(c_1:p,c_2:q)} { \tau_r = \tau_q,\, \theta_r = \theta_q \bigcup \theta_p}\\ \scalebox{\mathscalet}{\textrm{[CAST]}}\ \ 
%  &\dfrac{\tau_q,\, \theta_q,\, \tau_p,\, \theta_p : p=\code{cast}\,q} { \tau_p = \text{Type}(p),\, \theta_p = \theta_q}\\ \\  \scalebox{\mathscalet}{\textrm{[CALL]}}\ \ &\dfrac{\begin{aligned}&\text{\textbf{define}} \, func(arg) \{..., r \hookleftarrow arg\} \\ &\tau_{func}=(\tau_{ret}, \tau_q), \, \tau_q,\, \theta_q, : p=\code{call}\,func(q)\end{aligned}} { \tau_p = \tau_{ret},\, \theta_p = \theta_{func} \oplus \theta_q, \theta_{r\_iter} = \theta_r \oplus \theta_q}\\ \scalebox{\mathscalet}{\textrm{[RETURN]}}&\dfrac{\tau_p,\, \theta_p, : \text{\textbf{define}}\, func(...)\{..., \code{return} \, p\}} { \theta_{func} = \theta_p } \end{split}\]
%     \caption{The inference rules of types when handling different statements with type metadata.}
%     \label{fig:algorithm}
% \end{figure}




% \noindent [LOAD] $\quad \dfrac{p \stackrel{Load}{\longleftarrow} q, \tau \in \mathcal{T}(q)}{ p \stackrel{Copy}{\longleftarrow} \tau}$ 
% \\ \vspace{5pt} % or \mathcal{M}(p) = \mathcal{M}(q)
% \noindent [STORE] $\quad \dfrac{p \stackrel{Store}{\longleftarrow} q, \tau \in \mathcal{T}(q)}{ \tau \stackrel{Copy}{\longleftarrow} q}$ 
% \\ \vspace{5pt}

\subsection{Type-based Access Path (TAP)}

% misunderstanding, type usually means primitive types, such as bool and int.

% \jim{TODO: re-write the figure5 to make it more readable}



\begin{table}
\caption{Type transition rules of \typename{}.}
\label{algo:type}
% \begin{figure}
\rule{\linewidth}{0.5pt}
% \toprule[0.3pt]
% \toprule[0.2pt]
\noindent \small[\textsc{AddrOf}]
$ \dfrac{p \stackrel{AddrOf}{\longleftarrow} o, {\color{blue} \tau \stackrel{Type}{\longleftarrow} \mathcal{F}_1(o)}}{ [(\tau, \varnothing )] \in tap(p)}$ \BlankLine
% \\ \BlankLine\BlankLine
\noindent [\textsc{Field}]$  \dfrac{ p \stackrel{Field_i}{\longleftarrow} q, [\cdots,(\tau_q,\varnothing)] \in tap(q), {\color{blue} (\tau_f, f_i) \stackrel{Type}{\longleftarrow} \mathcal{F}_2(\tau_q, i)}} { [\cdots,(\tau_q, f_i), (\tau_f,\varnothing)] \in tap(p)}$ 
\\ \vspace{5pt}
\noindent [\textsc{Cast}] $ \dfrac{p \stackrel{Cast}{\longleftarrow} q, [\cdots,(\tau_q, \varnothing)] \in tap(q), {\color{blue} \tau_p \stackrel{Type}{\longleftarrow} \mathcal{F}_1(p)}}{[\cdots,(\tau_q, \varnothing),(\tau_p, \varnothing)] \in tap(p)}$
\\ \vspace{5pt}
\noindent [\textsc{Copy}] $\quad  \dfrac{p \stackrel{Copy}{\longleftarrow} q}{tap(q) \subseteq tap(p)}$ 
\\ \vspace{5pt}
%\noindent [LOAD] $\quad \dfrac{p \stackrel{Load}{\longleftarrow} q, [\cdots, (\tau_q,\varnothing)] \in tap(q)}{  [\cdots, (\tau_q,\varnothing)] \in tap(p)}$ 
%p \stackrel{Copy}{\longleftarrow} [\cdots, (\tau_q,\varnothing)]
\noindent [\textsc{Load}] $\quad \dfrac{p \stackrel{Load}{\longleftarrow} q, [\cdots, (\tau,\varnothing)] \in tap(q)}{   pt([\cdots, (\tau,\varnothing)]) \subseteq tap(p) }$
\\ \vspace{5pt} % or \mathcal{M}(p) = \mathcal{M}(q)
%\noindent [STORE] $\quad \dfrac{p \stackrel{Store}{\longleftarrow} q, [\cdots, (\tau_p,\varnothing)] \in tap(p)}{ [\cdots, (\tau_p,\varnothing)] \stackrel{Copy}{\longleftarrow} q}$ 
\noindent [\textsc{Store}] $\quad \dfrac{p \stackrel{Store}{\longleftarrow} q, [\cdots, (\tau,\varnothing)] \in tap(p)}{ tap(q) \subseteq  pt([\cdots, (\tau,\varnothing)])  }$
\\ \vspace{5pt}
\noindent [\textsc{Binary}] $\dfrac{r {\longleftarrow} p\otimes q}{tap(p) \bigcup tap(q) \subseteq tap(r)}$ 
\\ \vspace{5pt}
\noindent [\textsc{Phi}] \qquad $\dfrac{r \longleftarrow \phi(a,b)}{tap(a) \bigcup tap(b) \subseteq tap(r)}$
\\ 
% \bottomrule[0.2pt]
% \bottomrule[0.3pt]
\rule{\linewidth}{0.5pt}
 \begin{tablenotes}
    \footnotesize 
    \item[*] *The rules in blued are getting types from instrumented metadata.
    \end{tablenotes}
% \end{figure}
\end{table}
%\footnotetext{.}
%\notes{}

\begin{figure*}[t]
\centering
\includegraphics[width=.85\linewidth]{figure/llvm.pdf}
% \begin{minted}{llvm}
% define dso_local zeroext i1 @blk_update_request(%struct.request* noundef %0, i8 noundef zeroext %1, i32 noundef %2) #1 !dbg !11864 {
%   call void @llvm.dbg.value(metadata %struct.request* %0, metadata !11868, metadata !DIExpression()), !dbg !11878
%   ...
%   %27 = getelementptr inbounds %struct.request, %struct.request* %0, i64 0, i32 9, !dbg !11955
%   ...
%   %122 = getelementptr inbounds %struct.request, %struct.request* %0, i64 0, i32 3
%   ...
%   %174 = load %struct.bio*, %struct.bio** %27, align 8, !dbg !12136
%   ...
%   %182 = load i32, i32* %122, align 8, !dbg !12149
%   ...
%   %195 = and i32 %182, -1793, !dbg !12163
%   %196 = getelementptr inbounds %struct.bio, %struct.bio* %174, i64 0, i32 2, !dbg !12165
%   %197 = load i32, i32* %196, align 8, !dbg !12165
%   %198 = and i32 %197, 1792, !dbg !12166
%   %199 = or i32 %198, %195, !dbg !12167
%   store i32 %199, i32* %122, align 8, !dbg !12167
% }

% !2929 = !DIDerivedType(tag: DW_TAG_pointer_type, baseType: !2930, size: 64)
% !2930 = distinct !DICompositeType(tag: DW_TAG_structure_type, name: "bio", file: !258, line: 215, size: 768, elements: !2931)
% ...
% !3540 = !DIDerivedType(tag: DW_TAG_pointer_type, baseType: !3541, size: 64)
% !3541 = distinct !DICompositeType(tag: DW_TAG_structure_type, name: "request", file: !87, line: 118, size: 2176, elements: !3542)  
% !3542 = !{!3543, !3544, !3752, !3753, !3754, !3756, !3757, !3758, !3759, !3760, !3761, !3762, !3763, !3768, !3775, !3823, !3824, !3825, !3826, !3827, !3828, !3829, !3830, !3831, !3832, !3833, !3834, !3835, !3847, !3848}
% ...
% !3753 = !DIDerivedType(tag: DW_TAG_member, name: "cmd_flags", scope: !3541, file: !87, line: 123, baseType: !7, size: 32, offset: 192)
% !3760 = !DIDerivedType(tag: DW_TAG_member, name: "bio", scope: !3541, file: !87, line: 133, baseType: !2929, size: 64, offset: 448)
% !11868 = !DILocalVariable(name: "req", arg: 1, scope: !11864, file: !3, line: 1412, type: !3540)
% \end{minted}
\caption{The LLVM IR of data-dependency example in \cref{fig:example-data-control}, which is instrumented with metadata.}
\label{fig:example-type-metadata-ir}
\end{figure*}

\textbf{Program Representation.} 
The set of all variables $V$ is separated into two subsets, $A$ contains all possible abstract objects and their fields, i.e., address-taken variables of a pointer, and $P$ contains all top-level variables, including stack virtual registers (symbols starting with “\%”) and global variables (symbols starting with “@”). $\mathcal{T}$ is a type set that contains basic data types and derived data types. 
%All type metadata is put into a set $\mathcal{M}$. 
There are two ways to get the type from metadata using two functions: (1) $\tau \leftarrow F_1(v)$, we can obtain the type of a defined variable $v \in P$, including local variables (arguments) and global variables; (2) ($\tau_f, f_i) \leftarrow F_2(\tau_s, i)$, we can obtain the $i$th field type $\tau_f$ in a struct type $\tau_s$ based on the instrumented metadata and the field name $f_i$.

%All the non-pointer types (including the types pointers pointed) are in a set of $\Gamma$. 
When handling the value propagation of a variable, \typename{} can reason about the propagation by its type-based access path. We define a type-based access path as a vector, $[(\tau_1, f_1), (\tau_2, f_2),\cdots, (\tau_v, \varnothing)]$, $\tau_1, \tau_2, \tau_v \in \mathcal{T}$, where $f_1, f_2$ are field names. 
Note the final element represent the type of this variable with an empty field. 
For example, the typed-based access path vector of \code{req->bio->bi_opf} is $[(request, bio), (bio, bi\_opf), (unsigned \; int, \varnothing)]$. 
The last element in $\tau$ is the variable type without a field name $\varnothing$. Due to the \textsc{Phi} node and \textsc{Binary} operation, a variable can have multiple access path vectors. We define a map $tap$ that maps a variable to its corresponding set of access path vectors. 
$tap(v)$ obtains the set of type-based access path vectors of variable $v \in P$. Similarly, we define a map $pt$ that maps a set of access path vectors to the pointee set of access path vectors to deal with memory access statements.

%We define points-to sets for pointers $pts(p)$, which map to the set of access path of pointed objects.

%A $\tau$ in $\mathcal{T}$ for a variable $v$ is a sequence of struct-fields, which put together the ones originating from and the one representing the variable's type $\gamma_v$, $[(\gamma_1, f_1), (\gamma_2, f_2),\cdots, (\gamma_v, \varnothing)]$, $\gamma_1, \gamma_2, \gamma_v\in \Gamma$, $f_1, f_2$ are field names. 

Linux kernel is programmed by C language that is translated to LLVM's partial SSA formed. After the SSA conversion, a program is represented by eight types of statements: $p \leftarrow \&q$ (\textsc{AddrOf}), $p \leftarrow \&(q \rightarrow i)$ (\textsc{Field}), $p \leftarrow (type)q $ (\textsc{Cast}), $p \leftarrow q$ (\textsc{Copy}), $p \leftarrow *q$ (\textsc{Load}), $*p \leftarrow q$ (\textsc{Store}), $r \leftarrow p \otimes q$ (\textsc{Binary}), $r \leftarrow \phi(p,\,q)$ (\textsc{Phi}), where $p$, $q$, $r$ $\in P$, $i$ is the index. 

%Because the flags(fields) are barely taken addressed to propagate to pointers, therefore, we do not model load and store. \typename{} handles these statements to infer more accurate types of IR variables.

%For each variable $v$ in $\mathcal{V}$, we define its type as $\tau_v$ and the struct-fields it comes from as $s\!f[(\tau_1, f_1),(\tau_2, f_2),\cdots]$, where $\tau_v$, $\tau_1$, $\tau_2$ $\in \mathcal{T}$, $f_1$ is a field of $\tau_1$, $f_2$ is a field of $\tau_2$. For example, struct-fields of \code{req->bio->bi_opf} at line 6 in \cref{fig:example-data-dependency} are $s\!f[(request, bio),(bio, bi\_opf)]$, and the type deepest field \code{bio->bi_opf} is $\tau_v=(unsigned \; int, 0)$, where 0 indicates it is not a pointer. Due to the phi node and binary operation, a variable possibly originates from multiple struct-fields, thereby we use a set to store the struct-fields for the variable $\theta = s\!f_1 \bigcup s\!f_2 \bigcup \cdots$.

% \begin{figure}
%     \flushleft
%     \begin{small}
%     % \begin{align}
% % &\begin{scriptsize}[LOAD]\end{scriptsize}  \quad {\frac{\tau_q(\gamma_q, l_q), s\!f_q: p=*q}  { \tau_p(\gamma_p = \gamma_q, l_p=l_q-1),\, s\!f_p = s\!f_q} } \\[3pt]
% % &[GEP]   \quad {\frac{\tau_q, s\!f_q: p=\&(q \rightarrow i)}  {\tau_i \hookleftarrow (\tau_q, i),\, \tau_p(\gamma_p = \gamma_i, l_p = l_i + 1),\, s\!f_p =[s\!f_q, (\tau_q, i)]}} \\[3pt]
% % &[BINARY] \\[3pt]
% % &[PHI] \\[3pt]
% % &[CAST] \\[3pt]
%     % \end{align*}
% \noindent \begin{scriptsize}[LOAD] \end{scriptsize} 
% $ {\dfrac{\tau_q(\gamma_q, l_q),\, \theta_q: p=*q}  { \tau_p(\gamma_p = \gamma_q, l_p=l_q-1),\, \theta_p = \theta_q} }$ \\ [5pt]

% \noindent \begin{scriptsize}[GEP] \end{scriptsize} 
% $ {\dfrac{\tau_q,\, \theta_q: p=\&(q \rightarrow i),\, \tau_i =\text{Type}(\tau_q, i)}  { \begin{aligned}\tau_p(\gamma_p = \gamma_i, l_p = l_i + 1),\, &s\!f_p =[s\!f_q, (\tau_q, i)] \\ &\forall s\!f_p \in \theta_p, \forall s\!f_q \in \theta_q\end{aligned}}}$ \\ [5pt]

% \noindent \begin{scriptsize}[BINARY] \end{scriptsize}
% $\dfrac{\tau_q,\, \theta_q,\, \tau_p,\, \theta_p :r=p \otimes q} { \tau_r = \tau_q,\, \theta_r = \theta_q \bigcup \theta_p}$ \\ [5pt] 

% \noindent \begin{scriptsize}[PHI] \end{scriptsize}
% $\dfrac{\tau_q,\, \theta_q,\, \tau_p,\, \theta_p :r=\phi(c_1:p,c_2:q)} { \tau_r = \tau_q,\, \theta_r = \theta_q \bigcup \theta_p}$ \\ [5pt]

% \noindent \begin{scriptsize}[CAST] \end{scriptsize}
% $\dfrac{\tau_q,\, \theta_q,\, \tau_p,\, \theta_p : p=\code{cast}\,q} { \tau_p = \text{Type}(p),\, \theta_p = \theta_q}$ \\ [5pt]

% \noindent \begin{scriptsize}[CALL] \end{scriptsize}
% $\dfrac{\begin{aligned}&\text{\textbf{define}} \, func(arg) \{..., r \hookleftarrow arg\} \\ &\tau_{func}=(\tau_{ret}, \tau_q), \, \tau_q,\, \theta_q, : p=\code{call}\,func(q)\end{aligned}} { \tau_p = \tau_{ret},\, \theta_p = \theta_{func} \oplus \theta_q, \theta_{r\_iter} = \theta_r \oplus \theta_q} $ \\ [5pt]

% \noindent \begin{scriptsize}[RETURN] \end{scriptsize}
% $\dfrac{\tau_p,\, \theta_p, : \text{\textbf{define}}\, func(...)\{..., \code{return} \, p\}} { \theta_{func} = \theta_p } $ \\ [5pt]

%     \end{small}
%     % \end{align}
%     \caption{The transition of types and struct-fields when handling different statements with type metadata. \jim{TODO: align them}}
%     \label{fig:algorithm}
% \end{figure}



% \begin{figure}[t]
% \begin{minted}{c}
% static inline void bio_set_op_attrs(struct bio *bio, unsigned op,
% 		unsigned op_flags)
% {
% 	bio->bi_opf = op | op_flags;
% }

% static void do_region(int op, int op_flags, unsigned region,
% 		      struct dm_io_region *where, struct dpages *dp,
% 		      struct io *io)
% {
% ...
%     bio_set_op_attrs(bio, op, op_flags);
% ...
% }

% static void dispatch_io(int op, int op_flags, unsigned int num_regions,
% 			struct dm_io_region *where, struct dpages *dp,
% 			struct io *io, int sync)
% {
% ...
%     do_region(op, op_flags, i, where + i, dp, io);
% ...
% }

% static int async_io(struct dm_io_client *client, unsigned int num_regions,
% 		    struct dm_io_region *where, int op, int op_flags,
% 		    struct dpages *dp, io_notify_fn fn, void *context)
% {
% ...
%     dispatch_io(op, op_flags, num_regions, where, dp, io, 0);
%     return 0;
% }
 
% int dm_io(struct dm_io_request *io_req, unsigned num_regions,
%   struct dm_io_region *where, unsigned long *sync_error_bits)
% {
% ...
%   return async_io(io_req->client, num_regions, where, io_req->bi_op,
% 		io_req->bi_op_flags, &dp, io_req->notify.fn,
% 		io_req->notify.context);
% }

% \end{minted}
% \caption{Inter-procedural data population\jim{TODO: re-draw this pic to save space and highlight the parameter passing, drop the unnecessary data/parameter}.}
% \label{fig:inter-procedural}
% \end{figure}


\textbf{Type-based Access Path Transition.} \cref{algo:type} lists the eight kinds of statements, and the rules in blue obtain the types from metadata. 
(1) \textsc{AddrOf}: When a pointer $p$ initially points to $o$, \typename{} obtains the type in the metadata of $o$ and puts the type in the format of type-based access path vector $[(\tau, \varnothing)]$. Then it is put into the vector set of $p$, i.e., $tap(p)$. 
%This rule applies to global variables and local variables (parameters). 
(2) \textsc{Field}: When taking the $i$-th field of $q$ and storing its address to $p$, \typename{} derives the $i$-th field's type $\tau_f$ from the metadata of the known structure type $\tau_q$ with, and field name $f_i$. The field name replaces the empty field $\varnothing$ of the access path, and the field type with an empty type is pushed back to the access path vector. 
(3) \textsc{Cast}: The variable $q$ originates from $tap(q)$ is assigned to a variable $p$ that has a different type $\tau_p$ by casting, \typename{} resorts to type metadata to get the casting type $\tau_p$. Then the casting type is spliced behind every access path vector in $tap(q)$ to inherit the origin one. 
(4) \textsc{Copy}: We put each vector in set of the source operand $q$ to the set of the sink operand $p$, if there is an assignment between two variables. 
(5) \textsc{Load}: When $p$ loads from a pointer $q$, the vectors in the pointee set of $q$ are put into the vector set of $q$. In other words, the pointee set is a subset of the vector set of variables after loading.
(6) Store: When storing $q$ to $p$, the vector set of $q$ is a subset of the pointee vector set of pointer $p$.
(7) \textsc{Binary}: The variable $r$ is computed by two operands $p$ and $q$, so the value of $r$ is affected by the two operands. Therefore, \typename{} takes the union of the two vector sets for $tap(r)$. 
(8) A \textsc{Phi} node has multiple incoming values, \typename{} takes the union of vector sets of all incoming operands similarly as before.

We combine the example in \cref{fig:example-type-metadata-ir} to discuss the rules, which is the IR code of \cref{fig:example-data-dependency}. The first parameter \texttt{\%0} is instrumented in its type metadata \code{!11868} at line 2 (\textsc{AddrOf}). The metadata contains variable name \code{req}, and its type is in \code{!3540}, which implies it is a pointer type that points to a base type in \code{!3541}, i.e., struct type \code{request}. Therefore, the access path of \texttt{\%0} is $(request, \varnothing)$. One user of \texttt{\%0} is \texttt{\%27} (Field) at line 4, which means to get the ninth element address of \texttt{\%0}, counting from 0. After analyzing the elements of struct \code{request} using \code{!3542}, the ninth field is instrumented in \code{!3760} whose name is \code{bio} and type is in \code{!2929}. 
The access path set of \texttt{\%27} has a element, $(request, bio), (bio, \varnothing)$. Furthermore, we find that \texttt{\%27} is used in \texttt{\%174} at line 8, and the set is inherited (Load). Then it comes to another \code{getelementptr} (Field) at line 13, \typename{} figures type-based access path set of \texttt{\%196} has $[(request, bio), (bio, bi\_opf), (unsigned \; int, \varnothing)]$.
As mentioned before, binary operations introduce more than one access path. After handling the load from \texttt{\%196}, \typename{} encounters \code{and} and \code{or} instructions. The other operand of \code{and} is a constant, which does not influence the type-based access path. However, there are two operands in \code{or} instruction (Binary), \texttt{\%199}. The path of first (\texttt{\%199}) is $[(request, bio), (bio, bi\_opf),(unsigned \; int, \varnothing)$, the second is $[(request, cmd\_flags), (unsigned \; int, \varnothing)]$, \typename{} merges the two into a set. Finally, we find that there is a store instruction that populates from $(bio, bi\_opf)$, which is a critical flag that determines read/write direction, and the sink path $(request, cmd\_flags)$ is marked as critical also.

\begin{figure}[t]
\includegraphics[width=0.9\linewidth]{figure/cross-func.pdf}
\caption{Inter-procedural data population.}
\label{fig:inter-procedural}
\end{figure}
%$\theta = \{ s\!f_1[(request, bio), (bio, bi\_opf)], s\!f_2[(request, cmd\_flags\\)]\}$. \typename{} deals with \textbf{PHI} similarly by merging the struct-fields of each incoming value. As for \textbf{CAST}, \typename{} turns to type metadata to derive the accurate type and keeps the struct-fields same. Finally, we find that there is a store instruction that populates from $(bio, bi\_opf)$, which is a critical flag that determines read/write direction, and the sink struct-field $(request, cmd\_flags)$ is marked as critical also.

\textbf{Inter-procedural Analysis.}
We analyze the type-based access paths in an inter-procedural manner, which is necessary for \name{} to collect a complete set of critical flags (or tainted flows). 
As shown in \cref{fig:inter-procedural}, a function \code{dm_io()} calls \code{async_io()}, passing the arguments \code{io_req->bi_op} and \code{io_req->bi_op_flags}. 
The two flags eventually pass to \code{bio_set_op_attrs()} to set the value of \code{bio->bi_opf} after three layers of function calls, which are also critical. \typename{} splices the access paths of the argument at the call site before going forward to the callee to analyze deeper propagation between the access paths. \typename{} inter-procedurally analyzes the returned access paths of callee also. For example, function \code{pagecache_get_page()} returns a page pointer in page cache ($[(address\_space, i\_pages)]$), and the caller can get the returned value with the type-based access paths, knowing it is a page from the page cache.

==> back/_1-intro_bak.tex <==
\section{Introduction}

% (1) basic exploit: need leak
% (2) only a write without leaking.}

%介绍安全发展，现在到了non-control data
% non control data, page table cred等等一些敏感的都被保护了。
%介绍三个dirty CVE，引出看似无害的non-control data 同样对系统有影响，引出不sysmatically
%chanlleng summarize一段
%Tool实现和evaluation结果summarize一段
% contribution总结


%The operating system kernel often acts as the de facto trusted computing base for user space applications. 
%
% Non-control data presents as a prevailing attack surface in the operating system kernel.
% %The attack and defense on the operating system kernel have evolved over recent decades, from kernel code injection attacks to kernel code reuse attacks and then to non-control data attacks.
% %
% Nowadays, various protection techniques have been proposed and deployed to defend against kernel code injection attacks~\cite{azab2014hypervision,azab2016skee} and code reuse attacks\cite{cficarlini2015control,ge2016fine,yang2019arm,denis2020camouflage,yoo2022kernel,ClangCFI41:online}.
% %
% As a result, attackers cannot corrupt the code and the control data in the kernel, such as return addresses and function pointers.
% %
% %attracts many powerful attacks. Kernel developers and security researchers propose a number of defenses. One solution is CFI (Control-flow Integrity), which is an efficient defense to protect kernel from hijacking control-flow attacks. Widespread deployment of CFI in mainline Linux kernel on different architectures \cite{ClangCFI41:online, x86Addsu43:online, pal, camouflage,linuxaddcfi:online,cfiabadi2005lfar,cfiapplepa,cfiburow2017control, cficarlini2015control, cfiteam2015rap} making it difficult to corrupt control data for kernel exploitation.
% Naturally, attackers turn to non-control data for exploits.
% %
% %
% Over the years, attackers have designed various methods of exploiting sensitive non-control data in the kernel, such as page tables\cite{US22WANG2:online}, credentials structures, and user mode helper loading path in the Linux kernel~\cite{shen2017defeating}.
% %
% On the other side, security researchers have proposed various techniques, such as data-flow integrity, to monitor and protect this sensitive data~\cite {chen2005non,xiao2015kernel,song2016enforcing,2017PT,proskurin2020xmp,lin2022dirtycred,xu2022regvault}.





%"control flow hijack is defended heavily so people start using data-only attacks." --> "the most popular one is modprobe_path which is a global variable" --> "writing to global variable requires defeating KASLR, which is an additional complexity and can hurt exploit reliability" --> "there are in fact critical non-control data on heap as well. cred is an example but it is also defended in many cases" --> "we look into heap objects in the file subsystem because it controls much of kernel behaviors (e.g., being able to write to critical files leads to privilege escalation)"

Control flow hijacking used to be the mainstream attack method to exploit memory errors; however, it has become difficult to achieve after the Control Flow Integrity (CFI) defense is introduced.
On the other hand, in the context of the Linux and Android kernels, data-only attacks have been become popular not only because it does not require control flow hijack but also due to its simplicity. 
For example, the single most prevalent object being targeted in the Linux kernel is \code{modprobe_path}~\cite{CVE-2021-42008:online, CVE-2021-43267:online, CVE-2022-0185:online, CVE-2022-27666:online, CVE-2022-32250:online, CVE-2022-34918:online, CVE-2023-0179:online, CVE-2023-32233:online}. As long as an attacker can overwrite its value with a file path that points to the attacker-controlled executable file, it will be executed with the root privilege~\cite{modprobe_path}. There is no need to collect and stitch together ROP gadgets in such data-only attacks.
%In the context of the Linux kernel, many previous studies find more objects to facilitate the attack by providing various primitives~\cite{chen2019slake, chen2020systematic, liu2022release, wang2023alphaexp}, such as hijacking control flow, bypassing protection mechanisms, and leaking heap pointer address. However, they can not directly lead to privilege escalation. Many become no longer exploitable when all the protection mechanisms are enabled.
%
%These protections have been proposed and deployed in commercial kernels against kernel code injection attacks~\cite{azab2014hypervision,azab2016skee} and code reuse attacks\cite{cficarlini2015control,ge2016fine,ClangCFI41:online, yang2019arm,denis2020camouflage,yoo2022kernel}. For example, Android and Windows kernels have deployed CFI to defend attacks~\cite{androidcfi, wincfi}.

%As a result, attackers turn to non-control data in the kernel~\cite{US22WANG2:online,shen2017defeating, WillsRoo23:online}.
%

%\jim{Previous works aim to find the objects that facilitate the exploit of control flow hijacking~\cite{chen2020systematic, liu2022release, wang2023alphaexp}, such as finding objects, bypassing protection mechanisms, leaking heap pointer address, and so on. However, they can not directly lead to privilege escalation, and many of them are no longer exploitable when enabling all the protection mechanisms.}

%=======================================================
% Non-control data is detrimental that often leads to PE
%=======================================================
Non-control data become popular exploitable targets in the operating system kernel~\cite{US22WANG2:online,shen2017defeating, WillsRoo23:online}, while various protection techniques are proposed to protect them~\cite{PrivGuard, li2023hybrid, 2017PT, song2016enforcing}, and some are enforced in commercial kernels, such as \code{cred}~\cite{appleoss24:online, samsung1, samsung2}, and page table~\cite{appleoss24:online,samsung1, samsung2}, well-used \code{msg_msg} no longer available in Android~\cite{blackhat2023}.

%=======================================================================
% The Main challenge is that we don't know what the critical objects are
%=======================================================================
However, the protections fall apart when exploiting unrevealed non-control data outside the protected ones. 
%Malicious corruption toward the protected data becomes exceedingly challenging in commercial kernels.
%
Most protections safeguard manually selected data, leaving many critical non-control data in the dark. 
%Unias \cite{li2023hybrid} identifies the global variables not modified after kernel initialization. However, corrupting global variables usually requires arbitrary memory writes, which is relatively hard to obtain in real-world exploits. 
%
%
KENALI~\cite{song2016enforcing} makes an effort to identify the sensitive non-control data automatically. It uses static analysis to infer sensitive data by tracking POSIX-compatible error codes.
%
However, KENALI does not confirm whether the corruption of sensitive data can result in privilege escalation.
%
Consequently, KENALI overprotects the non-critical data and increases overhead.
Even worse, KENALI fails to discover critical non-control data unrelated to the error code. Exploiting these unprotected data results in privilege escalation.
%
%It is only until the attacks happen that security researchers pay attention to new data.
%
For example, Dirty COW (CVE-2016-5195)~\cite{DirtyCOW66:online} and another recent powerful Dirty Pipe (CVE-2022-0847)~\cite{CVECVE2059:online}.
%
State-of-the-art program analysis tools fail to detect the risk in the first place. 
It is only until the attacks happen that security researchers pay attention to new data.
%
As for the critical non-controlled data leading to privilege escalation, to the best of our knowledge, there is no work to automatically identify them.

\ziyue{However, we observe three challenges in combating non-control data exploits in the kernel. 
\textbf{\textit{Accurarcy}} Firstly, current approaches discover objects based on simple pattern. (cite kenali)
\textbf{\textit{Scalability}} Second, many works need human effort. (cite dirty cred, dirty pipe, page table)
\textbf{\textit{Validity}} Finally, the security impacts of the discovered objects remain unknown. (cite KENALI)}


% The hazards many critical non-control data can cause remain undiscovered for two reasons.
% %
% First, many critical non-control data are still in the dark, and no automatic tools exist to identify them. Data criticality relies highly on its semantics, such as the data representing page tables, process credentials, and so on. Critical non-control data have various functionalities and semantics, making identification difficult.
% %
% Second, exploiting a critical non-control object as a corrupting target requires aligning it with the capabilities of a memory corruption vulnerability. 
% %
% However, the bug's capabilities can vary a lot. More target objects provide more possibilities to match with different capabilities, resulting in more vulnerabilities to be exploited to achieve root.



%It is very challenging to match the critical data with the correct types of bug so that the bug can exploit that data to escalate privilege.

%The significant hazards of various bugs are still in the dark, as many critical non-control data remain undiscovered. On the one hand, limited target candidates lead to privilege escalation when enforcing the protections. Previous works dig more target objects~\cite{chen2020systematic, liu2022release, wang2023alphaexp}, but many of them are not available under protections. Besides, they do not directly cause privilege escalation but instead various primitives, such as hijacking control flow, bypassing protection mechanisms, and reading/writing certain memory regions. 
%On the other hand, automatic detection tools~\cite{syzbot22:online, googlesy60:online} keep reporting vulnerabilities with various capabilities daily. Only a few vulnerabilities prove useful in privilege escalation exploits due to the challenges of aligning their capabilities with the target objects. It is necessary to provide as many target candidates as possible to understand the bug hazards for security researchers.
%
%The capabilities can vary significantly across different vulnerabilities.
%Many works aim to comprehensively capture a bug's capabilities~\cite{dai2021facilitating, lin2022grebe, zou2022syzscope,jiang2022evocatio} and match them with target objects to be corrupted~\cite{wu2018fuze,chen2020koobe}.
%
%
%Though KENALI~\cite{song2016enforcing} applies an error-code-based heuristic to identify sensitive non-control data, it only captures a subset of critical data without studying their impacts and exploitability.
%


%\jim{Systematically and automatically identifying non-control data in the Linux kernel is hard, because it fundamentally requires an understanding of the semantics of each piece of data used in the kernel.
%Unfortunately, there are tens of thousands of unique data structures and many more fields defined in the kernel, and there exists no ground truth. \textbf{A recent work that attempts to do this, song chengyu~\cite{song2016enforcing}. }
%\zhiyun{discuss what it does and limitations. My understanding is that it applies a heuristic to search for non-control data that can alter the result of security checks, which can capture only a subset and lead to a large number of non-control data to protect (while many are not exploitable)}~\cite{song2016enforcing}. 
%It applies a heuristic (error-code) to search for non-control data that can alter the result of security checks, which can capture only a subset and lead to a large number of non-control data to protect, including the non-exploitable data. }


\ziyue{This work steps forward on discovering and exploiting the critical objects that lead to PE.}
To fill the gap, this paper is the first to automatically discover unprotected critical non-control data for privilege escalation in the file system. Evaluating data criticality depends on understanding its semantics, such as the data representing user credentials and page tables. 
%
%Modeling the semantics of all data in the Linux kernel is extensively challenging, with around 30 million lines of code of version 5.15~\cite{Some515d13:online}.
%Instead of attempting to cover the entire Linux kernel, which is overly ambitious, we focus on a commonly targeted Linux kernel subsystem, file system, because of the inspiration from the Dirty COW and Dirty Pipe vulnerabilities.
%
The file system code in the kernel is well-designed with multiple layers based on the semantics in different abstraction levels. 
The file system is prone to attacks like Dirty COW and Dirty Pipe.
Because files are closely related to kernel integrity and forced with access control checks, such as read, write, and execute. The attacker can launch privilege escalation if compromising a critical non-control object in the file system. 
%To the best of our knowledge, our work is the first to analyze the exploitability of non-control data in the file system from the perspective of semantics.
%

%To realize the systematic analysis for the Linux file system, we first model the semantics of an initial set of non-control data and then combine both static and dynamic techniques to identify all non-control data in the Linux file system and validate their exploitability.
%
%Though conceptually simple, we must resolve three challenges.


%\jim{There is gap: linux kernel -> file system in linux kernel. Instead of attempting to cover the entire Linux kernel, which is overly ambitious, we decide to focus on a commonly targeted Linux kernel subsystem, i.e., file system. By modeling a minimum set of semantics in Linux kernel file system, we can then automatically derive a number of likely exploitable non-control data, with a set of novel techniques we develop. This is feasible because a core philosophy in Linux kernel is ``Everything is a file'', thus the underlying file system has a large code-base that shares similar semantics. Furthermore, the file system in the kernel is well-designed with multiple layers of abstraction. }


%Current systems protect only a small portion of them, based on known dangerous ones~\cite{samsung1, samsung2, 2017PT, tan2023ptstore}.
%
%The protected data is selected based on known attacks or manual efforts, inevitably leaving most non-control data unprotected.
%



%\jim{introduce the semantic problem}

%We systematically summarize four attack methods. 
%Discerning the criticality of non-control data is challenging because it depends on semantics, which varies widely across different objects.
%which guides the systematic summary of attack methods from the ground up, . 
% \name{} identifies the most critical non-control objects, i.e., key objects, for each method. 
% The tool automatically identifies the most critical objects across the file system by taking input as anchor objects representing the abstract elements' semantics. 




We classify critical data (FSKO) based on the basic semantics of the file system, ensuring the discovery does not miss critical types of objects. 
%
The discovery starts with a few objects, called anchor objects, that are analyzed in abstraction layers of the file system. These layers abstract away the implementation details; thereby, the objects within the layers propagate to others in different implementations. 
%
We design three propagation rules customized to align with the characteristics of FSKOs in the file system. 
% The first two propagation rules are for flag objects and reference objects, respectively. We combine the two rules as the third one to trace COW-controlling flags. 
%
We propose a new technique named \name{} using static analysis to discover FSKO automatically by combining the above methods. 
%
\name{} finds 26 critical objects whose corruption directly achieves privilege escalation, and some only require a one-bit flip.

% For example, state-based flag propagation, page cache and disk number propagation, and COW-controlling flag discovery. 
% \name{} implements the rules using a type-based method, supporting multiple structure types and fields to refine the propagated results and build broken data flow across multiple entries, similar to previous works do~\cite{lu2019does, zhang2021statically, lu2023practical}.

%\name{} classifies the critical objects into two types and traces their propagations: reference and flag. The object serves as an index to find the location in the memory and the disk is considered a reference object, i.e., the pointer and sector number. The flag object represents a specific file system state with all its possible values/states predefined as constant numbers. Considering the file system's characteristics, we introduce state-based flag propagation and reference propagation. Furthermore, \name{} discovers the controlling flag after modeling the Copy-On-Write mechanism based on the two propagations. To refine the propagated results and re-establish data flow that may be broken across multiple entries~\cite{lu2019does, zhang2021statically, lu2023practical}, we employ a type-based method that supports multiple structure types and inside fields.



%\zhiyun{we don't seem to mention that we can automatically expand from the base objects?} 
%After validating the effectiveness of identified objects by dynamic verification, 

We adopt three exploit strategies to demonstrate the exploitability after dynamically verifying FSKO's effectiveness of privilege escalation, including our new hybrid strategy.
% The strategies include directly overwriting flag objects, swapping reference objects (a generalized Dirty Cred strategy), and 
%
The new strategy enables bridge objects to be exploitable to provide page UAF primitive to indirectly corrupt FSKOs.
%
% After constructing page UAF in the hybrid strategy, we can achieve both direct flag overwrite and FSKO swapping. 
%
We utilize a static analysis to identify the bridge ones and find that 70 are exploitable for privilege escalation, which can be achieved by a one-bit flip as well.

%\ziyue{test}

%
% First of all, we employ dynamic verification to confirm whether the identified objects actually lead to privilege escalation or not. The results show that attackers can corrupt the identified objects to become root as simply as flipping a single bit. Based on the confirmed objects, we investigate their exploitability by applying three kinds of exploit strategies: a general strategy, Dirty Cred, and page-level UAF. The exploit process can significantly differ depending on the chosen strategy. \name{} is able to find the credential objects used in Dirty Cred, \code{file->f_mode} contains the permission. We can apply this strategy to other credentials, such as \code{inode->i_mode}. Identifying the critical objects is the first step to understanding the hazards of a vulnerability completely, promoting new exploit strategies to corrupt the objects and new protection mechanisms to safeguard the objects from corruption.
% The initial step in achieving a comprehensive understanding of vulnerability hazards is the identification of critical objects. This identification not only promotes the development of new exploit strategies to corrupt these objects but also encourages the creation of new protection mechanisms to safeguard them from corruption.
% Therefore, identifying the most critical for privilege escalation is the primary problem that this work aims to solve. 

%We believe new exploit strategies to corrupt the critical objects for a more comprehensive understanding in the future.
%\jim{the relationship between ours and dirty cred, and hope for more strategies}




%We conduct the static analysis.

% \jim{No mention flag or reference}
%All the identified objects have two types; one represents the \textit{metadata} of file-related objects and operations, and the other represents \textit{references} to files. A reference object serves as an index to the location in memory or on disk, i.e., pointers and sector numbers. The flag-format non-control objects represent the kernel states, where the state value signifies a specific semantic that is shared across all files. For example, \code{inode->i_mode} encodes read, write, and execution permissions for each file on the disk. If an unprivileged user adds a specific write flag to a read-only file, he/she gains the ability to write to the file. Corrupting these flag objects does not require leaking the target value because they follow a fixed format. 


%As for reference-format non-control objects, a pointer is an index to locate the corresponding memory location, while the sector number is used for disk referencing. 



% To generalize the attack with more objects exploitable to match different vulnerability capabilities, we develop a novel exploiting technique targeting page cache, called \exploit{}.
% Page cache stages the file content into memory for fast access, which provides more attack surface. We replace the \code{page} pointer to make it point to the page cache so that we can write the file content through the corrupted pointer.
% The intuitive approach relies on a read primitive provided by a vulnerability to obtain the target address of \code{page} object. \exploit{} removes this restriction, 
% only assuming a vulnerability provides a limited heap-based write only, even one-bit flipping. \exploit{} is generalized to many heap objects, making them exploitable. 


%\name{} finds 26 critical objects that directly achieve root after corruption, some of them only require a one-bit flip. And 70 objects are more difficult to exploit directly but can be exploitable using the hybrid strategy, which can be achieved by a one-bit flip as well.

We consider the 26 FSKOs and 70 bridge objects as the corruption targets.
We evaluate their exploitability using 18 real-world CVEs covering all kinds of bugs, OOB, UAF, and DF. 
%With the kernel enabling all the latest protections, w
We write 9 end-to-end exploits to corrupt the targets, which will be open source for further security research.
%using three exploit strategies to achieve privilege escalation. 
The results show that the identified objects enable these CVEs to escalate their privilege and bypass all kernel protection, including control-flow integrity, credential safeguards, and page table protection~\cite{samsung1, samsung2, appleoss24:online}.
%Among the 9 exploits, we possess an exploit of a one-day CVE-2023-5345 that has no public exploits before.


% The file content in memory called page cache is one attack target object whose basic element is a page managed by \code{page} pointer. Our general exploit strategy directly constructs a stable page-level UAF without asking the slab to free all its objects on a page. Then we spray certain objects that connect the file's page cache to fulfill the freed page. Then we can read the address of the cached page and write the malicious content to the page cache. An unprivileged user can become root once he/she is able to write a read-only file. 


%Following the exploitability assessment, this paper introduces a novel kernel defense mechanism. It protects sensitive files within the Linux kernel from malicious corruption. Our measurement shows only minimal overhead will be introduced by this new defense.




\begin{comment}
    

First, we need to model the semantic meaning of the non-critical data.
%
The semantic meaning is necessary to understand what this data is used for, which can be used to infer its exploitability. However, the semantic meaning usually depends on the actual implementation, which is hard to extract automatically.
%
Therefore, we propose to classify the non-control data into different categories and model the semantic meaning of an initial set for each category.
%
Second, we need to trace the non-control data propagation precisely and efficiently.
%
As the value-flow analysis is not scalable for kernel \cite{sui2016svf}, we leverage types to refine data propagation.
%
However, the LLVM type system used by recent works~\cite{lu2019does, zhang2019pex,zhou2022automatic} might interchange the data types with the same memory layout, which loses the original type information. 
%Furthermore, it is not designed to carry semantics, according to LLVM community~\cite{LLVM30Ty17:online}.
%
To address this problem, we propose a novel technique named TAP (Type-based Access Path), which enhances the type resolution accuracy using the LLVM metadata.
%
Third, we need to verify the exploitability of the identified non-control data to reduce the false positives.
%
To achieve this, we develop a dynamic technique that leverages execution suspension and dynamic value reset to verify the effectiveness of non-control data.


Based on the above techniques, we have implemented an automatic tool named FSTAP (\underline{F}ile \underline{S}ystem analysis using \underline{T}ype-based \underline{A}ccess), which first conducts a static analysis to identify the sensitive non-control data and then verifies their exploitability dynamically.
%
We apply FSTAP on the Linux file system and identify 50 non-control data, 23 of which are dynamically verified, and 11 can be exploited to write read-only files. 
%
Moreover, several of the identified data can be used for privilege escalation by a one-bit flip, such as \code{bio->bi_opf} and \code{iomap_dio->flags}.
%
Therefore, by proposing new techniques and developing the automatic tool, our work further advances the current state of the art of non-control data attacks in the Linux file system.
\end{comment}



%Even though non-control-data attacks have been recognized in the research community as well \cite{lin2022dirtycred, chen2005non, davi2017pt, song2016enforcing, xiao2015kernel,shen2017defeating,proskurin2020xmp}, we believe currently discovered exploitable critical non-control data is only the tip of the iceberg. Understanding this has important implications for defense. For instance, the well-known exploitable non-control data can receive targeted defense such as hardening and monitoring with an acceptable overhead\zhiyun{we should cite KNOX here and its real-time protection solution which monitors page table, cred, and possibly others. Any other solution that does targeted protection should be cited here}. For example, ``cred'' \cite{shen2017defeating, proskurin2020xmp, hua2018epti}, ``file'', ``inode'' , page table \cite{davi2017pt, shen2017defeating, proskurin2020xmp}, security-error-code-related data \cite{song2016enforcing}, and the data that subverts some security mechanisms \cite{xiao2015kernel}.
%receive targeted defense such as hardening and monitoring \cite{lin2022dirtycred, davi2017pt, song2016enforcing}.
%However, if an attacker identifies new exploitable non-control data outside of the well-known ones, such targeted defenses will fall apart. 





%In this paper, we choose a different approach. Instead of attempting to cover the entire Linux kernel, which is overly ambitious, we decide to focus on a commonly targeted Linux kernel subsystem, i.e., file system. By modeling a minimum set of semantics in Linux kernel file system, we can then automatically derive a number of likely exploitable non-control data, with a set of novel techniques we develop.
%pinpoints more non-control data in file system that can be exploited for privileged escalation.
%This is feasible because a core philosophy in Linux kernel is ``Everything is a file'', thus the underlying file system has a large code-base that shares similar semantics. Furthermore, the file system in the kernel is well-designed with multiple layers of abstraction. 
%
%We find critical data is spread over all layers of the file system, called \textbf{\textit{Dirty Everywhere in File System}}. Corrupting any critical data can lead to a privilege escalation attack, even flipping a bit of the data works.
%

%It is important to note that we focus on the non-control data in heap as opposed to those defined as global variables in this project. This is because global variables require arbitrary memory write primitives to overwrite, which are more difficult to achieve oftentimes. In contrast, heap data can be overwritten with much weaker primitives such as out-of-bound write and use-after-free write. In other words, by arranging such exploitable non-control data in heap and overwriting it with weaker primitives, attackers can directly gain privilege escalation. Overall, 50 non-control data in total are identified in our analysis, and 11 out of them, across all file system layers, are verified to be exploitable. For instance, the data \code{bio->bi_opf} and \code{iomap_dio->flags} can be exploited to write the read-only file through a single-bit flip, from 0 to 1.

% \zhiyun{Here we should give an overview of our results, e.g., number of non-control data we find, number of exploitable ones. Also some surprising example (such as the single bit flip).}

%After digging into the files inherent to Linux operating system and studying privilege escalation attacks targeting the inherent files, we conclude an attack strategy - writing a read-only file, as shown in \cref{tab:attack-primitives}. Once the attackers achieve this strategy, they can gain root permission. \jim{TODO: we only consider the flag-format non-control data, not data pointer }
%

%\jim{Rewrite this to highlight the non-control data of file content and event types}

%\zhiyun{I do not think it is necessary to go into the details of file content and event types in intro. I would not mention any of these points above.}


%We further generalize two methods to achieve the primitive: one is directly writing a file's content buffer; the other is changing a file's metadata (usually representing permission) to indirectly write its content. We leverage a static analysis to trace the propagation of content buffer and metadata and identify the critical data among the propagation. Finally, we start up a GDB script to automatically verify the data effectiveness against privilege escalation.




%\jim{rewrite the following}
In summary, the paper makes three contributions.

\begin{itemize}[leftmargin = *]

    % \item \textbf{Systematic study of exploitable data in file system.}
    % %{Non-control data identification of file system.} 
    % This work is the first to systematically study exploitable non-control data in the Linux file system by modeling its semantics and summarizing classifications.
    %
    
    
    
    \item \textbf{FSKO automatic identification.} 
    We propose the technique, \name{},
    automatically identifies critical objects in the file system. It combines the characteristics of critical data propagation in the file system's multiple layers.
    
    %We implement the rules as an automatic tool, \name{}., identifies 26 key objects.
   % We automatically identify the most critical objects . The identification involves  
    %customizing them to identify state-based flags, COW flags, and page cache propagation.
    %Its inputs are minimum objects of semantics in four strategies. \name{} traces more propagated objects and dynamically verifies their exploitability.


   
    \item \textbf{New exploit strategy.} We apply three exploit strategies on the dynamically verified objects to explore their exploitability. Our new strategy allows for identifying bridge objects to indirectly corrupt FSKOs, thereby enhancing the potential to exploit a broader range of bugs for corruption. 



    \item \textbf{Practical evaluation and findings.} 
    We write and open-source 9 end-to-end exploits based on 18 real-world CVEs of 26 FSKOs and 70 bridge objects. The identified objects enable these CVEs to bypass all kernel protections and escalate privilege.

    % \item \textbf{Practical evaluation and findings.} 
    % \name{} identifies 26 critical objects that can be used to write read-only files. Moreover, 70 objects facilitate the new strategy with page cache. We evaluate them by 18 real-world CVEs and 9 end-to-end exploits, including an exploit for a CVE-2023-5345 that has not been exploited before.

    % The exploitation in wild targeting of non-control data is relatively rare. In order to prove the practicality of real-world exploitation, we evaluate attack effectiveness and required primitives of corrupting non-control data. Moreover, we modify xx existing kernel PoC to show that the identified non-control data can make the existing attack easier.

\end{itemize}

%\ziyue{We open our tool and evaluation to public to xxx}





==> back/_3-attack_goal_category.tex <==

%\wenbo{??} % 不连贯，to systematic analysis, we need goal
% goal is priv escalation

%\ziyue{Despite various CVEs or exploits targeting the file system, uncertainty remains regarding the types of non-control objects that can facilitate privilege escalation in the complex file system, leaving potential attacks in obscurity. To address this issue, it is crucial to define the attack goal: to achieve root-level privileges.}







%The file system has to design the data structures to represent the core semantics of the file carefully. 

%The core semantics includes the composition of file objects and the operations that apply to file objects, which . 

%\subsection{Attack Goal}

%\jim{(1) the insight to abstract the semantic and categorize the known data, based on the background. (2) scope-adaptive data flow analysis,  We do not sell the TAP, which is more like a standalone work. but sell the semantic related analysis. (3) dynamically verify. not only GDB, but also the analysis of data location and exploit time window. Move the challenge into goal.}




\begin{comment}

\textbf{Problem Scope.}
The types of non-control data divide into two categories, integer/bool type, and data pointer type. The integer/bool type is often implemented as a flag field in a structure because Linux kernel designs a structure type to represent specific semantics. The \textbf{flag-format} non-control data of integer/bool type is the target this work focuses on. Although the flag can be manipulated by substituting the whole data structure, i.e., corrupting the data pointer, we do not consider it in this work. We believe it is further work.
\zhiyun{we should mention we consider heap data only as opposed to global variables (I already had something written in intro)?}


\begin{table}[t!]
\centering
\caption{The malicious operations beyond file permissions lead to privilege escalation.}
% \begin{threeparttable}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c}
\toprule[0.3pt]
\toprule[0.2pt]

 \textbf{File}  & \textbf{\makecell[c]{Permissions}} & \textbf{\makecell[c] {Malicious \\ Read}} & \textbf{\makecell[c]{Malicious \\Write}}    & \textbf{\makecell[c]{Malicious Exec \\ with Setuid}}      \\ \hline
 \code{/etc/shadow} & \code{---} &  \XSolidBrush & \CheckmarkBold & \XSolidBrush \\ \hline
 \code{/etc/sudoers} & \code{---} &  \XSolidBrush & \CheckmarkBold & \XSolidBrush \\ \hline
 \code{/etc/passwd} & \code{r--} &  \textbf{---} & \CheckmarkBold & \XSolidBrush \\ \hline
 \code{/etc/group} & \code{r--} &  \textbf{---} & \CheckmarkBold & \XSolidBrush \\ \hline
 \code{/usr/bin/passwd} & \code{r-s} &  \textbf{---} & \CheckmarkBold & \textbf{---} \\ \hline
 \code{/usr/bin/vi} & \code{r-x} &  \textbf{---} & \XSolidBrush & \CheckmarkBold \\ 
 
 % \code{/usr/bin/nano} & \code{r-x} &  \textbf{---} & \XSolidBrush & \CheckmarkBold \\

% \code{---} & \CheckmarkBold\\\code{}\\  &     \XSolidBrush        \\ \hline
% \code{r--} & \begin{tabular}[c]{@{}c@{}}\CheckmarkBold\\ \code{/etc/passwd}\\ \code{/etc/group}\end{tabular}   &     \XSolidBrush        \\ \hline
% \code{r-x} & \XSolidBrush                                             & \begin{tabular}[c]{@{}c@{}}\CheckmarkBold \\\code{/usr/bin/vi} \end{tabular}\\ \hline
% \code{r-s} & \begin{tabular}[c]{@{}c@{}}\CheckmarkBold\\\footnotesize\code{/usr/bin/passwd}\\  Arbitrary Code Execution\normalsize \end{tabular}  &      \textbf{---}  \\

% \code{/usr/bin/passwd} & \code{r-x(s)} &  \textbf{---} & \CheckmarkBold & \textbf{---} \\
\bottomrule[0.3pt]
\bottomrule[0.2pt]
\end{tabular}
}
\label{tab:attack-primitives}
\end{table}

\end{comment}



\begin{figure*}[!th]
    \centering
    \includegraphics[width=.9\textwidth]{figure/overview.pdf}
    \caption{\ziyue{Fix anchor} The work overview consists of identifying key objects and their exploitability analysis to find effective objects.}
    \label{fig:overview}
\end{figure*}







\begin{comment}
    

\PP{Non-Control ``Dirty'' CVEs}
%\jim{TODO: give more explanation and comparison at the intro and related work.}
This section examines three well-known "dirty" CVEs or exploits, all aiming to escalate privileges by writing a read-only file. Both Dirty COW and Dirty Pipe gain invalid write on the file's page cache.


{Dirty Cred} \cite{lin2022dirtycred} is an exploit strategy that replaces a low-privilege credential with a high-privilege one to bypass permission checks. In particular, the struct \code{file} is created when opening a file on disk, representing the returned \code{fd}. The attack corrupts the \code{file} pointer after checking the permission of \code{file->f_mode}. By corrupting the file pointer, Dirty Cred replaces the entire read-write \code{file} structure with a read-only \code{file} to write a read-only file. 

%Specifically, after checking \code{file->f_mode} which holds read/write permission information, Dirty Cred replaces the whole read-write file structure with a read-only file by corrupting the file pointer.


{Dirty COW} \cite{CVECVE2014:online} (CVE-2016-5195) is a race condition bug. COW (Copy-On-Write) only duplicates a resource when writing it. One thread tries to access a new-allocated page, and the other thread races to free this page. A flag signifies no need to write to the page cache when successfully freeing the page. Therefore, the kernel just maps the page cache to user space to save memory to the first thread, making a normal user write the page cache. 
%Unprivileged attackers can write the read-only file' page cache without checking. The root cause is memory subsystem mishandles the copy-on-write (COW). When an unprivileged user requires to write the private mappings created by \code{mmap}, kernel is supposed to allocate new page(s), copy the original content of page cache to the new one, and finally re-map private mappings from page cache to the new page(s). 
The race condition influences the flag that controls the acquisition of either page caches or new pages, which is summarized as the corrupting file content.



{Dirty Pipe} \cite{CVECVE2059:online} (CVE-2022-0847) is a use-before-initialization bug in pipe implementation. The Linux kernel has a syscall \code{splice} for efficient exchange data between a file and a pipe. When reading a file, \code{splice} directly assigns the page in the page cache to a pipe buffer array without new page allocation. The pipe buffer is an array to handle multiple write operations, enabling them to access the same buffer. Whether to write to a new buffer or the last one is controlled by a flag. However, the flag is not initialized before use. Therefore, the exploit controls the flag's value to write the previous buffer containing the page cache instead of the next new buffer. This exploit strategy is similar to Dirty COW, the corrupting file content.

\end{comment}


% More target objects result in more 
% for example, CVE-2023-5345 has never been exploited before but is exploitable based on the \name{} identified objects. This UAF vulnerability allows invalid writing of the page pointer allocated in the heap array at function \code{configfs_write_iter}. Attackers can achieve root to write the page cache of a read-only file using page-UAF mentioned in \cref{sec:exploit}.
%\jim{decribe the bug capability and the used target object}




\begin{comment}
    
\begin{figure}[!t]
    \centering
    \includegraphics[width=.75\linewidth]{figure/motivating-example.pdf}
    \caption{Triggering an OOB bug that has a vulnerable object to overwrite the target object.}
    \label{fig:motivating-example}
\end{figure}

\section{Motivation}
\label{sec:motivation}


The initial step in both attack and protection is the identification of critical objects.
%
An increased number of target objects makes more bugs become exploitable for attacks and spawns more protections to defend against these attacks. 
%
Specifically, matching the bug's capability with the target objects aids in a comprehensive understanding of the bug's hazards. 
Taking an OOB bug as an example shown in \cref{fig:motivating-example}, it can overwrite a specific length of bytes starting from a particular offset. 
%
To clarify the invalid write, researchers define bug capabilities for OOB~\cite{chen2020koobe} and UAF~\cite{wu2018fuze}, including which slab cache the vulnerable object is in, where memory the bug can invalidly access, and what values can be set to the memory. 
%
The capabilities differ significantly among various bugs, which requires as many targets as possible to match different capabilities. Because critical data must fall within the overwrite range as illustrated in \cref{fig:motivating-example}. The increasing target objects bring more possibilities to be overwritten by various bugs.
%
However, fewer target objects are available when increasing protections are enabled. For example, a common method is to corrupt a function pointer to hijack control flow, but this approach is no longer effective due to CFI. 
%
In contrast, corruption of unprotected data, such as \code{pipe_buffer->flags}, which could be identified by \name{}, will directly escalate privilege.


\textbf{Increasing targets broadens matched bugs.} Having more objects as corruption targets expands the range of matched bugs to launch attacks. Countless bugs are reported every day thanks to the fuzzers~\cite{syzbot22:online, googlesy60:online}. However, only a few of them are finally exploitable to privilege escalation, leaving the majority remain unexploited.
% However, few bugs are exploitable to privilege escalation attacks, and the majority remain unexploited. 
%
Because their various capabilities are poised to align with limited known targets as corruption candidates. More targets bring more possibilities to match different capabilities.
Several works aim to enlarge the targets~\cite{chen2020systematic, liu2022release, wang2023alphaexp} to construct various primitives, such as control-flow hijacking, bypassing protection mechanisms, leaking heap pointer address, and so on. However, they can not directly lead to privilege escalation, and many of them are no longer exploitable when enabling all the protection mechanisms. %\jim{mention they are not the most critical for privilege escalation but lead to many different primitives.}
%



\textbf{Protection of the well-known objects.} Attackers have fewer candidates as corruption targets when the protection mechanisms are enabled.
Control-flow integrity mechanisms are forced in the mainline Linux kernel~\cite{ClangCFI41:online}, Windows~\cite{wincfi}, XNU~\cite{cai2023demystifying, appleoss24:online}, and Android~\cite{androidcfi}, making hijacking control flow increasingly difficult. Moreover, commercial kernels safeguard the non-control objects that are often used to achieve root privilege in real-world exploits, such as \code{cred}~\cite{samsung1, samsung2, appleoss24:online}, global variable \code{modprobe_path}~\cite{li2023hybrid}, and page table~\cite{samsung1, samsung2, appleoss24:online}. The well-used \code{msg_msg} is no longer available on Android devices~\cite{blackhat2023}.
%
Dirty Cred~\cite{lin2022dirtycred} proposes a protection mechanism for the credential objects, \code{file} and \code{cred}. 
% Dirty Cred~\cite{lin2022dirtycred} points out that \code{file} and \code{cred} contain credential information, and proposes a protection mechanism to protect them. 


\jim{
It is worth noting that we only focus on the discovery and exploitability of critical objects.
Automatic matching bug's capabilities with targeted objects is out of this paper's scope, since it is already a challenging problem. Researchers propose many methods solely for automatic matching~\cite{wu2018fuze,chen2020koobe, dai2021facilitating, lin2022grebe, zou2022syzscope,jiang2022evocatio}. 
Furthermore, our exploitability analysis consists of manually written end-to-end exploits.
The reason is that automatic exploit generation could be very challenging, and there is no fully automatic method. 
For example, to demonstrate the exploitability of proposed attack strategies, many researchers manually write exploits to make more bugs exploitable based on the known target objects~\cite{wu2019kepler, zeng2022playing, lin2022dirtycred, liu2022release}. 
%Nevertheless, the target objects are too limited to generalize the strategies for a broader range of bugs, and many remain unexploitable. 
}
\end{comment}



%Specifically, we adopt three exploit strategies to demonstrate practicality for the objects shown in \cref{fig:overview}.

%In summary, identifying the critical objects is the first step in exploring the bug hazards. The more critical objects are identified, the more significant potential for exploitation is exposed with various attack strategies. Besides, the discovery of new critical objects may lead to innovative strategies for easier exploitation. Therefore, this paper aims to identify new critical objects that escalate unprivileged users to root as long as they are corrupted. We evaluate them using existing attack strategies to demonstrate their practicality, and we anticipate that future development of new strategies will render more objects exploitable.
%identification and strategy. the relationship between DirtyCred and the other strategy







\begin{comment}
    

\section{Attack Goal}

The goal is to achieve local privilege escalation by corrupting objects in the file system of the Linux kernel.
Although several prominent exploits target objects in the file system, the entire landscape of exploitable file system objects is largely unknown.
%represent little remains regarding the types of non-control objects that can facilitate privilege escalation in the complex file system.
%Defining the attack goal of the file system is a crucial first step and forms the foundation of the systematic analysis. As long as the attacker attains this goal, he/she becomes root. 

To map out the landscape of exploitable objects, we first need to understand the semantics of key functionalities that pertain to privileges in the file system. 
As mentioned, previous exploits have corrupted sensitive file content not accessible to regular users (e.g., \code{/etc/shadow}).
%For example, \code{/etc/passwd} contains the registered users for the system and is read-only to non-root users.
%Therefore, we term these files as \textbf{\textit{sensitive files}}.
%
% To be more complete, we list five representative sensitive files in the Linux system that are worth targeting \cref{tab:attack-primitives}.
%Note that we only present a part of the files in the Linux kernel.
%\ziyue{why these files}. 
In addition, we show in the columns to describe which permissions (if gained by the attacker) can effectively achieve privilege escalation. They are read, write, and execution with setuid \zhiyun{should this be setuid root?}. 
%If the attacker can achieve root after obtaining one malicious operation, there will be a \CheckmarkBold; otherwise, \XSolidBrush. 
%\ziyue{can be more concise, polish required}
%Because when attackers obtain an invalid reading or execution, there is no inherent file that can be exploited for privilege escalation on a pure Linux system.

%Unfortunately, these sensitive files are also attackers' favorite targets.
%
As shown in the table, if attackers write the first five sensitive files successfully, they can achieve privilege escalation.
%
For example, a normal user uses Dirty COW vulnerability to overwrite the \code{/etc/passwd} to add herself/himself as root. \zhiyun{is it the /etc/suders file for adding a user to root? can you double check?} \jim{this can enable a user to execute sudo}
%
Furthermore, he/she can escalate to root by gaining setuid flag of the executable file \code{/usr/bin/vi}. 
%\ziyue{\code{/usr/bin/vi} and \code{/usr/bin/vi} duplication???}, and their owners are root. 
It works because we can execute them with setuid to edit a read-only sensitive file mentioned before.

Although writing any sensitive file lead to privilege escalation, files with read permission are preferred. Because many syscall calls can only be triggered with an opened file description, such as splice, mmap, and so on. The files without read permission cannot be opened at the beginning, reducing the exploit space. Note that the permission is part of the metadata, which can be corrupted to indirectly write the file content. Therefore, we set our goal as ``\textbf{writing the content of a read-only file}" both directly and indirectly.
\end{comment}


%\jim{I wrote it with reference to xinyu xing's paper. "We assume there is a PoC which triggers the vulnerability and leads to a control-flow hijacking primitive (CFHP). We assume the CFHP is already identified with the PoC through either manual analysis or dynamic analysis such as symbolic tracing, thus finding exploit primitives is orthogonal to our work and we can focus on evaluating the CFHP. We assume a restricted memory leak primitive to help infer coarse kernel memory layout (e.g., getting the base address of code section .text and physmap region). We do not assume the existence of an arbitrary memory write primitive which could write to arbitrary kernel memory address. We do not assume the existence of an arbitrary memory leak primitive that can dump arbitrary kernel memory content." Usenix Sec'19 Kepler: Facilitating Control-flow Hijacking Primitive Evaluation for Linux Kernel Vulnerabilities}



%Even worse, in our analysis, we find that Linux file systems often rely on non-control data (such as flags) to control the read/write operation of all files, including sensitive ones, which gives the attacker chances to alter the read/write operation of sensitive files by corrupting the non-control data.
%
%Therefore, in this paper, we conduct a systematic analysis to identify all non-control data that control read/write operation.


%The types of non-control data divide into two categories, integer/bool type, and data pointer type. The integer/bool type is often implemented as a flag field in a structure as the Linux kernel designs a structure type to represent specific semantics. The \textit{flag-format} non-control data of integer/bool type is the target this work focuses on. Although the flag can be manipulated by substituting the data pointer, this paper focuses more on the exploitability of the flag-format control data, leaving the data pointers to future work.



%The abstract objects that can be attacked in the file system when considering the realization.





\section{Scope and Assumptions}
\label{sec:threat-model}

%\ziyue{Add a section for Linux file system's background}

% We perform static analysis to collect all of the target objects.
%We  collect all of them as target objects.
%A straightforward strategy is a direct corruption of the key object. Moreover, we can swap the 



\subsection{Threat Model}
% \textit{Available Exploit Primitives to Attackers.}
We assume an unprivileged user aims to achieve local privilege escalation by exploiting a memory error in the kernel. 
Specifically, the error allows limited memory writes (e.g., OOB write or UAF write), possibly as limited as a single-bit write.
%writes a PoC to trigger a vulnerability for limited memory writes, even one single bit. 
%He/she achieves root privilege by leveraging this
%limited memory write without modifying the control flow.
We \textit{\textbf{do not}} assume the availability of arbitrary memory write primitives, i.e., write anywhere in memory. 
%
%In most cases, we do not require information leaks to obtain the target values of the critical objects. There are two kinds of objects that do not rely on the leakage. 
%First, a normal user achieves root if the objects are set with certain values, which can be analyzed from the source code in advance. These objects are the flag objects in~\cref{sec:FSKO-identification}.
%
%The second type is the object whose value has a specific format. Based on the special format, we only need to change the last several bits, even flip one bit. For example, the structure \code{page} manages a 4KB physical page, and its size is 0x40. By flipping from 0 to 1 at 0x40 bit, a \code{page} pointer will point to another \code{page}, which helps to construct a page UAF to achieve root. These are the extra target objects used in hybrid exploit strategy~\cref{sec:hybrid-strategy}.
%The leak only happens when corrupting the disk references with leaked target sector or block numbers.


% \textit{Enforced Mitigation.} 
We assume the Linux kernel enables all modern mitigations, including CFI~\cite{linuxaddcfi:online, x86Addsu43:online}, W$\oplus$X~\cite{Extendin37:online}, KASLR~\cite{Kernelad62:online}, SMAP/SMEP (x86)~\cite{Supervis7:online, Thestatu39:online, kernelor87:online},  PAN/PXN (ARM)~\cite{kernelor87:online}, and KPTI~\cite{Thecurre17:online}. An unprivileged user cannot modify kernel code or inject code into the kernel data segment, and the kernel address is randomized. The kernel is restricted from accessing the data or executing the code in user space. Control flow can not be hijacked. Besides, the well-known non-control data are safeguarded as well, such as \code{cred} and page tables.


\subsection{Problem Scope}

This work focuses on discovering unknown and critical non-control data that are not currently protected and can be exploited in practice.
%
We believe the problem is meaningful and non-trivial.
%
This is because there is no systematic approach for identifying non-control objects for privilege escalation. The identification is inherently challenging, distinguishing it from previous endeavors in object identification.
%
Previous works have proposed to find more objects to facilitate kernel exploitation to achieve various primitives~\cite{chen2019slake,chen2020systematic,liu2022release, wang2023alphaexp}. 
%
Among them, SLAKE~\cite{chen2019slake}, akin to our work, concentrates on the automated discovery of objects containing function pointers that can be exploited to achieve control flow hijacking in the Linux kernel. As Control Flow Integrity (CFI) is widely enforced, attackers turn to non-control data.
%
However, critical non-control data lacks explicit patterns like control data, making identification challenging. 

% No previous work has identified the critical non-control data exploitable for privilege escalation attacks, motivating our work. 



\PP{Attack Goal} 
Our goal is to achieve privilege escalation by corrupting critical non-control objects in the file subsystem of the Linux kernel. 
%
Clarifying the goal facilitates the discovery of the critical objects by analyzing whether they can lead to the goal.  
%
Corrupting critical objects provides attackers with malicious operations on sensitive files that are not allowed. 
There are two kinds of malicious operations on sensitive files after studying.
First, previous exploits~\cite{Arinerro42:online, DirtyCOW66:online, lin2022dirtycred} maliciously write read-only files. 
These files' owner is root, and they should not be written by normal users, e.g., \code{/etc/passwd}). 
%
Second, corrupting permission attributes to execute a file as root privilege, resulting in privilege escalation~\cite{Privileg73:online}. 
One method is to obtain extra setuid of a root's file, such as \code{/usr/bin/vi} to edit the root user's file \code{/etc/shadow}, and \code{find} allows us to execute a command \code{/bin/sh} using root privilege, i.e., arbitrary code execution as root. Another method is that a normal user creates many files with setuid, and maliciously corrupts a file's owner to root.
%
After discovering critical objects that can lead to attack goals, we will discuss how to corrupt these objects using three kinds of strategies in~\cref{sec:exploit-strategy-integration}, including our new hybrid strategy.
%\zhiyun{Are these exploit strategies also described in section 6.2? It feels like these two places both talk about exploit strategies but do not reference each other. Not clear whether they have any relationship.}

% preview: how to write using different strategies in sec 6.


% In summary, attackers can achieve privilege escalation if they successfully obtain malicious operations on sensitive files that are not allowed. 





\PP{Overview} 
% we show this work's overview. As shown in \cref{fig:overview}, 
Our work aims to discover the critical non-control data used to achieve malicious file operations to escalate privilege, consisting of two major parts, as shown in \cref{fig:overview}. 
%
We leverage static analysis to identify the FSKOs automatically in~\cref{sec:FSKO-identification}. 
%
% The identification begins with identifying anchor objects embodying the semantics of the file system.
% %
% Then, we design the propagation rules to discover the propagated objects that may affect or be affected by the anchor objects.
%
After dynamically verifying the identified objects lead to privilege escalation, we apply three exploit strategies to corrupt FSKOs~\cref{sec:exploit-analysis}, including our new strategy in~\cref{sec:hybrid-strategy}. 
%
% To enhance the generality of FSKOs across more vulnerabilities with diverse capabilities, we propose a hybrid exploit strategy that introduces extra target objects as corruption targets. We can tamper FSKOs indirectly after exploiting the vulnerability to corrupt the extra targets in~\cref{sec:hybrid-strategy}. 






%The work is proposed to achieve the attack goal, and 
%


\begin{comment}
The identification requires classifying the key (the most critical) objects based on the file system semantics. We select an anchor object for each type that serves as the propagation root.
%
Finally, we design the propagation rules specifically for the file system to discover more key objects.
%
The second part is the exploitability analysis of the identified objects through three exploit strategies. All strategies are applied to the validated objects after dynamical verification. The strategy can broaden the set of target objects to offer possibilities to match bugs with various capabilities, making more bugs exploitable. Attackers can corrupt these objects to achieve certain primitives to corrupt the key objects indirectly.   
\end{comment}



%\wenbo{4 is too details, 5 is not enough}


%by involving others to influence the key objects, beside another existing strategy~(\cref{sec:swapping-strategy}).

% %
% For example, a normal user uses Dirty COW vulnerability to overwrite the \code{/etc/passwd} to add herself/himself as root. \zhiyun{is it the /etc/suders file for adding a user to root? can you double check?} \jim{this can enable a user to execute sudo}
%
% However, the files with read-only permission are preferred (e.g., \code{/etc/passwd} is used in the three Dirty CVEs). Because many syscalls can only be triggered with an opened file description, such as splice, mmap, and so on. The files without read permission cannot be opened at the beginning, reducing the exploit space.
% %
% In summary, we aim at finding the key exploitable objects that enable an unprivileged user to \textbf{\textit{write a read-only file}} upon their corruption.










\section{FSKO Identification}
\label{sec:FSKO-identification}


This section presents the automatic identification of the FSKOs with file system semantics. 
%
In this paper, we term the most critical data in the file system as \textbf{\textit{FSKO}} (\underline{F}ile \underline{S}ystem \underline{K}ey \underline{O}bject): their corruption enables an unprivileged user to achieve root. 
%
Automatically identifying FSKOs poses significant challenges.
\textbf{\textit{C1}}: How can we autonomously uncover FSKOs across all layers, encompassing diverse file system implementations and disk drivers, while covering all types of FSKOs?
% What types of non-control data are critical, and how are these types classified to avoid missing critical ones? 
%
\textbf{\textit{C2}}: Are there any propagation rules between two FSKOs to help discover as many critical objects as possible?


We propose a new technique \name{} to solve the challenges.
%
% The identification should cover various types of FSKOs systematically and
% Our analysis aims to be compatible with different implementations and drivers.
\textbf{\textit{S1}}: \name{} starts with the anchor objects embodying the semantics of each kind of FSKO. They reside in the abstraction layer, hiding the details of various implementations.
%
% The classification comes from the abstract semantics of the file system in design, ensuring that it does not miss any targets. Corrupting the classified FSKOs achieves malicious operations on sensitive files. 
%
\textbf{\textit{S2}}: We design propagation rules to discover the propagated objects that may affect or be affected by the anchor objects in the specific implementations, combining the characteristics of the file system. 


%The rules model the characteristics of the file system and memory management. 
%
%
% We propose a static-analysis technique in accordance with the characteristics of the file system, \name{}. 




\PP{Data Semantics Representation}
%Considering the implementations, the kernel code must design specific type structures to represent the three elements. We term the instance of a particular type structure and inside field as \textbf{object}.
The well-designed data structures inherently encapsulate specific semantics. Therefore, we term the instance of a particular structure type and inside field as an \textbf{\textit{object}}. For example, rwx permissions are stored as a field inside a structure in the virtual file system layer, \code{inode->i_mode}, where each \code{inode} one-to-one manages a file on disk.





%It uses a type-based method to rebuild the broken data flow due to multiple entries. 

%The actual implementations bring restrictions. After considering them, we summarize four types of key objects.





% 解释为什么要做 FSKO classification。因为我们要找出 permission 相关的 non-control data







%
% Since normal users can validly read a sensitive read-only file, they can achieve root by corrupting the operation from read to write after checking the permission. Because the lower layers of the file system use the same functions for both read and write. 







% The file system has a well-designed structure, and we abstract it into two layers for better understanding: a virtual file system (VFS) and a physical file system (PFS). VFS collects and organizes the data for user-space access, making it compatible with different implementations.
% VFS introduces represent the three abstract elements. Specifically, it maintains a cache for content (known as page cache) and metadata. Page cache stages the file content into memory for quick access, with different file system implementations utilizing their own read or write functions. However, different implementations eventually call the same generic read/write functions to operate the page cache.  After mapping the elements from VFS to the PFS, both file metadata and content are translated to their corresponding sector number ID on disk. Importantly, the lower layer does not distinguish between file metadata and content and only concentrates on data exchange between memory and disk.







% In concept, we can corrupt three basic abstract (metadata, content and operation) objects to achieve malicious writing on a file. As discussed in \cref{sec:multi-layer-file-sysem}, 
% \wenbo{terms in 2.1 should be highlighted.}
% the user, acting as the subject, can perform different operations on the file object. The permission is part of the metadata, and corrupting it causes indirectly manipulating the file content. The user-triggered operation can be indirectly inverted from read to write to corrupt file content. 
% Of course, we can also directly corrupt the objects representing the file content. 


%Therefore, we set our goal as ``\textbf{writing the content of a read-only file}" both directly and indirectly.

%\guoren{Note that a file execution requires reading the file first. Specifically, the memory page containing file content is marked with an execution bit after reading from the disk. The CPU executes instructions on the page accordingly.}

% Note that file execution eventually translates to a file read that passes down through the file system. The memory page that holds file content is marked with an execution bit after reading from the disk. The CPU executes instructions on the page accordingly.



%In particular, the kernel retains the file content in memory for extended periods to facilitate rapid access, thereby reducing interactions with the disk. 


%In summary, we identify the objects is to corrupt the internal field instead of the whole structure.

% The metadata and content are cached into the memory from the disk for rapid access,
% Theoretically, we can corrupt the in-memory objects (page) and on-disk counterparts (sector). Besides, it is possible to invert a legal read operation into a malicious write operation during synchronization for both metadata and content. 
%Because lower layers in the file system primarily handle data exchange between memory and disk. 
% The difference between reading and writing lies in the direction of data exchange, which can be reversed.
%Reversing a read operation into a malicious write operation during synchronization applies the metadata and content in theory. Because they both the synchronization between memory and disk. 
%\ziyue{\sout{for both metadata and content}}.
%\guoren{not understand this sentence.}
% We can corrupt the metadata in memory because it is cached for a while. However, corrupting the metadata on the disk is hard to achieve, and more details in \cref{sec:write-disk}.




%In this section, we summarize four possible attacks on the file system to write a read-only file. The categorization is rooted in the two fundamental components of the file system: the file object (metadata and content) and the operations applied to the object.
%As discussed at \cref{sec:file-in-linux}, a file object further comprises, leading to various attack categories. 

%Finally, we discuss the high-level objects that contain multiple fundamental elements, leading to privilege escalation, as Dirty Cred does \cite{lin2022dirtycred}.






\begin{comment}
    

\subsection{Concrete Attack Method}

When the file system realizes the concept of the abstract objects, there will be four possible attack strategies to achieve root in \cref{fig:attack-elements}. 
\wenbo{why four?}
Two strategies are not unrealistic because of the realization, and we discuss the reasons at the beginning of the section. We introduce the details of each strategy using \cref{fig:attack-category}. 

\subsubsection{The Reason for Method Selection}
There are two ways to access the file content for read or write requests, as shown in \cref{fig:attack-elements}. 
\wenbo{why file contents}
(1) \textit{Buffered I/O}: This method involves accessing the file content stored in the page cache. If the file is not cached, the kernel will traverse the file system layers to retrieve the content from the disk. Afterward, the kernel builds its page cache for the subsequent accesses, following the Least-Recent-Used (LRU) principle. (2) \textit{Direct I/O}: kernel directly passes I/O request to the concrete file system implementation to compute the disk sector, and then it forwards the request to lower layers. 
%Optimizations and rescheduling of I/O requests happen in the generic block layer before 
The drivers finally send commands containing sector numbers to the hard disk to perform the data exchange.


Corrupting metadata (1) by substituting the sector number to corrupt it on disk and (2) by reversing read/write operations is both challenging and unnecessary for multiple reasons. (1) These two attack methods both occur at the lower layers, where the kernel does not differentiate metadata and content.
The metadata and content share the same data exchange interface and data structures when synchronizing between memory (page) and disk (sector), as illustrated in \cref{fig:attack-elements}. Therefore, there is no difference when applying the two methods to the file content and metadata because of the same object's corruption. However, corrupting file content is much easier to achieve for the following two reasons. 
%
(2) The implementation does not support the exchange between metadata on disk and a fully user-controllable metadata buffer. On the contrary, the user buffer for read/write file content is totally controlled by the user. (3) Kernel implements to synchronize multiple metadata in a page with the disk at once, leading to overwriting other unintended metadata of other files. However, file content is stored at page granularity in the page cache and block granularity when synchronizing to disk.

\end{comment}





% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figure/AttackCategory.pdf}
%     \caption{The attacks on four types of key objects achieve privilege escalation by writing to a read-only file.}
%     \label{fig:attack-category}
% \end{figure}


% \subsection{Anchor Object Selection} 
% \label{sec:Four-Attack-Methods}



%Converting the operation results in an inconsistency between the memory and disk, which can be solved by freeing the page cache and rebuilding it from the disk as before.
%\ziyue{polish requied}


%If we only change the content on the disk and keep the page cache untouched (C and D), there will be inconsistency between the memory and disk. We use \code{fadvise} to drop the page cache and buffered I/O to construct its page cache by reading data from the disk. \zhiyun{this paragraph seems to come out of the blue. need more context (refer to an earlier section?) How can we change the content on the disk without changing the page cache?} \jim{It is previously placed at implementation. Now I put it here.}

% struct A {
% page * f;
% }
% page ** stack = kmalloc\_array(); 

%\ziyue{This Dirty Cred seems abrupt}

%The read-write \code{file} with a read-only \code{file} after checking the permission in \code{file->f_mode}. The structure \code{file} is created after opening a file on disk successfully, which holds file metadata (\code{file->f_mode}) and file content (\code{file->i_mapping} and \code{file->f_inode->i_mapping}) both. Corrupting either metadata or content results in privilege escalation; however, replacing the whole \code{file} has to wait for metadata to complete its role, specifically, checking permission. To identify higher-level data structures, like \code{file}, encompassing various types of basic elements, we must first identify the data structures representing basic elements, including the file's metadata, content, and operation.


% \begin{figure}[t]

% % \begin{minted}[highlightlines={3,12}]{c} 
% % struct bio {
% %   ...
% %   unsigned int    bi_opf;	
% %   ...
% % }

% % #define bio_op(bio) \
% %   ((bio)->bi_opf & REQ_OP_MASK)

% % blk_qc_t submit_bio(struct bio *bio) {
% %   ...
% %   if (op_is_write(bio_op(bio))) {
% %     count_vm_events(PGPGOUT, count);
% %   } else {
% %     task_io_account_read(bio->bi_iter.bi_size);
% %     count_vm_events(PGPGIN, count);
% %   }
% %   ...
% % }
% % \end{minted}
% \centering
% \includegraphics[width=0.85\linewidth]{figure/bio_opf.pdf}
% \caption{\code{bio->bi_opf} controls the read/write direction.}
% \label{fig:example-read-write}
% \end{figure}

==> back/_4_design.tex.tex <==
\subsection{Anchor Object Discovery}
\label{sec:anchor-object}

%We consider two criterion in searching for \textit{\textbf{anchor objects}}. First, we need to abstract layers

%To be compatible with different implementations to find a complete list of FSKOs, our analysis starts with anchor objects in the abstraction layers.


We define \textit{\textbf{anchor objects}} to be FSKOs that (1) hold the semantic that has security implications (specifically three classes of semantics), and (2) reside in the abstract layer, making it more manageable to analyze, compatible with different implementations.






% These anchors serve as the root to discover the propagated FSKOs.

%\jim{heuristic and automatic analysis}



%\subsubsection{FSKO Classification}
%\label{sec:classification}

\begin{figure}[!t]
    \centering
    \includegraphics[width=.8\linewidth]{figure/concept.pdf}
    \caption{File system functionality in the abstract.}
    \label{fig:concept}
\end{figure}

%
\PP{Classes of Semantics.}
%We should consider the file system in design to ensure we find as many FSKOs as possible.
%
We start by laying out the basic design elements of file systems.
In general,
a file consists of two parts: \emph{file content} that stores the actual data; \emph{file metadata} that encompasses properties like creation time, name, ownership, and permission. 
We focus on the metadata related to access control policy (i.e., ownership and permission) because they directly influence the possibility of privilege escalation.
Furthermore, there are \emph{operations} performed over files, e.g., read, write, and execute. 
Naturally, they correspond to the three classes of semantics that matter to privilege escalation. We illustrate them in~\cref{fig:concept}.
%The these three types of objects can be beneficial

\textit{(1) Metadata}:
Unprivileged users can corrupt permission or ownership objects to obtain authorization over files that are not owned by the attacker.
For example, an attacker can weaken the permission or change the ownership so that a sensitive read-only file is writable by the attacker~\cite{Arinerro42:online}.
They can also create a new file with malicious payload and turn it into a setuid root executable which will execute as root~\cite{Privileg73:online}.

\textit{(2) Content}: Corrupting content of sensitive files can obviously lead to privilege escalation, e.g., \code{/etc/passwd}. In terms of heap objects, we know that file content can be represented as caches in memory~\cite{DirtyCOW66:online}, for buffered I/O. 
In the case of direct I/O, the write will occur directly on the hard drive.
%making it difficult to overwrite in memory. 

%In modern file systems (shown in~\cref{fig:concept})  supposed to be safeguarded by permission checks, which should not be changed maliciously. If unprivileged users manage to write malicious content to sensitive files, they can escalate to root, e.g., \code{/etc/passwd}.

\textit{(3) Operation:} An attacker can corrupt a file operation (represented by some heap object) from a read or an execute into a write, resulting in the corruption of file content indirectly (we have not seen any instance of similar strategies used in practice).%\zhiyun{any citation?} \jim{No previous works. We find corrupting read/write can achieve root.} 
This requires the attacker to have read or execute access already but not the write access.
Note that these operations are performed only after successful permission checks. This means that an attacker cannot prematurely corrupt the operation and has to wait until the permission check is passed~\cite{lin2022dirtycred}.

%Reading and writing operations span the entirety of the file system, which are considered not limited to read/write permissions but the broader context from the perspective of the entire file system.
%On the contrary, execution eventually evolves into reading the file from the disk. It solely marks the memory of file content as executable after loading (reading) the file content.



\cut{
\PP{Buffered I/O and Direct I/O}
Linux supports two file content access methods, as shown in \cref{fig:concept}. Files are cached in memory for better performance because communicating with the disk consumes a lot of time, called page cache. \textit{\textbf{Buffered I/O}}, used by default for all files, accesses the file content through the page cache.
%
The page cache undergoes periodic synchronization with the disk to maintain consistency. Throughout this synchronization, the kernel restructures the data layout in memory to align with the layout on the disk, as illustrated in \cref{fig:concept}. 
%
In addition, a user buffer can directly read/write to file content on disk, bypassing page cache, called \textit{\textbf{Direct I/O}}. Direct read and write can be achieved through an opened file descriptor with \code{O_DIRECT}.
}
%


\PP{Abstract file system layers.}
The Linux file subsystem is designed to be layered, much like any complex system. 
%
There are four layers from the top to the bottom: virtual file system (VFS), file system implementations, generic block, and drivers.
%
Specifically, we consider two well-known \textbf{\textit{abstract FS layers}} in the Linux kernel: the \textit{\textbf{VFS layer}} and the \textit{\textbf{generic block layer}}. The former sits immediately below the syscall interface, e.g., invoked by \code{open}, \code{read}, and \code{write}.
The latter sits below the layer of file system implementations that calculate file location on disk, so it connects the memory page and the disk sector. Both layers are agnostic to different underlying file system implementations (e.g., ext2, ext4) and various disk drivers.
% \zhiyun{wrong description. need fixes.}

We choose abstract layers as opposed to the concrete file system implementation layers because of the smaller and more manageable scope. It is also because sensitive FSKOs must already be defined in the abstract layers. Furthermore, such FSKOs may be propagated into various concrete file system implementation layers, which we will capture automatically through static analysis.
%which to ensure compatibility with diverse implementations, which are highlighted in blue in \cref{fig:file-system}. 
%In summary, \name{} identifies the anchor objects for each type after classification, combining the well-designed multiple layers of the file system structure.




\cut{
\subsubsection{Abstract Layer Identification} 



% \jim{abstract object.
% step1 2 3 4
% }


Even though we target VFS and generic block layer as the scope of anchor objects discovery, we still need to determine exactly what data structures and functions fall under the two layers.
We propose to define an abstraction layer as a set of commonly called functions by comparing the call graphs of different implementations.
%
The call graphs start from the read/write syscalls, go down to different file system implementations, and end with various disk drivers. 
%
To compare call graphs of different implementations, the call graph is built per file system implementation and per driver.
%
After analyzing call graphs, we find the commonly used functions in abstraction layers.
%
\jim{motivation, why we complete}


Specifically, we use \code{sys_read} as an example to find the commonly called functions of \textbf{\textit{VFS}}. The registered function pointers, such as \code{ext4_file_read_iter} and \code{ext2_file_read_iter}, call the same function \code{generic_file_read_iter}. The function continues to call \code{generic_file_buffered_read} to copy the page content loading from a tree \code{filp->f_mapping} to the user buffer. 
%
For the common functions of the \textbf{\textit{generic block layer}}, some file system implementations use \code{iomap_dio_rw}, including ext4, XFS, BtrFS, while others use \code{blockdev_direct_IO}, including ext2, FAT, exFAT. Both functions call \code{submit_bio} to deliver the read/write operations to specific drivers for disk synchronization. 
%We consider the tree as an anchor.
}





\PP{Object Identification}
To identify objects relating to the three classes of semantics described earlier, we first identify the syscalls that can potentially affect the corresponding semantics (e.g., \code{open()} relates to metadata). We then review the functions involved in the syscalls that fall under the two abstract layers. For a specific class of semantic, we also follow certain heuristics to help us narrow down the search scope.
%Drawing from the data semantics and implementation characteristics, we analyze the abstract objects within the abstraction layer. We will delve into the specifics of distinct characteristics and analyses for three types of objects.


%For example, all operating systems should design an object as the unique identifier to represent a file on disk for organization, \code{inode} in Linux kernel~\cite{Overview51:online} and \code{vnode} in FreeBSD~\cite{BasicVfs98:online}. These two are both in the VFS (virtual file system) abstraction level that is compatible with all file system implementations, e.g., EXT4, EXT2, etc. Locating the file's metadata and content through the object helps discover FSKO from the root.



\begin{figure}[!t]
    \centering

%\begin{subfigure}{.475\textwidth}
	\begin{minted}[highlightlines={6,15},samepage]{c}
static int acl_permission_check(struct inode *inode, int mask) {
	unsigned int mode = inode->i_mode;
	if (likely(uid_eq(current_fsuid(), inode->i_uid))) {
		mask &= 7;
		mode >>= 6;
		return (mask & ~mode) ? -EACCES : 0;
	}
 ...
}

int generic_permission(struct inode *inode, int mask) {
    int ret;
    ret = acl_permission_check(inode, mask);
    ...
    mask &= MAY_READ | MAY_WRITE | MAY_EXEC;
}
\end{minted}
\caption{DAC permission check validates the user-intended permission using defined macro (v5.15).}
\label{fig:macro_example}
\end{figure}



%\jim{reference, one object name}
\textit{(1) Metadata}:
%\zhiyun{Jinmeng, current description covers only permission metadata. can you add the descrption for ownership metadata as well?}
%\jim{(1) Can we directly use Chengyu Song's paper (kenali) to find the object for access control? The problem is that Kenali is not well implemented. We add a logic to dump only a few structures. (2) owner is well known using type \code{uid_t}, maybe we can use it as a domain knowledge}
We rely on well-defined keywords and macros that identify the permission objects in the VFS layer.
Specifically, we grep variable names and fields with ``uid'' and ``gid'' that identify \code{inode->i_uid} and \code{inode->i_gid}
as the user ID and group ID of the owner of the file.
Regarding permission objects, we reuse macros from a previous work aiming to identify permission-check-related kernel functions~\cite{zhou2022automatic}. 
We limit our scope to macros related to discretionary access control (DAC) (e.g., no SeLinux policy considered).
We include the three key macros: \code{MAY_EXEC}, \code{MAY_READ}, and \code{MAY_WRITE}, as well as \code{S_ISUID} and \code{S_ISGID} representing setuid and setgid permissions.
From these macros, we then statically track what variables are ``tainted'' by them using a simple data flow analysis.
The \code{mask} variable in line 15 in \cref{fig:macro_example} illustrates an example variable identified this way.
We additionally track what variables are involved in bitwise operations with the previously identified variables.
The \code{mode} variable in line 6 corresponds to this
All the objects that contain such variables are then recorded as anchor objects, e.g., \code{inode}, whose \code{i_mode} field corresponds to the \code{mode} local variable.


\cut{
which are used to check if the user request is valid. 
Specifically, the objects are an operand in the AND operation with another macro-related operand, and the AND result is in a conditional branch to determine if the request is valid. 
For example, \cref{fig:macro_example} shows a macro-related \code{mask} the macros at line 15, representing the user request.
% As the example shown in~, the parameter \code{mask} is in and logical expression (\&) with the three macros (\code{MAY_EXEC}, \code{MAY_READ}, \code{MAY_WRITE}), which represent the user intended permission. 
The value of \code{inode->i_mode} validates the user request at line 6.  so \name{} identifies it as an abstract object residing within the VFS layer and having one-to-one mapping with a file on disk~\cite{Overview51:online}. 

The macros used in this paper follow a previous work on identifying the permission-check functions using defined macros~\cite{zhou2022automatic}) while we only focus on discretionary access control (DAC). The reason is that, by default, the file system enforces the DAC~\cite{qiu1985trusted,national1987guide}. DAC restricts read, write, and execute (rwx) access to a file based on its owner identity (uid) or group (gid). The file supports attaching additional rwx access control lists (POSIX ACL)~\cite{Document54:online}.
%
The macros for user request (\code{MAY_EXEC}, \code{MAY_READ}, \code{MAY_WRITE}~\cite{zhou2022automatic}). Besides rwx, we select extra macros representing setuid and setgid permissions (\code{S_ISUID} and \code{S_ISGID}).
}


%The permission is stored as a part of file metadata in the file system. For example, the read, write, and execution (rwx) permissions are encoded into the metadata to enforce access control. 
% We describe the insights of permission metadata in implementation.
% The file system enforces the discretionary access control (DAC) by default~\cite{qiu1985trusted,national1987guide}. DAC restricts read, write, and execute (rwx) access to a file based on its owner identity (uid) or group (gid). The file supports attaching additional rwx access control lists (POSIX ACL)~\cite{Document54:online}.
% %
% We observe that the access control checks are implemented as well-defined macros. For example, the macros for user-intended request (\code{MAY_EXEC}, \code{MAY_READ}, \code{MAY_WRITE}~\cite{zhou2022automatic}), the ones representing a file's setuid and setgid permissions (\code{S_ISUID} and \code{S_ISGID}).





%\code{inode} is designed to manage and represent a file one-to-one. For example, \code{inode->i_mode} encodes the read, write, and execution (rwx) permissions for each file. 

%such as \code{inode->i_mode}, \code{file->f_mode}. 
%\guoren{Unprivileged users can indirectly obtain the write permission of a read-only file by corrupting the in-memory metadata.}
%Unprivileged users can indirectly write the content of a read-only file by writing the in-memory metadata to obtain write permission.


% \noindent \textit{B. Page Cache.} 


%(1) We select \code{inode->i_mode} in the VFS layer for permission, shown in \cref{fig:file-system} because it manages all files on the disk regardless of the type of file system (e.g., EXT4, EXT2, etc.). (2) Every file has its own dedicated page cache, pointed to by \code{inode->i_mapping}. We treat the sector numbers in \code{bio} as the content on disk, which connects the page cache and disk sector/block. (3) The kernel designs a general layer to support all types of file systems and drivers. All requests for copying data in or out of the disk go to the same interface \code{submit_bio}. Therefore, \code{bio->bi_opf} in the interface is used as an anchor object.

\textit{(2) Content}:
%\label{sec:anchor-of-file-content}
%Buffered I/O refers to the method of accessing a file's content through its page cache in memory, and the pages within the page cache are organized by memory management subsystem as shown in \cref{fig:file-system}. 
As alluded to earlier, file content can be represented in-memory (buffered I/O) or on disk (direct I/O). Specifically, the in-memory caches are accessible via data pointers; the on-disk file content is addressable by sector numbers. 
In reviewing the syscall documentation, we realize that a flag in the \code{open()} syscall controls the access mode, and therefore, we consider the access mode separately for \code{read()} and \code{write()} syscalls, i.e., we review their call graphs conditioned on the access mode.
In summary, we find page caches accessed through \code{inode->i_mapping} in the VFS layer, which is one anchor object. We find anchor object in the generic block layer that contains the sector numbers and interacts with the disk, \code{bio->bi_iter->bi_sector}.
\zhiyun{only two objects in this cateogry?}
%\zhiyun{list the specific objects we find here and briefly explain them (if too many, give a few examples and then a forward reference to the Tables that list all anchor objects of this type).}
%A separate call-graph analysis of two access modes is necessary to identify the two types of anchors. Based on the separated call graphs, we find the anchors in abstraction layers with specific patterns.
%
% Therefore, \name{} needs to identify the anchor objects for buffered and direct I/O, respectively. 
%

%
% Second, \name{} builds the call graph per file system after the discerning. Analyzing the same functions within the call graphs of different file systems contributes to identifying the anchor in compatible abstraction layers.
%



%
%As for the call-graph separation, we observe that upon opening a file with the argument \code{O_DIRECT}, the kernel stores the state into \code{file->f_flags}. This state is subsequently transmitted to \code{kiocb->ki_flags} with the value \code{IOCB_DIRECT}. This value aids \name{} in discerning between buffered I/O and direct I/O.
%
\cut{
Buffered I/O: 
\name{} finds that different file system implementations call the same functions back to VFS when accessing page cache.
%
Afterward, \name{} traces the argument representing the user buffer so that we spot the kernel buffer that copies to/from it. The abstract objects represent the kernel buffer (the file content). 
%
%
Direct I/O: The Linux kernel defines a type \code{sector_t} to represent a sector number (Note that block number also uses this type). 
%
To further refine objects with fields of type \code{sector_t}, \name{} compares the call graphs of different file systems to find the common functions in the generic block layer. 
%
We consider an abstract object embodying \code{sector_t} in the common functions, i.e., \code{bio->bi_iter->bi_sector}.
%
}

%The cached content of a file can be found in VFS, \code{inode->i_mapping}. As for the transient data representing the content on disk, we select the sector number in \code{buffer_head} in the general layer, which is compatible with all types of systems and device drivers.
%






% We select the anchor objects that record the read and write events: \code{bio->bi_opf} in the uniform recorded events representing read (from the disk to the memory) and write (from the memory to the disk).
%Because reading and writing are two opposite operations, the only difference is the copying direction between memory and disk. 
%


%Massive non-control objects have diverse semantics; more importantly, the criticality of an object is determined by its semantics. Unfortunately, there is no documentation on the semantic meaning of data structures. 
%\ziyue{\sout{Even worse, the kernel is changing from version to version, making it virtually impossible to keep documents updated in time.}}

%To resolve this challenge, we select a minimum set of non-control objects with the semantics of fundamental elements. 
%The initial seed objects are selecte following the concrete objects designed to serve as anchors, ensuring their general applicability across various kernel versions based on the kernel design (We term these objects as \textit{\textbf{anchor objects}}). 
%Through the analysis of anchor propagation, we can identify other critical objects. This section explores these objects within each attack strategy.



% One important function of the kernel is to manage the peripheral devices. 
% To monitor their states, the kernel provides various interfaces to record the events. 
% Whenever there is data exchange between memory and disk, the kernel records the event, including the direction.
% %The Linux kernel records data exchange events when exchanging data at the generic block layer. 
% As shown in the code snippet of kernel v5.15 \cref{fig:example-read-write}, \code{count_vm_events()} is called when there is a data exchange, and its first argument indicates the direction of copying from/to the memory. Here, \name{} takes the function name with selected values of its first argument, \code{PGPGOUT} and \code{PGPGIN} as an approximation of the ``anchor object''. 
% \zhiyun{which object is the anchor object here?} \jim{bio}










\begin{algorithm*}[!t]
    % \SetAlgoVlined
    \SetVlineSkip{0pt}
    
    
    \footnotesize
    \small
    \caption{\small \ziyue{This algorithm seems trivial and needs further polish} FSKO Propagation and Discovery}
    

\newlength\mylen
\newcommand\myoutput[1]{%
  \settowidth\mylen{\KwOut{}}%
  \setlength\hangindent{\mylen}%
  \hspace*{\mylen}#1\\}

\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
%\normalem %%%% disable auto underline
\DontPrintSemicolon

% input output

% \Statex{$Refs$ - A set of identified reference objects.}
%\Statex{$Keys$ - A set of identified key objects.}

\SetKwProg{Fn}{Function}{}{}
\SetKwFunction{isState}{isState}
\SetKwFunction{isReference}{isReference}
\SetKwFunction{FlagProp}{FlagProp}
\SetKwFunction{RefProp}{RefProp}
\SetKwFunction{COWDiscovery}{COWDiscovery}
\SetKwFunction{FlagInBranch}{FlagInBranch}
\SetKwFunction{FlagAffectedByBranch}{FlagAffectedByBranch}
\SetKwFunction{AssignLogic}{AssignLogic}
\SetKwFunction{AssignArith}{AssignArith}
\SetKwFunction{Main}{Main}

\SetKwData{Anchors}{Anchors}
\SetKwData{Flags}{Flags}
\SetKwData{Refs}{Refs}
\SetKw{KwNot}{Notations::}

\newcommand\mynot[1]{%
  \settowidth\mylen{\KwNot{}}%
  \setlength\hangindent{\mylen}%
  \hspace*{\mylen}#1\\}
  
\newcommand\myin[1]{%
  \settowidth\mylen{\KwIn{}}%
  \setlength\hangindent{\mylen}%
  \hspace*{\mylen}#1\\}
\vspace{-15pt}


\SetInd{0.5em}{0.5em}
\label{algo:main}


\setlength{\columnsep}{-5cm}
\begin{multicols}{2}


\KwIn{\Anchors: anchor objects including}
\nonl\myin{permission, content, and operation.}
\nonl\;
\KwOut{\Flags: identified flag objects.}
\nonl\myoutput{\Refs: identified reference objects.}
\vfill\null
\columnbreak

\nonl\textbf{Notations: }\isState{}: check whether the object is a state-based flag\\
\nonl\mynot{\isReference{}: check whether the object is a reference}
\nonl\mynot{\AssignLogic{}: get the flags used in the assignment with logic operations}
\nonl\mynot{\AssignArith{}: get the flags used in the assignment with arithmetic operations}
\nonl\mynot{\FlagInBranch{}: get the flags used in a branch}
\nonl\mynot{\FlagAffectedByBranch{}: get the flags affected by a branch}

\end{multicols}

\vspace{-15pt}

\setlength{\columnsep}{0cm}
%\vspace{-6pt}

% \begin{tablenotes}%\scriptsize
%     \item [1]{$\circleddash$: the pointer can point to another \code{page} object, triggering a page UAF. More objects are listed in reference \cref{tab:extended-page}.}
%     \item [2]{$\triangle$: the pointer connects page cache by data assignment.}
%     \item [3]{$\divideontimes$: the pointer can leak address of \code{page} object used as page cache.}
%     \item [3]{$\bigstar$: the pointer can write the page content through \code{page} pointer.}
% \end{tablenotes}
% \FlagProp{\FlagInBranch{flag}}\;
\nonl\hrulefill
\vspace{-10pt}


\begin{multicols}{3}
\Fn{\FlagProp{obj}}{
    \If{obj $\in$ \Flags $||$ $!$\isState{obj}}{
        \KwRet\;
    }
    \Flags $\leftarrow$ \Flags $\cup$ $\{obj\}$\;
    \For{flag $\in$ \AssignLogic{obj}}{
        \FlagProp{flag}\;
    }
    \For{flag $\in$ $\{$\FlagInBranch{obj} $\cup$ \FlagAffectedByBranch{obj}$\}$}{
        \FlagProp{flag}\;
    }
}

\Fn{\RefProp{obj}}{
    \If{obj $\in$ \Refs}{
        \KwRet\;
    }
    \Refs $\leftarrow$ \Refs $\cup$ $\{obj\}$\;
    \For{ref $\in$ \AssignArith{obj}}{
        \RefProp{ref}\;
        \COWDiscovery{ref}\;
    }
}

\Fn{\COWDiscovery{obj}}{
    \FlagProp{\FlagInBranch{obj}}\;
}

\vspace{+5pt}
\Fn{\Main}{
    \For{obj $in$ \Anchors}{
        \If{\isState{obj}}{
            \FlagProp{obj}\;
        }
        \ElseIf{\isReference{obj}}{
            \RefProp{obj}\;
        }
    }
}

\end{multicols}
\vspace{-6pt}
%\ULforem %%%% enable auto underline

% \begin{tablenotes} \scriptsize
%     \item [1]{$\circleddash$: the pointer can point to another \code{page} object, triggering a page UAF. More objects are listed in reference \cref{tab:extended-page}.}
%     \item [2]{$\triangle$: the pointer connects page cache by data assignment.}
%     \item [3]{$\divideontimes$: the pointer can leak address of \code{page} object used as page cache.}
%     \item [3]{$\bigstar$: the pointer can write the page content through \code{page} pointer.}
% \end{tablenotes}
\end{algorithm*}




\textit{(3) Operation:}
%
% \name{} respectively analyzes the call graphs of read and write to find their commonly-called function. 
% This analysis identifies the common functions generic to both read and write operations. 
We primarily focus on reviewing the \code{read()} and \code{write()} syscalls as the file operation is likely encoded in some form internally in the two abstract layers. 
To be more efficient, we compare the call graph of the two syscalls and focus on the intersected internal functions within the two abstract layers. This is because the objects that represent file operation should appear as arguments to common functions shared by \code{read()} and \code{write} syscalls. Otherwise, if they go down completely different paths, file operations may already be implicitly encoded in different function invocations.
Indeed, for buffered I/O, we find that there is no object representing file operations because the kernel already uses \code{vfs_read()} and \code{vfs_write()} to distinguish the operations. 
On the other hand, for direct I/O, we find there is 
an object called \zhiyun{complete this...} 



\cut{
after comparing call graphs of direct I/O, \code{sys_read} and \code{sys_write} go down to the same function, \code{submit_bio}.
%
Additionally, we observe an object that stores the operation in VFS right after handling read/write syscalls. 
Its value equals \code{WRITE} when writing and equals \code{READ} when reading. 
%
Its value (or called state) influences an object as an argument of \code{submit_bio} in the generic block layer. So we treat this object as an anchor.
%As shown in~\cref{fig:flag-mapping}, \code{iov_iter->type} from VFS first determine \code{dio->op} by control dependency at line 16-20, and \code{dio->op} is assigned to \code{bio->bi_opf} through data dependency at line 4 and 9. 
%Therefore, \code{bio->bi_opf} in the common-called function is an anchor.
%
%distinguishes read and write operations as shown in at line 16, and \code{iov_iter->type} is identified as an anchor.



We can refrain from analyzing the operation objects for buffered I/O.
% when reading and writing by accessing cached content, t
First, the call graphs of buffered read and write do not share functions in common. The kernel separates two sets of functions, such as \code{vfs_read} and \code{vfs_write}, instead of calling the same function with variables indicating two operations.
%
Additionally, when no cached data is available, the common function \code{submit_bio} is called to interact with the disk to construct the page cache. This function is already analyzed when conducting direct I/O analysis.
}




\subsection{Cross-Layer FSKOs Discovery}
\label{sec:type-based-object-discovery}
In order to find the complete list of FSKOs, we develop a static analysis solution, termed \name{}, that analyzes how the anchor objects we found in the abstract layers may generalize into other objects in the concrete implementation layers.
%the propagation of abstract objects, as they can propagate to specialized objects in implementation layers and other objects within the same abstraction layer.
More specifically, we design static analysis rule to track how anchor objects propagate into other objects across layers. In order to track the flow of these objects properly, these rules operate forward and backward. 
Ultimately, the key is to identify other objects that carry the same or similar semantics.


\name{} takes the abstract objects as input and outputs the propagated FSKOs, starting from \code{main} in~\cref{algo:main}.
%
%\name{} identifies propagated FSKOs by examining their influence on abstract objects or their being influenced by abstract objects. 
%
To capture this propagation in specific, \name{} explores the data dependency and control dependency of the FSKOs with characteristics in the file system.
%



\subsubsection{Discovery Scope}
%
%\jim{example}
Although the semantics classify three types of FSKOs, we must consider their code implementation when analyzing the source code.
%
\name{} traces two formats of implemented objects: flag and reference.
The \textbf{\textit{flag}} object signifies shared states among all files, and direct \textit{overwriting} with a predetermined value can lead to privilege escalation. The objects representing permission and operations are implemented as flag objects. 
%
The \textbf{\textit{reference}} objects represent the unique memory locations (pointers) and disk locations (sector numbers). The two kinds of objects correspond to buffered I/O and direct I/O, respectively.
Modifying the reference from pointing to a read-write file to a read-only one achieves root; we can apply the \textit{swapping} to the reference objects.
%



Moreover, \name{} only focuses on the most basic objects representing three kinds of semantics while excluding the wrapper objects.
We term the \textbf{\textit{wrapper}} as the objects containing multiple kinds of FSKOs.
Though swapping a whole wrapper can achieve root as Dirty Cred does, analyzing the wrapper propagation is unnecessary.
%
The wrapper recognition is naturally iterative to ensure discovering the complete lists of wrappers. The reason is, theoretically speaking, swapping a wrapper's wrapper can eventually swap the internal FSKOs.
%
Nevertheless, the one-layer wrappers are already extensive and propagated in numerous locations, resulting in a multitude of critical objects. For example, 146 wrappers containing \code{file *} are used in Dirty Cred, and 153 wrappers containing \code{inode *}. Besides, the wrappers contain too many other fields, so swapping the whole object may cause side effects that crash the kernel. 
%
It's worth noting that identifying wrappers becomes straightforward once basic FSKOs are identified. But, assessing whether a wrapper is critical and exploitable can be challenging, necessitating extensive manual efforts, thus deferred to future work.








\subsubsection{Propagation Analysis}

The file system is well-suited for applying multi-layer type analysis to trace critical data.
% 
The basic idea is that if an instance is stored as a particular structure type, it is later loaded from the same type to use. Therefore, we use type consistency instead of a heavy points-to analysis to trace instances.
%
The data flow or control flow may be broken in the cross-syscall (cross-entry) program, leading to a miss of propagated objects~\cite{zhang2021statically,lu2023practical}. The case gets even worse in the file system because many syscalls can be triggered after calling \code{open} a file, such as \code{read}, \code{write}, and \code{mmap}. We use structure types to re-establish the propagation relationship. 
For example, the page cache in \code{inode->i_mapping} is assigned to \code{file->f_mapping} in \code{open} syscall. In another syscall \code{splice}, the page is loaded from \code{file->f_mapping} and subsequently assigned to \code{pipe_buffer->page}.
%
We leverage multi-layer type analysis to resolve it since cross-syscall objects have consistent structure types.
% \zhiyun{The purpose of this paragraph is unclear. Is it an overview of the following sections? If it is an overview, it should not contain low-level technical details such as how to track data flow and control flow across syscalls. }


%\name{} designs three propagation rules based on the file system characteristics to achieve precise results. Regular data and control dependencies introduce many non-critical objects and miss critical ones. First, we trace the propagation between a flag and another flag, creating a state mapping involving logic expressions. Second, a reference can propagate to another reference with arithmetic computing. Third, we consider the page cache's specific mechanism, Copy-On-Write (COW). A flag can influence a reference value through control dependency, which combines the first two propagation rules. As shown in~\cref{algo:main} (line 23), \name{} starts with \code{main} function to trace each anchor to send to \code{FlagProp} for flags and \code{RefProp} for reference.



% \jim{ref - ref, data. COW: flag - ref, control} 
% \jim{input output(graph), when use type, when use data-flow, cross-syscall}

% \jim{three prop, determine is flag or ref}
% According to the characteristics of the two types of objects, we trace the propagation of state-based flag objects (\cref{sec:flag-propagation}) and reference objects (\cref{sec:ref-propagation}), respectively. \name{} takes the anchors as input and outputs the found flag and reference objects, as shown in \code{main} in~\cref{algo:main} (line 37). 
% Considering the specific mechanism named Copy-On-Write (COW) of the page cache, we combine the flag and reference propagation to find the COW-controlling flags (\cref{sec:cow-flag}). 
% %
% All the propagation rules are type-based analyses for better precision.


% According to the characteristics of the two types of objects, we trace the propagation of state-based flag objects and reference objects, respectively. \name{} takes the anchors as input and outputs the found flag and reference objects, as shown in \code{main} in~\cref{algo:main} (line 37). 
% Considering the specific mechanism named Copy-On-Write (COW) of the page cache, we combine the flag and reference propagation to find the COW-controlling flags. 
% %
% All the propagation rules are type-based analyses for better precision.
%\name{} flags them as potentially critical by tracing along data dependency and control dependency.

\begin{comment}
    

\algdef{SE}[VARIABLES]{Variables}{EndVariables}
   {\algorithmicvariables}
   {\algorithmicend\ \algorithmicvariables}
\algnewcommand{\algorithmicvariables}{\textbf{vars}}

\begin{algorithm}[t]
\scriptsize
\caption{\small Key Objects Discovery}
\label{algo:main}

\begin{algorithmic}[1]
\INPUT
\Statex{$Anchors$ - A set of anchor objects: permission, content, and operation.}

\OUTPUT

\Statex{$Flags$ - A set of identified flag objects.}
\Statex{$Refs$ - A set of identified reference objects.}
%\Statex{$Keys$ - A set of identified key objects.}

\end{algorithmic}

\begin{multicols}{2}
\begin{algorithmic}[1]

\Variables
\State Flags $\leftarrow$ \{\}
\State Refs $\leftarrow$ \{\}
\EndVariables

\Statex
\Statex

\Procedure{FlagProp}{A}
  \If{A $\in$ Flags || !IsState(A)}
    \State\Return 
  \EndIf
  \State Flags $\leftarrow$ Flags $\cup$ \{A\}
  \For {N $\in$ AssignFrom(A)}
    \State \scshape FlagProp\upshape(N)
    \State \scshape FlagProp\upshape(FlagInBranch(N))
    % \For {F $\in$ FlagInBranch(N)}
    %     \State FlagProp(F)
    % \EndFor
  \EndFor
  \For {N $\in$ AssignTo(A)}
    \State \scshape FlagProp\upshape(N)
    \State \scshape FlagProp\upshape(FlagInBranch(N))
    % \For {F $\in$ FlagInBranch(N)}
        
    % \EndFor
  \EndFor
  
  %   \State Source $\leftarrow$ getSourceAlgebra(U)
  %   \State Sink $\leftarrow$ getSinkAlgebra(U)
  %   \If {Source == A}
  %     \State FlagPropagation(Sink)
  %   \ElsIf {Sink == A}
  %     \State FlagPropagation(Source)
  %   \EndIf
  %   \State F $\leftarrow$ getFlagInBranch(U)
  %   \State FlagPropagation(F)
  % \EndFor
	% \State\Return Flags
\EndProcedure

\Statex

\Procedure{COWDiscovery}{N}
    \State \scshape FlagProp\upshape(FlagInBranch(N))
\EndProcedure

\Statex

\Procedure{RefProp}{A}
    \If{A $\in$ Refs}
        \State\Return 
    \EndIf
    \State Refs $\leftarrow$ Refs $\cup$ \{A\}
	\For {N $\in$ ArithmeticFrom(A)}
            \State \scshape RefProp\upshape(N)
            \State \scshape COWDiscovery\upshape(N)
        \EndFor
        \For {N $\in$ ArithmeticTo(A)}
            \State \scshape RefProp\upshape(N)
            \State \scshape COWDiscovery\upshape(N)
        \EndFor
        % \State Source $\leftarrow$ getSourceArithmetic(U)
        % \State Sink $\leftarrow$ getSinkArithmetic(U)
        % \If {Source == A}
        %     \State RefPropagation(Sink)
        % \ElsIf {Sink == A}
        %     \State RefPropagation(Source)
        % \EndIf
        
        %\State Refs $\leftarrow$ Refs $\cup$ New
    % \EndFor
\EndProcedure

\Statex

\Procedure{Main}{}
\For{A $\in$ Anchors}
    \If {isState(A)}
        \State \scshape FlagProp\upshape(A)
    \ElsIf{isReference(A)}
    \State \scshape RefProp\upshape(N)
    \EndIf
\EndFor
\EndProcedure
\end{algorithmic}
\end{multicols}
\end{algorithm}

\end{comment}




% \subsubsection{Type-Based Analysis}
% \label{sec:type-based-analysis}






%We match multiple layers of types (cite access path, suture) to enhance the result precision. For example, the \code{page} structure type is designed to manage 4KB physical memory pages. However, our focus lies solely on the \code{page} responsible for caching file content, making it the target of interest, while other \code{page} instances are not considered trace targets. We can identify the instances for page cache by matching the higher-level structure that is designed for page cache management, namely, \code{inode->i_mapping}. 


%\jim{we choose the type-based method to solve cross-syscall, the same problem that Hang's paper tries to solve.}




% \begin{figure}
% \centering
% \begin{subfigure}
% \begin{minted}[fontsize=\scriptsize, highlightlines={6}]{c}
% bool blk_update_request(struct request *req, 
%     blk_status_t error, unsigned int nr_bytes) {
% ...
% 	if (req->rq_flags & RQF_MIXED_MERGE) {
% 		req->cmd_flags &= ~REQ_FAILFAST_MASK;
% 		req->cmd_flags |= req->bio->bi_opf & REQ_FAILFAST_MASK;
% 	}
% ...
% }
% \end{minted}
% \caption{The assignment from a flag state to another flag with boolean algebra computing.}
% \label{fig:example-data-dependency}
% \end{subfigure}

% \begin{subfigure}
% \begin{minted} [fontsize=\scriptsize, highlightlines={11,12,15}]{c}
% static inline unsigned char iov_iter_rw(const struct iov_iter *i)
% {
% 	return i->data_source ? WRITE : READ;
% }

% static ssize_t __blkdev_direct_IO(struct kiocb *iocb, 
%     struct iov_iter *iter, unsigned int nr_pages) {
%   ...
%   bool is_read = (iov_iter_rw(iter) == READ)
%   ...
%   if (is_read) {
%     bio->bi_opf = REQ_OP_READ;
%     ...
%   } else {
%     bio->bi_opf = dio_bio_write_op(iocb);
%   }
%   ...
% }
% \end{minted}

% \caption{A flag state is determined by another using a conditional branch.}
% \label{fig:example-control-dependency}
% \end{subfigure}
% \caption{Two methods for mapping a flag state to another, resulting in state-based propagation.\jim{maybe delete them.}}
% \label{fig:example-data-control}

% \end{figure}

\begin{figure}[!t]
    \centering

%\begin{subfigure}{.475\textwidth}
	\begin{minted}[highlightlines={4,9,16, 17},samepage]{c}
// state mapping through data dependency
static inline void bio_set_op_attrs(struct bio *bio, unsigned op,
		unsigned op_flags) {
	bio->bi_opf = op | op_flags;
}
static inline void dio_bio_alloc(struct dio *dio, ...) {
  struct bio *bio;
  ...
  bio_set_op_attrs(bio, dio->op, dio->op_flags);
  ...
}
// state mapping through control dependency
static inline ssize_t do_blockdev_direct_IO(...) {
  struct dio *dio;
  ...
  if (iov_iter_rw(iter) == WRITE) {
		dio->op = REQ_OP_WRITE;
		...
  } else {
		dio->op = REQ_OP_READ;
  ...
}
\end{minted}
\caption{The state mapping between two flag objects.}
\label{fig:flag-mapping}
\end{figure}






%\label{sec:flag-propagation}

% Take an anchor object as an example, the lower bits of \code{inode->i_mode} indicate rwx access permission of a file, having the states including \code{MAY_READ}, \code{MAY_WRITE}, etc.
%
%We consider an integer-type object as a NON-flag if its value does not represent any semantic state. We apply specific rules to prune non-flag objects. First, the objects used in boundary checks represent size information. Second, the object serves as a reference counter, commonly involved in addition and subtraction computations. Last, the object containing the error code represents the return states, but it falls outside the scope of critical objects.

%\code{bio->bi_opf} has the states defined as \code{REQ_OP_READ}, \code{REQ_OP_WRITE}, etc. And


\begin{figure*}[!t]
    \centering
    \includegraphics[width=.85\linewidth]{figure/file-system.pdf}
    \caption{Some key objects identified by \name{} are highlighted in red, propagating all file system layers.}
    \label{fig:file-system}
\end{figure*}


\PP{Rule 1: Flag Propagation}
Permission information and file operations are implemented as a flag field in the structures.
%
A flag object has multiple but limited states, often implemented as different macros predefined by constant numbers.
%
%\name{} traces the propagation by analyzing the state mapping between flag objects. 
%
A flag state can be mapped to another through data or control dependency, as illustrated using \code{FlagProp} in ~\cref{algo:main}. First, direct assignment between two flags and the assignment involving a logical expression, AND(\&), OR(|), NOT($\sim$). \name{} analyze this data dependency using \code{AssignLogic}.
For example, \cref{fig:flag-mapping} at line 9 shows that \code{dio->op} and \code{dio->op_flags} are assigned to \code{bio->bi_opf} after OR(|) operation.
The second mapping utilizes control dependency to influence flag states implemented as condition branches. \name{} gets the flags used in a branch using \code{FlagInBranch} and the flags affected by other flags in a branch using \code{FlagAffectedByBranch}. 
As shown in~\cref{fig:flag-mapping} at lines 16-22, \code{dio->op} are affected by the abstract object \code{bio->bi_opf}. 
%
% The data and control dependency are built for each newly discovered object iteratively.

%This flag in \code{iov_iter} represents the user's request to perform a read or write operation. If its value is not NULL, the flag in \code{bio} is set to a constant macro, \code{bio->bi_opf = REQ_OP_READ;}; otherwise, the flag is set to the return value of \code{dio_bio_write_op()}.




\PP{Rule 2: Reference Propagation}
%\label{sec:ref-propagation}
The reference object propagates its particular value only through the assignment. This is because distinct reference types, namely, sector numbers and \code{page} pointers, serve as unique reference identifiers. 
%Since the unique values cannot be predicted or predefined, assignment remains the sole propagation method. The reference objects can be corrupted to point from a writable file to a read-only file, enabling a normal user to achieve root.
%
After identifying the abstract reference objects as the input, \name{} finds the objects assigned to or from the page cache and sector numbers using \code{RefPropagation} in \cref{algo:main}. These assignments may involve arithmetic operations, and we conservatively consider they are target objects after the arithmetic. Similarly, \name{} traces the propagation forward and backward by iteratively the source and sink at lines 15-20 using \code{AssignArith}.
%\jim{Not all page, but only page cache}

% Identifying reference objects is important because a normal user can write to a read-only file by replacing the reference with the file's . As for the content on disk, there is no permission check at the low layers of the file system. 
% The file system focuses on efficient data exchange below the buffer cache layer. 
%Therefore, analyzing the data assignment is sufficient to find critical objects representing sector numbers.





\PP{Rule 3: COW-Controlling Flag Discovery}
%\label{sec:cow-flag}
While both disk and memory support Copy-On-Write (COW), \name{} focuses on the memory COW.
%identifying the flag objects responsible for controlling the COW mechanism in the page cache. 
%
%
The reason is that a normal user can trigger a memory COW but is not permitted to trigger a disk COW of a read-only file.
% The kernel can map the page cache of a read-only file to a user for reading. It will not allocate a new memory region until write requests. Corrupting the COW-controlling flag can map the page cache instead of the new memory region with read-write permission, achieving a malicious write on the read-only file.
% %
% In contrast, disk COW in some file systems, like Btrfs~\cite{BtrfsWik97:online}, ZFS~\cite{ZFSWikip35:online}, and XFS~\cite{Newtrick63:online}, creates the copy only after checking writing permission. A normal user cannot trigger disk COW, lacking write permission. 
%
Specifically for memory COW, \name{} finds the flag in a conditional branch controlling whether to obtain the existing page cache or allocate a new page.
After collecting the propagation sites of the page cache and the new-page allocation sites, we trace the conditional branches that determine whether to execute the propagation site or allocation site. \name{} gets the flag in branch at the line 21 in \cref{algo:main} by calling \code{COWDiscovery}.
%
Then, \name{} analyzes all objects contributing to the branch condition, which relies on the state-based flag propagation \code{FlagPropagation}. The output set of flag objects will be completed after the COW-controlling flag discovery.



%However, memory management controls all pages, and their semantics should be considered. The kernel follows the Copy-On-Write(COW) principle to avoid unnecessary new page allocation and memory copying. More importantly, access control is guaranteed by both the page table and several permission checks in the kernel. If an unprivileged user requests a read-write memory, the kernel maps the page cache to the user by modifying the controlling flag, which is prone to be corrupted as Dirty COW and Dirty Pipe do. 



%Furthermore, memory management enlarges the attack surface of \code{page} pointer corruption. We propose a novel exploit strategy: \exploit{} to write a sensitive page cache, which makes many objects exploitable for various vulnerability capabilities. Our technique needs as little as a one-bit write on a heap and does not rely on information leaks. More details are in \cref{sec:exploit}.





\subsection{Summary of Identified Objects}
Some identified objects are highlighted in red in \cref{fig:file-system}, spreading from the top VFS layer to the bottom driver layer. 
%
We manually analyze the semantics of the whole file system and summarize its layers in \cref{fig:file-system}.
%
The left part represents the metadata, while the right side represents the content, with a dotted vertical line separating them. 
%
Taking metadata as an example to show the propagation, the abstract object representing permission \code{inode->i_mode} can \textit{affect other object's value}; in other words, it propagates to another object \code{file->f_mode} which indicates permission as well. 
%
Additionally, \code{inode} is a nested structure of the larger parent object in specific file system implementation, e.g., \code{ext2_inode_info}. 
%Therefore, when dereferencing \code{inode}, the pointer points to the inside of the larger object.
The parent object's fields come from (\textit{are affected by}) \code{ext4_inode}, which organizes the metadata based on the data layout on the disk. Finally, the object is delivered to lower layers to retrieve the data from the disk. 
%
The lower layers from the buffer cache to the driver transfer the read/write operations to the disk, which does not differentiate content or metadata shown in~\cref{fig:file-system}. Many FSKOs are involved during low-level synchronization, e.g., \code{iomap_dio->flags} represents the read/write direction.



\PP{Summary of existing dirty CVEs and exploits.}
Both Dirty Pipe and Dirty COW involve manipulating COW-controlling flags that control the user to write either the page cache or a newly allocated page. After corrupting the controlling flags, the malicious user buffer will be written into the page cache. As shown in~\cref{fig:file-system}, the Dirty Pipe flag belongs to the pipe subsystem, and Dirty COW occurs in memory management. Dirty Cred~\cite{lin2022dirtycred} is a new exploit strategy that swaps low-privilege objects with high-privilege ones, using objects representing permission in VFS, i.e., \code{file->f_mode}.


% After studying the results, we find corrupting metadata on disk is challenging and unnecessary for three reasons.
% (1) This attack method occurs at the lower layers, from the buffer cache layer to the driver layer in \cref{fig:file-system}, where the kernel does not differentiate content or metadata.
% Therefore, they use the same synchronization interfaces and data structures, causing the corruption of the same objects for both metadata and content. However, corrupting file content is much easier for the following two reasons. 
% %
% (2) The Linux kernel does not support direct data exchange between metadata on disk and a user buffer. On the contrary, a fully user-controlled buffer can be exchanged with file content on disk using direct I/O. While accessing the cached data from user space is called buffered I/O in \cref{fig:file-system}.
% %
% (3) Multiple metadata are placed on a page to synchronize with a continuous region on disk. Replacing the disk number overwrites the other unintended files' metadata. However, file content is stored at page granularity in memory and at block granularity on disk, not affecting other files.




% Moving from abstract semantics to theoretical implementations, there are five kinds of key objects in concept, which we classify their semantics as: (1) metadata in memory, (2) metadata on disk, (3) the content in memory, (4) content on disk, and (5) operations on the file content. A file entity that includes metadata and content is stored permanently on the disk. When a user requests to execute the operations on the file, the kernel eventually loads the data from the disk. However, communicating with the disk consumes much time, so the kernel caches the file entity in memory for better performance, including metadata and content. Specifically, we define the cached content as page cache, shown in \cref{fig:attack-elements}. The user accesses the cached data that periodically synchronizes with the disk, called buffered I/O. The kernel also provides the interfaces for users to access the disk directly, i.e., direct I/O.



% However, due to many optimizations to simplify the code complexity in the actual kernel implementations, \textit{only four kinds of objects exist}. Corrupting the metadata on disk is both challenging and unnecessary for three reasons.



% In the context of this attack, only direct I/O is susceptible, as it allows the user to control the buffer and synchronize a malicious payload with the file content on the disk. But for buffered I/O, controlling the content in the page cache is necessary before converting the operation, which would be futile. This is because privilege escalation has already been achieved through the overwritten page cache, as described in the second method (B), rendering the direction corruption unnecessary. 

% The sector numbers determine the disk placement; we can replace them to write a sensitive file.
% As for the content in the page cache, the Linux kernel synchronizes the page with the disk periodically (or when calling sync syscall). Direct I/O can directly exchange the file content between the user buffer and disk, where the user buffer has to be aligned with the page's size. Before the data exchange for both access types, we replace the sector number of a read-write file with the one of a sensitive file. 

\begin{comment}
    

\subsubsection{Tracing Flag Object}
\label{sec:tracing-flag}

First, \name{} locates anchor objects among file system source code.
%
Permission is implemented as a flag field in the structures, so \name{} directly uses it to trace its control and data dependency. 
%
Regarding file operations, they are implemented as flag objects.
Based on the anchors indicating the data exchange event, \name{} finds the flag objects that manage either memory copy from and to the disk. 
Specifically, \name{} searches the control dependency tree to find them in the conditional branches.   
%
Another type of flag object controls obtaining the existing page cache or a newly allocated one. 
After identifying the propagation of page cache in \cref{sec:tracing-reference}, \name{} analyze the control dependency to find the controlling flag objects.

Once the source objects are located, \name{} analyzes the data and control dependencies both forward and backward. The semantics of an object is transferred to another object in two ways: (1) data assignment, which flows through data dependency, and (2) its state is controlled by or controls the others' state. For example, the flag \code{bio->bi_opf} indicates the data exchange direction. In \cref{fig:example-data-dependency}, the flag is assigned to \code{request->cmd_flags} at the driver layer by data dependency. In \cref{fig:example-control-dependency}, the value of \code{bio->bi_opf} is determined by a local variable \code{is_read} whose value comes from \code{iov_iter->data_source}. This flag represents the user's request to perform a read or write operation. All three objects (fields) indicate the semantics to do a memory copy out or in.

\subsubsection{Tracing Reference Object}
\label{sec:tracing-reference}
\end{comment}





% \subsubsection{Analysis Scope}

% This paper focuses on corrupting or replacing an object representing a single abstract element.
% %\guoren{What does this mean? corrupting the fundamental elements in file objects?}
% Our scope excludes composite objects that encompass multiple abstract elements because these objects can be difficult to exploit.
% %
% For instance, one \code{inode} one-to-one manages the metadata and content of a file. However, substituting the whole \code{inode} achieves nothing due to the failure at the permission check towards \code{inode->i_mode}.
% In contrast, this internal field containing a single semantic of an abstract element, i.e., \code{inode->i_mode}, is one target of our work, but the whole \code{inode} is not. Although Dirty Cred substitutes a composite object containing both permission and content. Such exploitation requires the other technique to extend the time window using FUSE \cite{fuse}.
% Additionally, because analyzing dependency introduces many false positives, our analysis is not iterative and uses one-layer trace depth, which may lose some true positives.





% \jim{remove the following to implementation and summary.}
% The permission metadata stored for each file serves as a starting point to discover more populated data. VFS provides abstract interfaces to generalize different FS implementations, where the Linux kernel designs a data structure, \code{inode}. Each \code{inode} manages a single file on disk, establishing a one-to-one relationship. We can find more data tracing its propagation, such as the permission in \code{file}, including access time, permission, and so on. Note that ``\code{file}" indicates the data structure defined in the kernel code to represent the opened file descriptor, and ``file" means a normal file on disk. 

% As shown in \cref{fig:file-system}, \code{inode} is a nested field of the FS-specific data structure with more implementation details to provide abstracted file information. For example, \code{ext4_inode_info} has a field whose type is \code (not pointer); its functionality is similar to the page cache, which caches FS-specific information. Following the least recently used policy, the kernel maintains its allocation and deallocation depending on the memory's sufficiency and explicit dropping from user requests.


% The cached metadata requires to exchange data with the disk. To align with the layout on the disk, the Linux kernel takes out the fields in \code{ext4_inode_info} and incorporates them into a new data structure, \code{ext4_inode}. All files in an EXT4 file system use \code{ext4_inode} for synchronization, and their metadata are contiguous on disk. Besides, the kernel directly allocates a page and divides it into multiple \code{ext4_inode} structures to make them contiguous in memory, leading to better data exchange performance. As shown in \cref{fig:file-system}, the buffer cache layer connects the page with its corresponding sector number. Substituting a metadata sector leads to at least multiple metadata \code{ext4_inode} in a page, which is hard to be stable. Furthermore, file content uses the same interface and data structures to synchronize with the disk, which can be exploited easier because it takes at least one page to hold its content.

% manual filter. numbers.
% summary the figure \cref{fig:file-system}.

%When considering the initial semantics in \cref{sec:initial-semantic}, only the file content in the page cache cannot apply simple tracing because of \code{page} pointer stored in the \code{address_space}. The pointer can point to any page in memory rather than the page caches. 

%\jim{How general pipe is}




\begin{comment}

\subsection{Methodology Overview}
\jim{Answer the question of how to achieve the goal in section 4.1. All in all, make it simple and reasonable by clarifying the metadata and content. DO NOT mention the read/write direction, make it into metadata and content.}
% challenge：
%(1)semantic identify (type-based and struct-based method ) -> 
% first step is manually label, and then use MAPS to trace the propagation
%(2) how to verify -> dynamic technique

This paper conducts a systematic
study to identify all exploitable non-control data in all layers of the Linux file systems.
%
More specifically, we design new techniques combining static analysis and dynamic verification to identify and confirm all non-control data in the file system. The attacker can easily exploit these data to launch the privilege escalation attack.
%
To analyze effective non-control data in the file system systematically and automatically, we need to resolve three challenges.

% \wenbo{one sentence summarize challenge. Several to explain this.
% Our solution, basic idea 
% }

\textbf{Challenge 1.} 
It is hard to model the semantic meaning of the non-critical data.
%How to use the minimum initial seed of labeled data to find more critical data in multi-layer file system automatically and systematically?
As mentioned in the previous sections, we need to know the semantic meaning of non-control data so that we know its controllability and whether it can be exploited to achieve privilege escalation.
%
Unfortunately, there is no documentation on the semantic meaning of the non-control data. Even worse, the kernel is changing from version to version, making it virtually impossible to document the usage of all non-control data.
%
To resolve this challenge, we propose to first classify the non-control data into different categories and model the semantic meaning of an initial set of non-control data for each category (\cref{sec:data-category}). After the modeling, the initial set of non-control data is passed to the automatic identification and verification tool to identify all non-control data in all file system layers.

%The seed data must cover the semantics of all layers, which is the input of our tool \name{} to find more critical flags by tracing seed propagation. In order to be general and systematic, we need to model the semantics of critical data by summarizing and distilling the file system data from the past. Finally, we summarize the non-control data category in \cref{sec:data-category}
%\wenbo{why we need three categories}


\textbf{Challenge 2.} 
It is challenging to achieve a precise and efficient static data propagation analysis on the whole kernel scale.
%
As discussed previously, we need a precise and efficient static analysis to find all critical data propagation automatically, with the initial non-control data as the input.
%
The value-flow analysis based on pointer analysis is not scalable for the kernel. 
%Researchers turn to type matching to refine propagation. 
Although existing works \cite{lu2019does, zhang2019pex} leverage the type to refine targets of function pointers, they still suffer from imprecision problems for two reasons.
%
First, the original LLVM type system is inaccurate, leading to wrong propagation analysis.
Second, there are no formal rules to model the type transition on memory access statements.
%
As a result, the type information is lost on memory access.
%
To overcome this challenge, we propose a novel technique called \textit{Type-based Access Path} (a.k.a. TAP), which defines a set of formal type transition rules and leverages the type metadata to achieve precise and efficient type analysis (\cref{sec:type-analysis}).
%We propose an efficient method, \typename{}, uses the type-based access path to refine data propagation considering memory access, which utilizes accurate types from the type system based on LLVM's metadata, more details of \typename{} in \cref{sec:type-analysis}.
%type-based access path ()
%\wenbo{challenges first, one leads to MAP}


\textbf{Challenge 3.} 
It is difficult to dynamically verify the exploitability of non-control data identified by static analysis.
%
To reduce the false positives, we need to verify the exploitability of the identified non-control data.
%
Unfortunately, the identified non-control data may be scattered on the different layers of the file system.
%
Without specific domain knowledge, it is impossible to know whether it can be exploited to write into a read-only file.
%
To resolve this challenge, we propose a new dynamic approach, which leverages the execution suspension and dynamic value reset to verify the exploitability of non-control data (\cref{sec:dyn_veri}).

%Based on the three data categories, we design a tool \name{}, which uses static analysis to automatically identify critical non-control flags and dynamic verification to confirm whether the flag is effective for attacks.
%We design a tool for \underline{C}ritical n\underline{O}n-control data identification used in \underline{P}ermission \underline{E}scalation attacks, \name{}.
%\wenbo{how to confirm PE? full term is too long}

\vspace{+4pt}
\textbf{Overview}.
\cref{fig:overview} shows the overall structure of our methodology.
%
\cref{sec:data-category} presents the non-control data classification and modeling, in which we propose to classify the non-control data into three categories: file metadata, file content, and read/write direction data.
%
\cref{sec:type-analysis} details the type-based access path, which leverages the LLVM metadata to improve the type resolution precision.
%
\cref{sec:design_imple} talks about the design and implementation of our analysis tool, which takes the initial set of non-control data as the input, and conducts static analysis and dynamic verification automatically to identify the non-control data in the file system that can be exploited to write to read-only files.


%it takes as input the specific modeling in Linux kernel of generic data categories mentioned in \cref{sec:data-category} and kernel bitcode, outputs the effective flags.

%Therefore, one only needs to provide the least modeling of the generic data categories to analyze other file systems.
%three basic elements of file system for the tool, including file metadata, file content, and read/write direction.
%We use types of objects and sub-fields to specify the modeling of the semantics in file system, including non-control data. \textbf{\textit{Our key insight is that Linux kernel well designs the data structure to represent specific semantics.}} For example, \code{inode} and file metadata are one-to-one correspondences, and some of its fields are critical flags in VFS, such as \code{i_mode}. Page cache is organized by \code{address_space->i_pages}, which can be represented for file content in \cref{fig:file-system}.

% This work focus on the non-control data in heap, which can be overwritten with much weaker primitives. Global variables are out of the scope because they relies on arbitrary write primitives, so it is hard to corrupt global variables in the real world.



% \textbf{Assumptions.} 
% %In this work, we consider the capability of a vulnerability through a PoC to write a bit at least and write an integer in memory at most. 
% \zhiyun{This sounds like a restriction. I think we should just say that we assume the capability to be standard heap corruption primitives such as UAF write and OOB write (any version of it even if it just writes a single bit). But we do not assume any arbitrary memory write primitive. Check what wrote in intro. I think they can be put here also.} 
% In this work, we consider the capability of a vulnerability to be standard heap corruption primitives, such as UAF write and OOB write. Any version of the bug works well, even if it just writes a single bit. We do not assume any arbitrary memory write primitive because we focus on overwriting data in heap but not global variables. Besides, Security researchers can manually get the capability of a vulnerability with the assistance of debugging tools. This work leverages the manual capability to automatically verify the effectiveness of identified flags.

% %The required capabilities vary for different identified flags. For example, changing \code{bio->bi_opf} from 0 to 1 can turn reading into writing. However, only enabling the write permission for \code{file->f_mode} leads to a kernel crash, which requires writing the whole integer. More radically, the requirement of changing one bit can be met by rowhammer. Security researchers can manually get the capability of a vulnerability with the assistance of debugging tools. This work leverages the manual capability to automatically verify the effectiveness of identified flags.
% \zhiyun{I do not think we need the above line is needed (starting from ``The required capabilities vary''). When we talk about assumptions, it is unnecessary to include details about }


    
%old comment
\section{Methodology \& Overview}
% why we analyze the three kinds of data
This section describes the study methodology to ensure analyzing non-control data is systematic. After that, It gives a design overview of \name{} drawn from the systematic methodology, which is able to automatically pinpoint the effective dirty flags.


\subsection{Study Methodology}

To meet the demand for systematically analyzing the dirty non-control data in file system, we need to answer three questions. \zhiyun{We need to point out what we are doing fundamentally here. At a high level, this is how I understand it: First, we need to model the semantics of critical data by summarizing and distilling the file system data from the past. Second, we develop automated methods to extrapolate based on an initial seed of labeled data. The two steps basically map to the two questions below. I would suggest mention the two questions first and then talk about the two high-level steps we take to answer the questions.}

\textit{\textbf{Q1:} Which kinds of high-level file-related exploit strategies can result in privilege escalation?} 
As mentioned in \cref{sec:known-cves}, Dirty Cred, Dirty COW, and Dirty pipe have the same attack strategy, writing a read-only file. It is unknown whether there are other strategies. For example, the malicious modification of \code{/etc/shadow} enables the attackers to gain root, and this file (\code{---}) cannot be read, written, or executed by normal users. If attackers can execute \code{/usr/bin/vi} with setuid bit, they can write the file only accessed by root using \code{vi} because its owner is root and executable by normal users (\code{r-x}). 

%\textit{\textbf{Q2:} What is the insight to achieve the attack primitive when mapping the flags of known dirty CVEs into the multi-layer file system? \zhiyun{It is unclear what point we are trying to make (the description is vague). Consider removing the question? The two remaining questions are good enough to me.}} Although we know the root cause of the three CVEs, the abstracted forms of dirty flags from the perspective of file system are quite necessary for a systematic method. For example, the mentioned \code{bio->bi_opf} is not related to the known flags at first glance. We analyze the basic elements of file system to explain the underlying logic of these non-control data.
%underlying logic

\textit{\textbf{Q2:} Which kinds of non-control data support the high-level file-related exploit strategies?} At last, we systematically propose the categories in order to guide the design of automatic tool \name{}.
%^What are the categories of the non-control data based on the insight from known dirty CVEs?} At last, we systematically propose the categories in order to guide the design of tool \name{}.
%\zhiyun{I would move this point up and tie it to Q1, and call it something like ``What are kinds of non-control data support the high-level file-related exploit strategies''. This motivates the need to do an automated solution.}


%that can be exploited for privilege escalation attacks.
%First, we explore the attack of file system for privilege escalation and give the reason for selecting the primitive, writing a read-only file. Then we abstract the form of critical non-control data used in well-known dirty CVEs from the perspective of file system. Finally, we systematically propose three categories of critical non-control data considering the known CVEs abstraction and file system architecture.

\subsubsection{High-Level File-Related Exploit Strategy}

% \begin{table}[t!]
% \centering
% \caption{Inherent files on Linux system as attack targets}
% \begin{tabular}{c|c|c}
%     & Write                                                              & Setuid      \\ \hline
% --- & \begin{tabular}[c]{@{}c@{}}/etc/shadow\\ /etc/sudoers\end{tabular} &             \\ \hline
% r-- & \begin{tabular}[c]{@{}c@{}}/etc/passwd\\ /etc/group\end{tabular}   &             \\ \hline
% r-x & Insert Malicious Code                                              & /usr/bin/vi \\ \hline
% r-s & Arbitrary Code Execution                                           &            
% \end{tabular}
% \label{tab:attack-primitives}
% \end{table}



We study the inherent files that have different permissions for normal users, and the inherent files are the ones on a pure Linux system without installing any user program. 
As shown in \cref{tab:attack-primitives}, the columns represent different kinds of permissions of inherent files, and the rows mean the target operations of attacks. The table only includes two target operations, writing and execution with setuid. Because when attackers obtain an invalid reading or execution, there is no inherent file that can be exploited for privilege escalation on a pure Linux system. The other file operations mentioned in \cref{sec:file-on-disk} are barely used in attacks also.


We use an example to explain \cref{tab:attack-primitives}, the second element (Write) of the third row (\code{r--}) is on behalf of the attacks that conduct write operations on read-only files, which can gain privilege escalation by writing \code{/etc/passwd} or \code{/etc/group}. Although writing to a file without any permission(\code{---}) is able to cause an attack successfully, attackers even cannot open the file leading to fewer permitted operations. Therefore, we select a looser restriction for the attack, writing a read-only file.


Note that attackers can escalate to root by gaining \code{setuid} flag of the executable file \code{/usr/bin/vi}, which fits in the strategy also. Because the file's owner is root and \code{setuid} makes an executable run with privileges of the owner of the file. Once the attackers gain \code{setuid} flag, they can write to the files that are root-writable only using \code{/usr/bin/vi} eventually, for example, the files mentioned before \code{/etc/passwd} or \code{/etc/group}. Essentially the escalation is a result of write operations on read-only files by changing files' metadata, i.e., \code{setuid} flag. 
%
Besides, execution eventually translates to a read that passes down the file system layers, and the permissions of executing and setuid are stored in file metadata. Therefore, we can model the flags related to execution by metadata.


\textit{\textbf{A1:} We extract a high-level file-related strategy to privilege escalation after studying the inherent files -- writing a read-only file.}


% \subsubsection{``Dirty" in File System}
% \label{sec:dirty-in-file-system}

%old comment
% \textit{\textbf{A2:} We abstract the forms of dirty flags using two basic parts of the storage format of a file: file metadata and file content. Considering the design of the multi-layer file system, we abstract out the unified data exchange between main memory and disk for both metadata and content.}

\subsection{Non-control Data Classification and Modeling}
\label{sec:data-category}
% \wenbo{we observe}
In general, any file system of any operating system should design the file metadata (contains permission) and content to organize a file. Importantly, file system does not distinguish metadata or content below the buffer cache layer, as shown in \cref{fig:file-system}. The relative lower layers focus on exchanging data according to the flags representing read/write direction, which only requires the page that stores metadata or content and its corresponding block number on disk. 
Therefore we extract three kinds of elements of the file system and delimit the corresponding three categories of non-control data, which are generic to apply to any other file system.

%the flags that decide read/write direction are critical.

%and handle the data exchange between the main memory and disk. 

%As shown in \cref{fig:file-system}, file metadata and content are the two parts of a file stored on the disk. Dirty Cred attacks the flags signifying metadata, while Dirty COW and Dirty Pipe are related to file content. We explain the reason and detail as follows.
\textbf{File Metadata.} Attackers leverage corruption of file metadata to bypass security checks in VFS layer to gain root, such as Dirty Cred. The permission information of a file is abstracted as metadata. Besides, executing a file translates to a read request passed down the layers of the file system, as mentioned in \cref{sec:file-on-disk}. From the perspective of the file system, the differences between executing and reading are the execution bit and a setuid bit, also metadata. Therefore metadata can be treated as critical.

\textbf{File Content.} It is the primary data that is stored on the disk or cached by page cache. As discussed in \cref{sec:known-cves}, Dirty COW (page cache layer) and Dirty Pipe (file system implementation layer) gain write access to the page cache by corrupting the non-control data. The flags that influence file content are dirty. The non-control flags that determine to obtain the content are critical.

\textbf{Read/write Direction.} File metadata and content are both stored on disk and loaded into the main memory when accessing. Read and write operations are passed down in the whole file system from the top VFS layer to the bottom disk for data exchange. In the process of passing down, the file system distinguishes metadata and content above the file system implementation layer but not below the buffer cache layer. Linux kernel records the unified data exchange events between the disk and main memory in the generic block layer, as shown in \cref{fig:file-system}. We treat the flags that decide read/write direction as critical.

In order to analyze more automatically with minimum input modeling, we select the struct types with field names in the layers that have uniform interfaces, which are framed by gray in \cref{fig:file-system}. (1) File metadata: VFS hides the different implementations to provide abstract interfaces, we select the data structure in this layer to represent file metadata. (2) File content. We select the data structure representing the content of the file in the page cache layer, which is relatively independent of different file system implementations. (3) Read/write direction: Linux kernel uniformly records read/write events when exchanging data at the generic block layer, no matter if it is exchanged for file metadata or content.

%\jim{Our insight, why dirty everywhere}
%\jim{need to be more abstract and systematic}

% \begin{itemize}[leftmargin=*]
% \item \textbf{File metadata} contains permission information, thus metadata itself is critical non-control data, such as \code{file->f_mode} and \code{inode->i_mode}.

% \item \textbf{File content} is cached by page cache in memory for fast access. The non-control flags that determine to obtain the content are critical, i.e., page in page cache. For example, the flags used in Dirty COW and Dirty Pipe.

% \item \textbf{Read/write direction} is represented by flags in lower layers to decide copying from/to the disk. If the data is exchanged in the opposite direction (some only need to flip one bit, such as \code{bio->bi_opf}), we can alter a read to a write, which is also critical. We find several flags that can achieve privilege escalation, as shown in \cref{fig:example-read-write}. This kind of attack is practical because of direct IO for file content, which can exchange the data on a user-controlled buffer with a disk directly. Attackers open a file with valid read permission and conduct direct reading from a disk. During reading, they can write to the file content using a controlled buffer by flipping a critical flag.

% \end{itemize}

% \textit{\textbf{A2:} Based on the three basic elements of file system, file metadata, file content, and data exchange direction, we define three categories of non-control data.}

%\jim{TODO: why we use data structure types}


% \begin{minted}[highlightlines={5,6}]{c}
% static loff_t
% iomap_dio_bio_actor(struct inode *inode, loff_t pos, 
%     loff_t length, struct iomap_dio *dio, struct iomap *iomap) {
% ...
% 	if (dio->flags & IOMAP_DIO_WRITE) {
%         bio->bi_opf = REQ_OP_WRITE | REQ_SYNC | REQ_IDLE;
%         ...
%     } else {
%         bio->bi_opf = REQ_OP_READ;
%         ...
%     }
% ...
% }
% \end{minted}  

%Show the existence and propagation of these three kinds of data in a multi-layer file system.
%\jim{TODO: give examples}
% \jim{TODO: refine value-flow  -\>  type based  -\>  multi-type access path}
% \jim{TODO: map -\> Multi-type-based Access Path}
% \name{} conducts a static analysis to find the start-up flags for three kinds of input struct-fields, and 

% % \subsubsection{Flags Preparation}
% For file content, \name{} traces the struct-field representing in page cache to find where and which variables are stored with the page in page cache. After obtaining the location (instruction) of getting the page, \name{} launches a backward analysis on the control-dependency graph to analyze the non-control flags that control to execute the instruction.

% For read/write direction, \name{} identifies the unified function for recording with the event type argument as shown in \cref{fig:example-read-write}. \name{} backward tracks the control dependency of executing the function to collect the flags to record either read or write.

% In order to analyze more automatically with fewer input struct-fields, \name{} selects the struct-fields in the layers that use uniform interfaces for interactions, which are framed by gray in \cref{fig:file-system}. 
% \begin{itemize}[leftmargin=*]
% \item Modeling file metadata. VFS hides the different implementations to provide abstract interfaces, therefore \name{} takes as input struct-fields representing metadata which is one-to-one a file (\code{inode}) at VFS layer only. After automatic static analysis of data propagation, the tool is able to find more critical data, such as the fields in \code{file}.

% \item Modeling file content. Page cache layer stages the content of the file, and it is relatively independent of different file system implementations. We choose the struct-field representing page cache to feed to \name{}.

% \item Modeling read/write direction. As mentioned in \cref{sec:dirty-in-file-system}, Linux kernel records read/write event when submitting IO requests containing block numbers at generic block layer. \name{} utilizes the unified interfaces for recording the events without considering different file system implementations and different drivers.
% \end{itemize}

%Because the analysis requires precise and stable struct type information, \name{} employs \typename{}, more details in \cref{sec:type-analysis}.

%We model the data structures that represent their existence and propagation. Then we conduct a static analysis to identify the critical data using \name{}. Show the details of static analysis \cref{fig:overview}.
%After building the program dependency graph (PDG), \name{} traces the propagation of start-up flags to find more effective flags on PDG through data dependency and control dependency. And we find the critical non-control data covers all layers of file system shown in \cref{tab:identified-data}. 

%We launch GDB scripts to automatically verify the data effectiveness that is identified by static analysis. Show the detail. 


\subsection{Layer-based Scope Analysis}
\jim{We want to make the analysis closer to the file system. Try to analyze each file system and driver, including vertical and horizontal data-flow between different layers. We can call it scope-adaptive analysis.}

\subsubsection{Horizontal Internal-Layer Analysis}
\jim{Per file system and per driver}

\subsubsection{Vertical Cross-Layer Analysis}
\jim{abstract the shared gv and cross-layer function calls.}

\subsection{Scope-Adaptive Data Propagation Analysis}




\subsection{Exploitability Analysis}
If this section takes too much time to implement, we can consider it as future work?
\subsubsection{Data Allocation Sites}

\subsubsection{Time Window}

\subsubsection{Syscall Identification}

    
\end{comment}

==> back/_5_exploit_bak.tex <==

\section{Exploitablity Analysis}
\label{sec:exploit-analysis}

Instead of forcing the corruption of FSKOs using GDB scripts, we apply three exploit strategies and manually write end-to-end exploits using real-world CVEs to demonstrate the practical exploitability. 
First, we utilize dynamic verification to confirm whether identified objects lead to privilege escalation. 
Then, we use three exploit strategies toward critical objects and summarize them in~\cref{tab:summary}. (1) the direct strategy to corrupt the flag objects, (2) the swapping strategy (generalized Dirty Cred) to replace the whole key object by corrupting reference objects, and (3) the hybrid strategy using page UAF that can be used to corrupt both flag and reference objects. 








\PP{Exploiting with Vulnerability}
There are strict requirements to tamper with FSKOs successfully through memory-corruption bugs.
The corruption capabilities differ significantly among various bugs, and critical data must fall within the overwrite range, as illustrated using an OOB bug example in \cref{fig:global-heap-attacks}.
To clarify the invalid corruption, researchers define bug capabilities for OOB~\cite{chen2020koobe} and UAF~\cite{wu2018fuze}, including which slab cache the vulnerable object is in, where memory the bug can invalidly access, and what values can be set to the memory. 
%
Concerning the memory layout manipulation, the vulnerable and target objects usually share the same cache. Cross-cache attacks would be necessary if these objects reside in different caches, relying on page-level heap fengshui. 
This manipulation guarantees the target objects fall within the overwrite range originating from the vulnerable object.
%
Increasing target objects brings more possibilities for bugs with various capabilities to overwrite them.  
The well-used control flow hijacking by corrupting function pointer is no longer practical due to CFI enforcement.
In contrast, corruption of unprotected data, such as \code{pipe_buffer->flags} identified by \name{}, will directly escalate privilege.
%
All the FSKOs and bridge objects in the hybrid strategy can be corruption targets when exploiting vulnerabilities.


% The initial step in both attack and protection is the identification of critical objects.
% %
% An increased number of target objects makes more bugs become exploitable for attacks and spawns more protections to defend against these attacks. 
% %
% Specifically, matching the bug's capability with the target objects aids in a comprehensive understanding of the bug's hazards. 
% Taking an OOB bug as an example shown in \cref{fig:motivating-example}, it can overwrite a specific length of bytes starting from a particular offset. 
% %

% %
% However, fewer target objects are available when increasing protections are enabled. For example, a common method is to corrupt a function pointer to hijack control flow, but this approach is no longer effective due to CFI. 
% %
% In contrast, corruption of unprotected data, such as \code{pipe_buffer->flags}, which could be identified by \name{}, will directly escalate privilege.



%



% There are two reasons why identifying new critical objects becomes more urgent during mutual reinforcement of attack and defense. 
% %
% First, attackers have fewer candidate objects available as corruption targets since more well-known objects are safeguarded, including function pointer, \code{cred} pointer, page table, etc. 
% %
% Then, the bugs with various capabilities keep emerging, requiring as many critical target objects as possible to match different capabilities. More details are shown as follows.


% Move to intro? A successful attack exploit lies in determining which target objects to corrupt and devising the exploit strategy of how to corrupt.



%Given that writing capability, which objects are the corruption targets is still unclear.



% \textbf{Increasing targets broadens matched bugs.} Having more objects as corruption targets expands the range of matched bugs to launch attacks. Countless bugs are reported every day thanks to the fuzzers~\cite{syzbot22:online, googlesy60:online}. However, only a few of them are finally exploitable to privilege escalation, leaving the majority remain unexploited.
% % However, few bugs are exploitable to privilege escalation attacks, and the majority remain unexploited. 
% %
% Because their various capabilities are poised to align with limited known targets as corruption candidates. More targets bring more possibilities to match different capabilities.
%\jim{mention they are not the most critical for privilege escalation but lead to many different primitives.}
%





% Dirty Cred~\cite{lin2022dirtycred} points out that \code{file} and \code{cred} contain credential information, and proposes a protection mechanism to protect them. 

% \jim{
% It is worth noting that we only focus on the discovery and exploitability of critical objects.
% Automatic matching bug's capabilities with targeted objects is out of this paper's scope, since it is already a challenging problem. Researchers propose many methods solely for automatic matching~\cite{wu2018fuze,chen2020koobe, dai2021facilitating, lin2022grebe, zou2022syzscope,jiang2022evocatio}. 
% Furthermore, our exploitability analysis consists of manually written end-to-end exploits.
% The reason is that automatic exploit generation could be very challenging, and there is no fully automatic method. 
% For example, to demonstrate the exploitability of proposed attack strategies, many researchers manually write exploits to make more bugs exploitable based on the known target objects~\cite{wu2019kepler, zeng2022playing, lin2022dirtycred, liu2022release}. 
% %Nevertheless, the target objects are too limited to generalize the strategies for a broader range of bugs, and many remain unexploitable. 
% }

% The exploit strategies can broaden the target objects to match more vulnerabilities with various capabilities, making them exploitable. We term these as \textbf{extra target objects}. Corrupting these extra target objects achieves specific primitives to corrupt the key objects indirectly. 
% %
% Especially, page cache, a part of memory management, consists of particular reference objects of type \code{page}. This can be used to achieve page UAF primitive to corrupt key objects in hybrid exploit, causing greater attack impact.
% %
% Furthermore, we develop a static analysis to support the static analysis and find the objects that facilitate page-UAF exploits. 


%We believe that security researchers will propose more strategies to exploit the objects more easily in the future.

%We write PoC to trigger memory corruption bugs to directly corrupt the object with the target value as dynamic verification does. We also discuss the adoption of the Dirty Cred strategy to our identified credential objects.



% For flag objects, the verification process involves three steps. First, we record the flag's value when legally writing to a read-write file. Then, we attempt to write to a read-only sensitive file by resetting the flag's value using the recorded one. Finally, we check whether the sensitive file's content is changed. If so, the flag is treated as critical.
% %
% As for reference objects, we have \code{page} pointer for memory dereference and \code{sector_t} for disk dereference. 
% We obtain the target page address or sector number when performing a valid read operation on a sensitive file. 
% During the valid writing to a read-write file, we substitute the pointer or sector number from the read-write file to the sensitive file. Finally, we read the sensitive file again to inspect whether its content is overwritten.










% \begin{table}[t]
% \centering
% \caption{The summary of exploit strategy to corrupt FSKOs.}
% \label{tab:summary}
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{c|c|c|c}
% \bottomrule[0.1pt]
% \bottomrule[0.1pt]
% Strategy & Target Object   &  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Requirement\\ Information Leakage \end{tabular}}         &  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Requirement\\ Overwriting capability \end{tabular}}    \\ \hline

% \rowcolor{mygray}
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Direct\\ Overwriting \end{tabular}}  
%   & Flags        & /  & One bit flipping    \\ \hline



% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swapping with \\a specific value \end{tabular}}
% & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Flags and\\References \end{tabular}}
%     & Require   & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Corrupting \\ a pointer/integer \end{tabular}}   \\ \hline



% \rowcolor{mygray}
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Swapping\\ (Dirty Cred) \end{tabular}} &
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Flags and\\References \end{tabular}}
%  & /   & Nullify the last few bits    \\ \hline


% % \rowcolor{mygray}
% % \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sector\\ references  in~\cref{tab:identified-ref} \end{tabular}}    & Require   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Corrupt an integer\\ with specific value \end{tabular}}     & Swapping  \\


% Hybrid &
% Bridge objects
%  & /   &  One bit flipping            \\


% \bottomrule[0.1pt]
% \bottomrule[0.1pt]

% \end{tabular}}
% \end{table}


\begin{table}[t]
\centering
\caption{Our exploit strategies apply to FSKOs.}
\label{tab:summary}
\resizebox{1\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule[0.1pt]
\toprule[0.1pt]
\textbf{Strategy} & \textbf{Target} & \textbf{\begin{tabular}[c]{@{}c@{}}Information \\ Leakage\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Memory Corruption \\ Capability\end{tabular}} \\
\midrule
\begin{tabular}[c]{@{}c@{}}Direct \\ overwrite\end{tabular} & Flags & / & One bit flipping    \\ \hline

\multirow{3}*{Swap} & Memory pointers & Required  & Directly set target value  \\ \cline{2-4}

~   &  Memory pointers  & /  & Nullify the last few bits   \\ \cline{2-4}
~   &  Disk sector numbers  & /  & Directly set target value  \\ \hline
Hybrid  & Bridge objects  & / & One bit flipping \\ 

\bottomrule[0.1pt]
\bottomrule[0.1pt]

\end{tabular}}
\end{table}









% However, it places requirements on the bug's capability, including the slab cache it uses, the offset and length it can write, and the value it can set. One special case is the cross-cache exploit, which solves the problem that the vulnerable and target objects are not allocated in the same slab cache. It becomes more difficult because of the manipulation 
% of the buddy system's page.

%In the following, we introduce the possibity the four kinds of

%The basic exploit process is divided into several steps. First, we write a PoC to trigger a vulnerability multiple times to spray vulnerable objects. After that, we spray a bunch of target critical objects in the heap. The spraying continues until a vulnerable object becomes adjacent to a target object (Out-Of-Bounds), or a target object occupies the location of a freed but still vulnerable object (Use-After-Free). Afterward, we utilize the write primitive provided by the vulnerability to corrupt the critical objects with the intended value. Finally, an unprivileged user becomes a root after writing \code{/etc/passwd}. The case will be complicated when considering cross-cache corruption because of the involvement of freeing and requesting pages from the buddy system. But the basic idea of the exploit is the same. We apply the general strategy to the representative objects of four kinds of data mentioned in \cref{sec:key-object-classification}.


%\jim{mark 1234, evaluation table}







\subsection{Exploit Strategy Integration}
\label{sec:exploit-strategy-integration}
%\subsubsection{Overwriting Flag Objects}
%\label{sec:direct-exploit-strategy}
%\jim{Directly corrupting the critical data before the data plays its role.}
%\jim{highlight the key point}

\subsubsection{Direct Overwriting Flags (DO)}
Direct corruption is straightforward without information leaks because the intended value is known in advance, requiring one-bit flipping as shown in~\cref{tab:summary}. By placing the target flag adjacent to the vulnerable object (OOB) or taking the freed slot of the vulnerable (UAF) after heap fengshui, we can directly corrupt the target object with an intended value. 

Besides, we can swap the whole structure containing a flag using the swapping reference strategy in~\cref{sec:swapping-strategy}. For example, there is a flag \code{posix_acl->a_entries->e_perm}, and overwriting its value with \code{MAY_WRITE} achieves root. We can swap the whole permission structure by corrupting the pointer of \code{posix_acl *} type. 
%\PP{Substituting the Whole Flag Object}


\subsubsection{Swapping Objects}
\label{sec:swapping-strategy}
We can swap a reference pointing from one location to another. As for privilege escalation, we can modify the reference pointing from a read-write file (low-privilege) to a read-only file (high-privilege).
Note that both reference objects for file content (i.e., memory pointer and sector integer number) and the wrappers (high-level pointers) can apply the swapping strategy. 

Corrupting sector number does not require an information leakage primitive because unprivileged users can obtain the target value through a valid system call \code{ioctl} that eventually calls \code{ioctl_fiemap} to retrieve the logical and physical block numbers. The sector numbers can be directly computed by shifting several bits. The following paragraphs describe two strategies applied to memory pointers with/without information leakage.




%
%FSKO-level UAF Strategy is a generalized Dirty Cred strategy. It broadens the set of target objects by involving higher-level objects and provides possibilities to match potential bugs with capabilities.
%
%The required bug capability is broadened by writing the higher object's offset that stores \code{file} pointers.
 

%\jim{strength and weakness. Dirty cred has a check}







% For example, the Dirty Cred exploit strategy~\cite{lin2022dirtycred} trigger OOB or UAF to overwrite zero to the last two bytes of the pointer referencing the credential object. The other bugs are unusable for two reasons: 1) They cannot nullify the last two bytes; 2) The bug must corrupt a certain offset in an object, which is a field pointing to the credential, such as \code{file}.


% \noindent \textit{Corrupt Permission.} Dirty Cred~\cite{lin2022dirtycred} highlights that \code{file} and \code{cred} are considered credential objects susceptible to exploitation through the Dirty Cred strategy. In this paper, we also found the \code{file->f_mode} encodes the rwx permission after analyzing the propagation of \code{inode->i_mode}. Besides, \code{inode} also encodes the permission, which allows applying the Dirty Cred strategy. The basic idea of this strategy is as follows: (1) an unprivileged user sprays many low-privilege \code{file} objects, which means opening many of his/her own read-write files. (2) After checking the permission with the low-privilege object, i.e., \code{file->f_mode}, Dirty Cred utilizes FUSE to extend the time window. (3) During the extended time, this strategy swaps the low-privilege \code{file} with a high-privilege \code{file}, a.k.a., the object created for the opened file \code{/etc/passwd}. Therefore, the user can write this sensitive file by accessing its associated page cache without any permission check.


% Dirty Cred strategy is adopted for \code{inode} object due to its inside permission fields, making it a credential object. Similarly, an unprivileged user can create many low-privilege files. Besides, the permission checking of \code{inode} is in \code{sys_open}, and the actual write is performed in \code{sys_write}, which has a long time window without the extending technique. If swapping \code{inode} using the Dirty Cred strategy, the \code{file->f_inode} will point to the high-privilege object instead of directly corrupting the \code{file->f_inode} as mentioned before. The results are the same with swapping and writing the page cache, and only the file system implementations use \code{file->f_inode->i_mapping} to obtain the page cache, e.g., Btrfs.




%\name{} finds many objects can be used to .  as .  


%We use \code{pipe_buffer} as an example to explain the complex strategy, as shown in \cref{fig:exploit} step 1. We repeatedly allocate these objects in the heap to generate multiple objects holding the \code{page *}. The PoC triggering the vulnerability corrupts one of \code{page} pointers, making two pointers pointing to the same \code{page} in step 2. Thanks to the aligned size of 0x40, we only need the bug capability of flipping a single bit. For example, if the \code{page1} address's lower bytes are 0x00, the next one (\code{page2}) will be 0x40, differing by just one bit while sharing the same higher bytes. After making two pointers point to the same \code{page2} object by flipping the bit, we free the \code{page2} through a pointer in step 3, and the corresponding physical page is freed. We can still access the freed page using the other pointer, resulting in a page-level UAF.


%Therefore, we need to corrupt the unprotected objects used in the direct exploit strategy. 

% \noindent \textit{Corrupt Permission \& Write Disk \& Reverse Operation.} The exploit process of these object are similar to the direct exploit strategy \cref{sec:general-exploit-strategy}. The difference is that this strategy sprays many critical objects to request the freed page from the buddy system. Page-level UAF provides a dangling pointer to write the entire content page, i.e., corrupt any objects inside the page with the intended value.


% \noindent \textit{Write Page Cache.} Because the page cache is a part of memory management, and page-level UAF occurs during managing memory.






%In the following, we discuss the details of this exploit strategy and the static analysis to find more objects to show the generality.







\PP{Swapping with Specific Value with Information Leakage (S+I)}
It directly corrupts the pointer's value with the specific value, swapping the pointer pointing from a regular file to a sensitive file. It requires the acquisition of the target value by information leakage, i.e., the target pointer value.



\PP{Swapping without Information Leakage (S)}
As for the memory pointers, there is an advanced method based on specific patterns of their values without information leakage. The heap objects with the same type are allocated in the same slab cache. If we can add an object's size to a pointer, it will point to the next object. Therefore, nullifying a pointer's last two bytes makes it point to the first object on a page, resulting in the swapping of the pointee objects. 



\PP{Relationship with Dirty Cred} 
Dirty Cred is a special case that simultaneously swaps one wrapper in the file system containing the flag and content, i.e., \code{file}. 
Specifically, it nullifies the last two bytes of the \code{file} pointer to construct a \code{file} UAF.
% making it point to the first object on a page. 
% Afterward, freeing the object through one pointer causes a \code{file} UAF; the other dangling pointer can still write the file. 
The UAF swaps from a low-privilege \code{file} to a high-privilege one for a read-only file.
%
\name{} finds out that \code{file} has \code{f_mode} representing permission and \code{f_inode} or \code{f_mapping} representing the file content. After checking the inside permission, Dirty Cred pauses the kernel execution using the FUSE technique. Then, it swaps the whole \code{file} to write the file content through a \code{file} UAF. The wrapper objects contain a pointer pointing to \code{file} to construct \code{file} UAF, such as \code{vdpa_map_file->file} and \code{usb_dev_state->file}. 


The corruption targets can be extended by adding wrappers containing multiple kinds of FSKOs, but it requires comprehensive dynamic verification. 
%
For example, \name{} identifies \code{inode} also contains content and metadata. Furthermore, massive wrappers contain a field of type \code{inode *}, which could be the corrupt targets, for example, \code{binder_device->binderfs_inode}.
%
However, exploitability validation for these wrapper objects presents two challenges.
%
Firstly, it is essential to dynamically trigger all feasible paths of a wrapper to ascertain its effectiveness. Secondly, due to the potential variety of fields within a wrapper, replacing the entire structure can lead to unintended side effects and an anomalous state in the entire system. The verification may require pausing the kernel at specific points to swap the objects, which is challenging also.
Hence, we defer the validation of wrappers to future work. This work identifies only three types of FSKOs, not wrappers, but FSKOs can guide wrapper discovery.



\subsubsection{Hybrid Exploit Strategy (H)}
Due to the various capabilities of different vulnerabilities, some cannot corrupt a single bit but can corrupt multiple bits. To align with these vulnerabilities, we can apply the hybrid exploit strategy by nullifying the last few bits or setting the target value after leaking information. (But the table 2?)
From the exploit results, the hybrid strategy allows reading and writing to a 4KB physical page by corrupting bridge objects resulting from a vulnerability. Subsequently, we can spray FSKOs on the freed page to read or write them. 
%
% The target values of flag objects can be analyzed from the source code in advance, which only requires triggering the write on the page. 
% %
% As for reference objects, we read the target value of the reference of a sensitive read-only file. Afterward, we set the reference of a read-write file as the target value.
%
% Note that the syscalls used vary significantly depending on the specific FSKO being exploited. 
% %
% We will delve into the details using an example to illustrate the general exploit steps, as depicted in \cref{fig:exploit}.


\begin{comment}
    

\PP{Flag Overwriting}
% After obtaining invalid access to a freed page, attackers can fulfill the page with the key flag objects and corrupt them with intended values. As the example in the first four pictures in \cref{fig:exploit}, we trigger vulnerability to construct a page UAF by corrupting a \code{page} pointer allocated in \code{pipe_buffer}. Afterward, we free one pointer, leaving another pointer points to the released page and can write the whole page. 
%
We use \code{pipe_buffer} object as an example, and spray many these objects into the freed page. As shown the first step in second row of~\cref{fig:exploit}, we call \code{splice} to assign the page within the page cache of a read-only file to \code{pipe_buffer->page}, e.g, the file \code{/etc/passwd}. 
Finally, we trigger a write after free by dangling pointer of the freed page to write \code{pipe_buffer->flags}, which is marked in red. The corruption grants an unprivileged user the ability to write the read-only file's page cache.


%In particular, we can corrupt the page cache because it is a part of memory management. The existing exploit~\cite{arttnba30:online} sprays the known and protected objects, including control data, \code{cred}, and page table. These objects are under protection in many commercial kernels mentioned in \cref{sec:motivation}, no longer available. We propose using page UAF to facilitate page cache writing for more stable and less complex exploits. The following sections introduce the details of the exploit (\cref{sec:strategy-page-cache}) and the static analysis to find more feasible objects (\cref{sec:static-analysis-page-cache}).



\PP{Reference Swapping}
%
As shown in \cref{fig:exploit}, two arrays of \code{page} pointer are allocated in the two functions \code{configfs_read_iter} and \code{configfs_write_iter}. 
%
We construct page UAFs in the two functions, enabling the reading and writing of the freed page, respectively. 
%
We spray \code{file} objects on the freed page by opening many read-only files. Then, we read the pointer value stored in \code{file->f_mapping}, which points to the tree of the page cache. 
%
Afterward, we spray read-write \code{file->f_mapping} on another freed page by opening a read-write file. We can corrupt it with the value read before to write read-only files through this \code{file}.
\end{comment}


% \label{sec:strategy-page-cache}
%
%We assume the attacker is only granted limited writing (even one-bit flipping) on a heap object without any read primitive, enabling all mitigation and protection mechanisms. 

% The reference objects are also integrated into this exploit strategy to understand the exploitable objects completely. This understanding helps to design the protection mechanisms to prevent all possible attacks with as few flaws as possible.
% %Some flag objects may not be easy to exploit due to the short time window. Furthermore, we %
% The whole exploit is divided into two main steps after a page UAF construction. First, we fill up the freed page using the objects that contain a \code{page} pointer or the pointer of \code{page} tree. These pointers must point to the read-only file's page cache. 
% %
% (2) It triggers a UAF read on the freed page to get the pointer's value, i.e., the address for the page cache. UAF write is triggered to set to another pointer with the read value, which initially has write permission. Finally, we can write the page cache of a sensitive file. 
% \textbf{Page Cache Separation.}
% After obtaining a page UAF, the straightforward idea is to let a read-only file request the freed page and fill its content, treating it as its page cache. 
% %
% However, the page allocated for the slab cache is separated from the page cache, which means the freed page is never used for page cache. 
% The kernel defines several migration types to group pages with similar movability properties to reduce memory fragments. 
% %The pages in the page cache belong to the type \code{MIGRATE_MOVABLE} group, which is separated from other types, especially the pages used by the slab. 
% Thus, we cannot directly read or write the page cache in the slab cache through the UAF.
% %
% Fortunately, we can cross the group separation to corrupt the \code{page} pointer pointing to the page cache. These pointers are allocated in the slab cache and fall into the corruption scope of page UAF. Besides, \name{} identifies the objects stored with the page cache using reference propagation in \cref{sec:ref-propagation}.

%We use \code{pipe_buffer} as an example to explain the strategy. 


%



% Since the pages allocated for \code{pipe_buffer->page} and the pages for slab cache are in the same group. We can request the freed page by many object allocations using the slab cache, illustrated in step 2-1 of \cref{fig:exploit}. 
% In step 2-2, we assign the page cache's address to the new-allocated objects.
% Specifically, \code{page} pointer in \code{pipe_buffer} can validly point to the cached page when using syscall \code{splice()}. For example, we have the pointer in \circled{3} points to \code{page3} for a read-only file and \circled{4} for \code{page4} of a read-write file. 

% %Therefore, we can leak the address of the cached page of a read-only file by reading the pointer's value in \circled{3}. Back to the exploit, we allocate multiple \code{pipe_buffer} objects to request the freed page from the buddy system for these objects, as depicted in step 4. Then we call \code{splice} to assign the address of the cached page to \code{pipe_buffer->page}. Note the kernel will not allocate a new page until there is a write because of COW.
% %There are data assignments between the page.


% \textbf{Page Cache Read/Write.}
% The kernel provides interfaces to read/write the content in a 4KB physical page through \code{page} pointer. For example, \code{pipe_read} and \code{pipe_write} can access the page by the pointer inside of \code{pipe_buffer}. Specifically, they use the low-level interface, \code{copy_page_to_iter} and \code{copy_page_from_iter}.
% %
% Our exploit uses \circled{2} to read and write (UAF) the freed page full of objects (UAF) pointing page caches. Some point to the read-only file's page cache, and others point to the read-write ones.
% %After calling \code{splice}, the value of \code{page} pointer in \circled{3} is the address of the cached \code{page3} for a read-only file, and another pointer in \circled{4} points to the cached \code{page4} for a normal read-write file. 
% In step 3-1 of \cref{fig:exploit}, \circled{2} provides a read-after-free to obtain the address of \code{page3} for a read-only file. 
% In step 3-2, a write-after-free sets the pointer's value in \circled{4} with the read address. Therefore, the \code{page} pointer's value in \circled{4} is changed from a read-write file to a read-only file. Finally, a normal user can write the read-only file's page cache through \circled{4}.









\begin{comment}
    

\subsubsection{Static Analysis for More Feasible Objects}
\label{sec:static-analysis-page-cache}
We extend \name{} to conduct the first static analysis to find all feasible objects to facilitate the page UAF, making the strategy general from three aspects. The state-of-the-art exploits utilize page UAF to achieve arbitrary read or write~\cite{Interrup28:online, arttnba30:online}. However, these exploits are based on well-known objects, and no systematic analysis exists to find all feasible objects. \name{} (1) first selects the objects in the heap and contains \code{page *} fields, which can be corrupted to achieve page UAF. Subsequently, we trace the data flow of these objects to identify those that (2) are assigned with the page cache and (3) are useful to achieve arbitrary read and write. 

% The exploit is general for many objects to facilitate different parts, making them exploitable to match different capabilities of vulnerabilities. The end of this section discusses the generality and stability of \exploit{}.

% The objects related to the page cache can be abused to write sensitive read-only files. 

(1) The objects cause page UAFs. We identify the objects that contain the \code{page} pointers that point to the page in the same group because a page is recycled within a page group.
%We are interested in two kinds of groups; the page group contains slab pages, and the other one contains the pages in the page cache. 
As discussed before, the page allocated to \code{pipe_buffer}'s inside pointer is in the same group as the slab. We can re-allocate the free page to fill it up with target objects. Besides the group that slab pages belong to, another group that contains the pages in the page cache is also considered.
%For the second type, if a \code{page} pointer points to the \code{page} in the same group as page cache (\code{MIGRATE_MOVABLE}), the exploit will be easier without crossing the page group separation. After obtaining the page-level UAF in step 3, we read a sensitive file using buffered I/O to build its page cache, which requests the freed page. We can directly write the page cache using the UAF. The page cache can be dropped by \code{fadvise} and be created when accessing by buffered I/O for better exploitation.

(2) The objects with the pointer pointing to the \code{page} for a read-only file. 
Initially, the \code{page} pointers in a file's page cache are organized by \code{address_space} as a radix tree \code{xarray} that is stored in \code{inode}. 
%The corresponding \code{page} pointers are stored in the tree, actually. 
However, the pointer spreads throughout the kernel, leading to many objects being assigned with the pointer. Using these assigned objects, we can leak the address of \code{page} used by the page cache. 
%are granted the address of the cached page.


(3) The objects involved in interfaces to read and write the page content.
Numerous objects have fields of type \code{page} pointer, which the kernel uses to copy in/out user buffer. \name{} identifies these objects by analyzing the copying interfaces from their usage paths. 


%All files share the states of the flag objects, so the exploit can directly corrupt a flag with a known value in advance. On the contrary, the exploits of the reference objects must leak the target location. Intuitively, we rely on the read primitive provided by a vulnerability. To dispense with the read primitive, we propose a new exploit technique: \exploit{} for page reference, given a limited write primitive only. Therefore, we introduce the conventional method to corrupt non-page objects, including the flag and sector reference objects. Subsequently, we delve into the specifics of \exploit{} tailored to page references.
\end{comment}


%\subsection{Dirty Cred Strategy}









\begin{comment}
    


\subsection{\exploit{}: Exploit Technique on Page Cache}
\jim{make it compact and merge it to section 6.2}
We propose a new exploit technique: \exploit{} to write the file content in the page cache. 
We assume the kernel enables all exploit mitigation and protection mechanisms. \textit{The attacker is only granted limited writing on a heap object, even flipping one bit, without any read primitive.} The exploit begins by constructing a page-level UAF by corrupting a limited heap memory. Before delving into the strategy specifics, we introduce the allocation of \code{page} structure, which plays a critical role in locating the target object. Then, we fill up the invalid freed page using the target object that contains a \code{page} pointer pointing to the read-only file's content. Then, trigger the UAF to read the value of the \code{page} pointer. UAF is used again to write to another pointer with the read value, making it point to the page cache. Finally, we write to the page cache through the corrupted pointer. We use \code{pipe_buffer} as an example to explain the complex strategy. The exploit is general for many objects to facilitate different parts, making them exploitable to match different capabilities of vulnerabilities. The end of this section discusses the generality and stability of \exploit{}.




\subsubsection{Exploit Generality}
We first discuss additional objects that facilitate different parts of the exploit, making \exploit{} more general for vulnerabilities with various capabilities. Next, we demonstrate the practicality of this strategy. The required capability is relatively easy to satisfy for a real-world heap-based vulnerability. 
Finally, we discuss the stability of this exploit that avoids the wrong place corruption to make the kernel crash. 

\noindent \textit{More Exploitable Objects.}
\label{sec:more-page-objects}
We can use different objects in the three exploit parts, and the results are shown at \cref{sec:imp-eva}. The reason we select \code{pipe_buffer} is that it happens to fulfill the three requirements as follows.

(1) The objects cause page-level UAFs. We implement \name{} to identify the objects that contain the \code{page} pointers that point to the page in the same group. Because the pages in the same group can be adjacent. A page freed by one pointer can be reallocated to another pointer if the two pointers point to the same group.
%We are interested in two kinds of groups; the page group contains slab pages, and the other one contains the pages in the page cache. 
As discussed before, the page allocated to \code{pipe_buffer}'s inside pointer is in the same group as the slab. We can re-allocate the free page to fill it up with target objects. Besides the group that slab pages belong to, another group that contains the pages in the page cache is also considered.
%For the second type, if a \code{page} pointer points to the \code{page} in the same group as page cache (\code{MIGRATE_MOVABLE}), the exploit will be easier without crossing the page group separation. After obtaining the page-level UAF in step 3, we read a sensitive file using buffered I/O to build its page cache, which requests the freed page. We can directly write the page cache using the UAF. The page cache can be dropped by \code{fadvise} and be created when accessing by buffered I/O for better exploitation.


(2) The objects with the pointer pointing to the \code{page} for a read-only file. 
Initially, the \code{page} pointers in a file's page cache are organized by \code{address_space} as a radix tree \code{xarray} that is stored in \code{inode}. 
%The corresponding \code{page} pointers are stored in the tree, actually. 
However, the pointer spreads throughout the kernel, leading to many objects being assigned with the pointer. Using these assigned objects, we can leak the address of \code{page} used by the page cache. The trace of the page cache assignment is discussed at \cref{sec:tracing-reference}.
%are granted the address of the cached page.


(3) The objects involved in interfaces to read and write the page content.
Numerous objects have fields of type \code{page} pointer, which the kernel uses to copy in/out user buffer. \name{} identifies these objects by analyzing the copying interfaces from their usage paths.  


\noindent \textit{Required Vulnerability.}
\exploit{} requires a limited write on kernel heap memory without any read primitive. By flipping the bit aligned with 0x40, the size of \code{page}, we can move a pointer's value from the address of one \code{page} to another. Furthermore, we can corrupt the least several bits to zero, making it a point to the first \code{page} object in a physical page, as DirtyCread does \cite{lin2022dirtycred}. We demonstrate the practicality by using real-world CVEs in \cref{sec:imp-eva}.



\noindent \textit{Exploit Stability.}
Maintaining kernel stability during the exploit is crucial. We achieve this by leveraging the interface \code{copy_page_to_iter}, which allows us to read the page content to a user buffer. We can read the pointer's value on the page to ensure to obtain the target address without guessing. Additionally, we compare the page's content with the file's content to confirm that the \code{page} address is for a read-only file. All these reading operations are carefully performed to avoid crashing the kernel. The possibility of obtaining the freed page is relatively high because \code{page} directly frees a physical page to the buddy system. There will be more noise when freeing all objects used by the slab to return the slab page to the buddy system, as \cite{US22WANG2:online} does.

\end{comment}
